GPT-NeoX-20B: An Open-Source Autoregressive Language Model

We introduce GPT-NeoX-20B, a 20 billion parameter autoregressive language model trained on the Pile, whose weights will be made freely and openly available to the public through a permissive license. It is, to the best of our knowledge, the largest dense autoregressive model that has publicly available weights at the time of submission. In this work, we describe \model{}'s architecture and training and evaluate its performance on a range of language-understanding, mathematics, and knowledge-based tasks. We find that GPT-NeoX-20B is a particularly powerful few-shot reasoner and gains far more in performance when evaluated five-shot than similarly sized GPT-3 and FairSeq models. We open-source the training and evaluation code, as well as the model weights, at https://github.com/EleutherAI/gpt-neox.

==> Figures/tokenization/examples_new/Books3.tex <==
\begin{minipage}{\textwidth}
\subcaption*{{GPT-2 Tokenization}}
\small\vspace{-0.5\baselineskip}\centering{258 tokens}
\begin{tokenized}
\parbox{\linewidth}{\small
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{**}\linebreak[3]\tokenbox{EAR}\linebreak[3]\tokenbox{LY}\linebreak[3]\tokenbox{~B}\linebreak[3]\tokenbox{IRD}\linebreak[3]\tokenbox{~BOOK}\linebreak[3]\tokenbox{S}\linebreak[3]\tokenbox{**}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{**}\linebreak[3]\tokenbox{FR}\linebreak[3]\tokenbox{ESH}\linebreak[3]\tokenbox{~E}\linebreak[3]\tokenbox{BOOK}\linebreak[3]\tokenbox{~DE}\linebreak[3]\tokenbox{ALS}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~DEL}\linebreak[3]\tokenbox{IVER}\linebreak[3]\tokenbox{ED}\linebreak[3]\tokenbox{~DA}\linebreak[3]\tokenbox{ILY}\linebreak[3]\tokenbox{**}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{BE}\linebreak[3]\tokenbox{~THE}\linebreak[3]\tokenbox{~FIRST}\linebreak[3]\tokenbox{~TO}\linebreak[3]\tokenbox{~KNOW}\linebreak[3]\tokenbox{—}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{NEW}\linebreak[3]\tokenbox{~DE}\linebreak[3]\tokenbox{ALS}\linebreak[3]\tokenbox{~H}\linebreak[3]\tokenbox{ATCH}\linebreak[3]\tokenbox{~EVERY}\linebreak[3]\tokenbox{~DAY}\linebreak[3]\tokenbox{!}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{P}\linebreak[3]\tokenbox{raise}\linebreak[3]\tokenbox{~for}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~Age}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~Un}\linebreak[3]\tokenbox{reason}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{"}\linebreak[3]\tokenbox{~\_}\linebreak[3]\tokenbox{New}\linebreak[3]\tokenbox{ton}\linebreak[3]\tokenbox{'s}\linebreak[3]\tokenbox{~Cannon}\linebreak[3]\tokenbox{\_}\linebreak[3]\tokenbox{~features}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~classic}\linebreak[3]\tokenbox{~elements}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~science}\linebreak[3]\tokenbox{~fiction}\linebreak[3]\tokenbox{:}\linebreak[3]\tokenbox{~high}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{tech}\linebreak[3]\tokenbox{~gadget}\linebreak[3]\tokenbox{ry}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~world}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{threatening}\linebreak[3]\tokenbox{~superpower}\linebreak[3]\tokenbox{~conflict}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~quest}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~save}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~world}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~teen}\linebreak[3]\tokenbox{~hero}\linebreak[3]\tokenbox{~who}\linebreak[3]\tokenbox{'s}\linebreak[3]\tokenbox{~smarter}\linebreak[3]\tokenbox{~than}\linebreak[3]\tokenbox{~most}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~adults}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~The}\linebreak[3]\tokenbox{~historical}\linebreak[3]\tokenbox{~setting}\linebreak[3]\tokenbox{~gives}\linebreak[3]\tokenbox{~this}\linebreak[3]\tokenbox{~book}\linebreak[3]\tokenbox{~something}\linebreak[3]\tokenbox{~extra}\linebreak[3]\tokenbox{...}\linebreak[3]\tokenbox{~Powerful}\linebreak[3]\tokenbox{."}\linebreak[3]\tokenbox{~—}\linebreak[3]\tokenbox{~\_}\linebreak[3]\tokenbox{USA}\linebreak[3]\tokenbox{~Today}\linebreak[3]\tokenbox{\_}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{"}\linebreak[3]\tokenbox{Prom}\linebreak[3]\tokenbox{ises}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~follow}\linebreak[3]\tokenbox{~honor}\linebreak[3]\tokenbox{ably}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~footsteps}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~[}\linebreak[3]\tokenbox{Or}\linebreak[3]\tokenbox{son}\linebreak[3]\tokenbox{~Scott}\linebreak[3]\tokenbox{]}\linebreak[3]\tokenbox{~Card}\linebreak[3]\tokenbox{'s}\linebreak[3]\tokenbox{~\_}\linebreak[3]\tokenbox{Al}\linebreak[3]\tokenbox{vin}\linebreak[3]\tokenbox{~Maker}\linebreak[3]\tokenbox{\_}\linebreak[3]\tokenbox{~saga}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~Key}\linebreak[3]\tokenbox{es}\linebreak[3]\tokenbox{~knows}\linebreak[3]\tokenbox{~his}\linebreak[3]\tokenbox{~history}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~knows}\linebreak[3]\tokenbox{~his}\linebreak[3]\tokenbox{~science}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~knows}\linebreak[3]\tokenbox{~how}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~tell}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~story}\linebreak[3]\tokenbox{."}\linebreak[3]\tokenbox{~—}\linebreak[3]\tokenbox{~\_}\linebreak[3]\tokenbox{Book}\linebreak[3]\tokenbox{list}\linebreak[3]\tokenbox{\_}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{"}\linebreak[3]\tokenbox{Master}\linebreak[3]\tokenbox{ful}\linebreak[3]\tokenbox{...}\linebreak[3]\tokenbox{~A}\linebreak[3]\tokenbox{~brav}\linebreak[3]\tokenbox{ura}\linebreak[3]\tokenbox{~performance}\linebreak[3]\tokenbox{...}\linebreak[3]\tokenbox{~[}\linebreak[3]\tokenbox{An}\linebreak[3]\tokenbox{]}\linebreak[3]\tokenbox{~ingenious}\linebreak[3]\tokenbox{~m}\linebreak[3]\tokenbox{é}\linebreak[3]\tokenbox{l}\linebreak[3]\tokenbox{ange}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~Age}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~Un}\linebreak[3]\tokenbox{reason}\linebreak[3]\tokenbox{~period}\linebreak[3]\tokenbox{~details}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~stunning}\linebreak[3]\tokenbox{~psychic}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~al}\linebreak[3]\tokenbox{chemical}\linebreak[3]\tokenbox{~phenomena}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~[}\linebreak[3]\tokenbox{and}\linebreak[3]\tokenbox{]}\linebreak[3]\tokenbox{~fetch}\linebreak[3]\tokenbox{ing}\linebreak[3]\tokenbox{~poetic}\linebreak[3]\tokenbox{~descriptions}\linebreak[3]\tokenbox{...}\linebreak[3]\tokenbox{~Lav}\linebreak[3]\tokenbox{ish}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~thoughtful}\linebreak[3]\tokenbox{."}\linebreak[3]\tokenbox{~—}\linebreak[3]\tokenbox{~\_}\linebreak[3]\tokenbox{Publisher}\linebreak[3]\tokenbox{s}\linebreak[3]\tokenbox{~Weekly}\linebreak[3]\tokenbox{\_}\linebreak[3]\tokenbox{~,}\linebreak[3]\tokenbox{~starred}\linebreak[3]\tokenbox{~review}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{"}\linebreak[3]\tokenbox{In}\linebreak[3]\tokenbox{vent}\linebreak[3]\tokenbox{ive}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~exciting}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~filled}\linebreak[3]\tokenbox{~with}\linebreak[3]\tokenbox{~clever}\linebreak[3]\tokenbox{~details}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~high}\linebreak[3]\tokenbox{~adventure}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~[}\linebreak[3]\tokenbox{~\_}\linebreak[3]\tokenbox{The}\linebreak[3]\tokenbox{~Shadows}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~God}\linebreak[3]\tokenbox{\_}\linebreak[3]\tokenbox{~]}\linebreak[3]\tokenbox{~brings}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~close}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~sequence}\linebreak[3]\tokenbox{~that}\linebreak[3]\tokenbox{~seem}\linebreak[3]
}
\end{tokenized}
\end{minipage}
\vskip1.5em
\begin{minipage}{\textwidth}
\subcaption*{{\model{} Tokenization}}
\small\vspace{-0.5\baselineskip}\centering{263 tokens}
\begin{tokenized}
\parbox{\linewidth}{\small
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{**}\linebreak[3]\tokenbox{E}\linebreak[3]\tokenbox{AR}\linebreak[3]\tokenbox{LY}\linebreak[3]\tokenbox{~B}\linebreak[3]\tokenbox{IRD}\linebreak[3]\tokenbox{~B}\linebreak[3]\tokenbox{OO}\linebreak[3]\tokenbox{KS}\linebreak[3]\tokenbox{**}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{**}\linebreak[3]\tokenbox{FR}\linebreak[3]\tokenbox{ESH}\linebreak[3]\tokenbox{~EB}\linebreak[3]\tokenbox{OOK}\linebreak[3]\tokenbox{~DE}\linebreak[3]\tokenbox{ALS}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~DEL}\linebreak[3]\tokenbox{IVER}\linebreak[3]\tokenbox{ED}\linebreak[3]\tokenbox{~DA}\linebreak[3]\tokenbox{ILY}\linebreak[3]\tokenbox{**}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{BE}\linebreak[3]\tokenbox{~THE}\linebreak[3]\tokenbox{~FIRST}\linebreak[3]\tokenbox{~TO}\linebreak[3]\tokenbox{~KNOW}\linebreak[3]\tokenbox{—}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{NEW}\linebreak[3]\tokenbox{~DE}\linebreak[3]\tokenbox{ALS}\linebreak[3]\tokenbox{~H}\linebreak[3]\tokenbox{ATCH}\linebreak[3]\tokenbox{~EVERY}\linebreak[3]\tokenbox{~DAY}\linebreak[3]\tokenbox{!}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{P}\linebreak[3]\tokenbox{raise}\linebreak[3]\tokenbox{~for}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~Age}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~Un}\linebreak[3]\tokenbox{reason}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{"}\linebreak[3]\tokenbox{~\_}\linebreak[3]\tokenbox{Newton}\linebreak[3]\tokenbox{'s}\linebreak[3]\tokenbox{~Cannon}\linebreak[3]\tokenbox{\_}\linebreak[3]\tokenbox{~features}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~classic}\linebreak[3]\tokenbox{~elements}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~science}\linebreak[3]\tokenbox{~fiction}\linebreak[3]\tokenbox{:}\linebreak[3]\tokenbox{~high}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{tech}\linebreak[3]\tokenbox{~gad}\linebreak[3]\tokenbox{get}\linebreak[3]\tokenbox{ry}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~world}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{threatening}\linebreak[3]\tokenbox{~super}\linebreak[3]\tokenbox{power}\linebreak[3]\tokenbox{~conflict}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~quest}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~save}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~world}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~teen}\linebreak[3]\tokenbox{~hero}\linebreak[3]\tokenbox{~who}\linebreak[3]\tokenbox{'s}\linebreak[3]\tokenbox{~smarter}\linebreak[3]\tokenbox{~than}\linebreak[3]\tokenbox{~most}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~adults}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~The}\linebreak[3]\tokenbox{~historical}\linebreak[3]\tokenbox{~setting}\linebreak[3]\tokenbox{~gives}\linebreak[3]\tokenbox{~this}\linebreak[3]\tokenbox{~book}\linebreak[3]\tokenbox{~something}\linebreak[3]\tokenbox{~extra}\linebreak[3]\tokenbox{...}\linebreak[3]\tokenbox{~Power}\linebreak[3]\tokenbox{ful}\linebreak[3]\tokenbox{."}\linebreak[3]\tokenbox{~—}\linebreak[3]\tokenbox{~\_}\linebreak[3]\tokenbox{USA}\linebreak[3]\tokenbox{~Today}\linebreak[3]\tokenbox{\_}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{"}\linebreak[3]\tokenbox{Prom}\linebreak[3]\tokenbox{ises}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~follow}\linebreak[3]\tokenbox{~honor}\linebreak[3]\tokenbox{ably}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~footsteps}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~[}\linebreak[3]\tokenbox{Or}\linebreak[3]\tokenbox{son}\linebreak[3]\tokenbox{~Scott}\linebreak[3]\tokenbox{]}\linebreak[3]\tokenbox{~Card}\linebreak[3]\tokenbox{'s}\linebreak[3]\tokenbox{~\_}\linebreak[3]\tokenbox{Al}\linebreak[3]\tokenbox{vin}\linebreak[3]\tokenbox{~Maker}\linebreak[3]\tokenbox{\_}\linebreak[3]\tokenbox{~saga}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~Key}\linebreak[3]\tokenbox{es}\linebreak[3]\tokenbox{~knows}\linebreak[3]\tokenbox{~his}\linebreak[3]\tokenbox{~history}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~knows}\linebreak[3]\tokenbox{~his}\linebreak[3]\tokenbox{~science}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~knows}\linebreak[3]\tokenbox{~how}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~tell}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~story}\linebreak[3]\tokenbox{."}\linebreak[3]\tokenbox{~—}\linebreak[3]\tokenbox{~\_}\linebreak[3]\tokenbox{Book}\linebreak[3]\tokenbox{list}\linebreak[3]\tokenbox{\_}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{"}\linebreak[3]\tokenbox{Master}\linebreak[3]\tokenbox{ful}\linebreak[3]\tokenbox{...}\linebreak[3]\tokenbox{~A}\linebreak[3]\tokenbox{~brav}\linebreak[3]\tokenbox{ura}\linebreak[3]\tokenbox{~performance}\linebreak[3]\tokenbox{...}\linebreak[3]\tokenbox{~[}\linebreak[3]\tokenbox{An}\linebreak[3]\tokenbox{]}\linebreak[3]\tokenbox{~ingen}\linebreak[3]\tokenbox{ious}\linebreak[3]\tokenbox{~m}\linebreak[3]\tokenbox{él}\linebreak[3]\tokenbox{ange}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~Age}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~Un}\linebreak[3]\tokenbox{reason}\linebreak[3]\tokenbox{~period}\linebreak[3]\tokenbox{~details}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~stunning}\linebreak[3]\tokenbox{~psychic}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~al}\linebreak[3]\tokenbox{chemical}\linebreak[3]\tokenbox{~phenomena}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~[}\linebreak[3]\tokenbox{and}\linebreak[3]\tokenbox{]}\linebreak[3]\tokenbox{~fet}\linebreak[3]\tokenbox{ching}\linebreak[3]\tokenbox{~poetic}\linebreak[3]\tokenbox{~descriptions}\linebreak[3]\tokenbox{...}\linebreak[3]\tokenbox{~Lav}\linebreak[3]\tokenbox{ish}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~thoughtful}\linebreak[3]\tokenbox{."}\linebreak[3]\tokenbox{~—}\linebreak[3]\tokenbox{~\_}\linebreak[3]\tokenbox{Publ}\linebreak[3]\tokenbox{ishers}\linebreak[3]\tokenbox{~Weekly}\linebreak[3]\tokenbox{\_}\linebreak[3]\tokenbox{~,}\linebreak[3]\tokenbox{~starred}\linebreak[3]\tokenbox{~review}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{"}\linebreak[3]\tokenbox{In}\linebreak[3]\tokenbox{vent}\linebreak[3]\tokenbox{ive}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~exciting}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~filled}\linebreak[3]\tokenbox{~with}\linebreak[3]\tokenbox{~clever}\linebreak[3]\tokenbox{~details}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~high}\linebreak[3]\tokenbox{~adventure}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~[}\linebreak[3]\tokenbox{~\_}\linebreak[3]\tokenbox{The}\linebreak[3]\tokenbox{~Sh}\linebreak[3]\tokenbox{adows}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~God}\linebreak[3]\tokenbox{\_}\linebreak[3]\tokenbox{~]}\linebreak[3]\tokenbox{~brings}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~close}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~sequence}\linebreak[3]\tokenbox{~that}\linebreak[3]\tokenbox{~seem}\linebreak[3]
}
\end{tokenized}
\end{minipage}

==> Figures/tokenization/examples_new/Enron_Emails.tex <==
\begin{minipage}{\textwidth}
\subcaption*{{GPT-2 Tokenization}}
\small\vspace{-0.5\baselineskip}\centering{206 tokens}
\begin{tokenized}
\parbox{\linewidth}{\small
\tokenbox{Sh}\linebreak[3]\tokenbox{ir}\linebreak[3]\tokenbox{ley}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{Please}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~cancel}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~talk}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{V}\linebreak[3]\tokenbox{ince}\linebreak[3]\tokenbox{$\hookleftarrow$$\hookleftarrow$}\newline
\tokenbox{~-----}\linebreak[3]\tokenbox{Original}\linebreak[3]\tokenbox{~Message}\linebreak[3]\tokenbox{-----}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{From}\linebreak[3]\tokenbox{:}\linebreak[3]\tokenbox{~}\linebreak[3]\tokenbox{$\longrightarrow$}\linebreak[3]\tokenbox{"}\linebreak[3]\tokenbox{P}\linebreak[3]\tokenbox{rak}\linebreak[3]\tokenbox{ash}\linebreak[3]\tokenbox{~Nar}\linebreak[3]\tokenbox{ayan}\linebreak[3]\tokenbox{an}\linebreak[3]\tokenbox{"}\linebreak[3]\tokenbox{~<}\linebreak[3]\tokenbox{pn}\linebreak[3]\tokenbox{ar}\linebreak[3]\tokenbox{ayan}\linebreak[3]\tokenbox{@}\linebreak[3]\tokenbox{and}\linebreak[3]\tokenbox{rew}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{cm}\linebreak[3]\tokenbox{u}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{edu}\linebreak[3]\tokenbox{>}\linebreak[3]\tokenbox{@}\linebreak[3]\tokenbox{EN}\linebreak[3]\tokenbox{RON}\linebreak[3]\tokenbox{~}\linebreak[3]\tokenbox{~}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{Sent}\linebreak[3]\tokenbox{:}\linebreak[3]\tokenbox{$\longrightarrow$}\linebreak[3]\tokenbox{Sunday}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~December}\linebreak[3]\tokenbox{~02}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~2001}\linebreak[3]\tokenbox{~9}\linebreak[3]\tokenbox{:}\linebreak[3]\tokenbox{28}\linebreak[3]\tokenbox{~PM}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{To}\linebreak[3]\tokenbox{:}\linebreak[3]\tokenbox{$\longrightarrow$}\linebreak[3]\tokenbox{K}\linebreak[3]\tokenbox{am}\linebreak[3]\tokenbox{inski}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~Vince}\linebreak[3]\tokenbox{~J}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{C}\linebreak[3]\tokenbox{c}\linebreak[3]\tokenbox{:}\linebreak[3]\tokenbox{$\longrightarrow$}\linebreak[3]\tokenbox{C}\linebreak[3]\tokenbox{ren}\linebreak[3]\tokenbox{shaw}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~Shirley}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{Subject}\linebreak[3]\tokenbox{:}\linebreak[3]\tokenbox{$\longrightarrow$}\linebreak[3]\tokenbox{Talk}\linebreak[3]\tokenbox{~on}\linebreak[3]\tokenbox{~Friday}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{Dear}\linebreak[3]\tokenbox{~Vince}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{How}\linebreak[3]\tokenbox{~are}\linebreak[3]\tokenbox{~you}\linebreak[3]\tokenbox{?}\linebreak[3]\tokenbox{~I}\linebreak[3]\tokenbox{~understand}\linebreak[3]\tokenbox{~that}\linebreak[3]\tokenbox{~things}\linebreak[3]\tokenbox{~are}\linebreak[3]\tokenbox{~extremely}\linebreak[3]\tokenbox{~he}\linebreak[3]\tokenbox{ctic}\linebreak[3]\tokenbox{~for}\linebreak[3]\tokenbox{~you}\linebreak[3]\tokenbox{~right}\linebreak[3]\tokenbox{~now}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{but}\linebreak[3]\tokenbox{~I}\linebreak[3]\tokenbox{~was}\linebreak[3]\tokenbox{~wondering}\linebreak[3]\tokenbox{~if}\linebreak[3]\tokenbox{~we}\linebreak[3]\tokenbox{~are}\linebreak[3]\tokenbox{~going}\linebreak[3]\tokenbox{~ahead}\linebreak[3]\tokenbox{~as}\linebreak[3]\tokenbox{~schedule}\linebreak[3]\tokenbox{f}\linebreak[3]\tokenbox{~on}\linebreak[3]\tokenbox{~fr}\linebreak[3]\tokenbox{iday}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~It}\linebreak[3]\tokenbox{~would}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{be}\linebreak[3]\tokenbox{~great}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~hear}\linebreak[3]\tokenbox{~from}\linebreak[3]\tokenbox{~you}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{Best}\linebreak[3]\tokenbox{~Reg}\linebreak[3]\tokenbox{ards}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{P}\linebreak[3]\tokenbox{rak}\linebreak[3]\tokenbox{ash}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{P}\linebreak[3]\tokenbox{rak}\linebreak[3]\tokenbox{ash}\linebreak[3]\tokenbox{~Nar}\linebreak[3]\tokenbox{ayan}\linebreak[3]\tokenbox{an}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{412}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{422}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{3}\linebreak[3]\tokenbox{287}\linebreak[3]\tokenbox{~(}\linebreak[3]\tokenbox{Home}\linebreak[3]\tokenbox{)}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{412}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{607}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{53}\linebreak[3]\tokenbox{21}\linebreak[3]\tokenbox{~(}\linebreak[3]\tokenbox{Mobile}\linebreak[3]\tokenbox{)}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{63}\linebreak[3]\tokenbox{15}\linebreak[3]\tokenbox{~Forbes}\linebreak[3]\tokenbox{~Avenue}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{Ap}\linebreak[3]\tokenbox{artment}\linebreak[3]\tokenbox{~\#}\linebreak[3]\tokenbox{~8}\linebreak[3]\tokenbox{09}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{Pitt}\linebreak[3]\tokenbox{sburgh}\linebreak[3]\tokenbox{~PA}\linebreak[3]\tokenbox{~15}\linebreak[3]\tokenbox{217}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{pn}\linebreak[3]\tokenbox{ar}\linebreak[3]\tokenbox{ayan}\linebreak[3]\tokenbox{@}\linebreak[3]\tokenbox{and}\linebreak[3]\tokenbox{rew}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{cm}\linebreak[3]\tokenbox{u}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{edu}\linebreak[3]
}
\end{tokenized}
\end{minipage}
\vskip1.5em
\begin{minipage}{\textwidth}
\subcaption*{{\model{} Tokenization}}
\small\vspace{-0.5\baselineskip}\centering{204 tokens}
\begin{tokenized}
\parbox{\linewidth}{\small
\tokenbox{Shirley}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{Please}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~cancel}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~talk}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{V}\linebreak[3]\tokenbox{ince}\linebreak[3]\tokenbox{$\hookleftarrow$$\hookleftarrow$}\newline
\tokenbox{~-----}\linebreak[3]\tokenbox{Original}\linebreak[3]\tokenbox{~Message}\linebreak[3]\tokenbox{-----}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{From}\linebreak[3]\tokenbox{:}\linebreak[3]\tokenbox{~}\linebreak[3]\tokenbox{$\longrightarrow$}\linebreak[3]\tokenbox{"}\linebreak[3]\tokenbox{P}\linebreak[3]\tokenbox{rak}\linebreak[3]\tokenbox{ash}\linebreak[3]\tokenbox{~Nar}\linebreak[3]\tokenbox{ayan}\linebreak[3]\tokenbox{an}\linebreak[3]\tokenbox{"}\linebreak[3]\tokenbox{~<}\linebreak[3]\tokenbox{pn}\linebreak[3]\tokenbox{ar}\linebreak[3]\tokenbox{ayan}\linebreak[3]\tokenbox{@}\linebreak[3]\tokenbox{and}\linebreak[3]\tokenbox{rew}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{c}\linebreak[3]\tokenbox{mu}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{edu}\linebreak[3]\tokenbox{>}\linebreak[3]\tokenbox{@}\linebreak[3]\tokenbox{ENRON}\linebreak[3]\tokenbox{~~}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{}\linebreak[3]\tokenbox{Sent}\linebreak[3]\tokenbox{:}\linebreak[3]\tokenbox{$\longrightarrow$}\linebreak[3]\tokenbox{Sunday}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~December}\linebreak[3]\tokenbox{~02}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~2001}\linebreak[3]\tokenbox{~9}\linebreak[3]\tokenbox{:}\linebreak[3]\tokenbox{28}\linebreak[3]\tokenbox{~PM}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{To}\linebreak[3]\tokenbox{:}\linebreak[3]\tokenbox{$\longrightarrow$}\linebreak[3]\tokenbox{Kam}\linebreak[3]\tokenbox{inski}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~Vince}\linebreak[3]\tokenbox{~J}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{C}\linebreak[3]\tokenbox{c}\linebreak[3]\tokenbox{:}\linebreak[3]\tokenbox{$\longrightarrow$}\linebreak[3]\tokenbox{C}\linebreak[3]\tokenbox{ren}\linebreak[3]\tokenbox{shaw}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~Shirley}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{Subject}\linebreak[3]\tokenbox{:}\linebreak[3]\tokenbox{$\longrightarrow$}\linebreak[3]\tokenbox{Talk}\linebreak[3]\tokenbox{~on}\linebreak[3]\tokenbox{~Friday}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{Dear}\linebreak[3]\tokenbox{~Vince}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{How}\linebreak[3]\tokenbox{~are}\linebreak[3]\tokenbox{~you}\linebreak[3]\tokenbox{?}\linebreak[3]\tokenbox{~I}\linebreak[3]\tokenbox{~understand}\linebreak[3]\tokenbox{~that}\linebreak[3]\tokenbox{~things}\linebreak[3]\tokenbox{~are}\linebreak[3]\tokenbox{~extremely}\linebreak[3]\tokenbox{~he}\linebreak[3]\tokenbox{ctic}\linebreak[3]\tokenbox{~for}\linebreak[3]\tokenbox{~you}\linebreak[3]\tokenbox{~right}\linebreak[3]\tokenbox{~now}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{but}\linebreak[3]\tokenbox{~I}\linebreak[3]\tokenbox{~was}\linebreak[3]\tokenbox{~wondering}\linebreak[3]\tokenbox{~if}\linebreak[3]\tokenbox{~we}\linebreak[3]\tokenbox{~are}\linebreak[3]\tokenbox{~going}\linebreak[3]\tokenbox{~ahead}\linebreak[3]\tokenbox{~as}\linebreak[3]\tokenbox{~schedule}\linebreak[3]\tokenbox{f}\linebreak[3]\tokenbox{~on}\linebreak[3]\tokenbox{~fr}\linebreak[3]\tokenbox{iday}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~It}\linebreak[3]\tokenbox{~would}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{be}\linebreak[3]\tokenbox{~great}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~hear}\linebreak[3]\tokenbox{~from}\linebreak[3]\tokenbox{~you}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{Best}\linebreak[3]\tokenbox{~Reg}\linebreak[3]\tokenbox{ards}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{P}\linebreak[3]\tokenbox{rak}\linebreak[3]\tokenbox{ash}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{P}\linebreak[3]\tokenbox{rak}\linebreak[3]\tokenbox{ash}\linebreak[3]\tokenbox{~Nar}\linebreak[3]\tokenbox{ayan}\linebreak[3]\tokenbox{an}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{412}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{422}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{32}\linebreak[3]\tokenbox{87}\linebreak[3]\tokenbox{~(}\linebreak[3]\tokenbox{Home}\linebreak[3]\tokenbox{)}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{412}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{607}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{5}\linebreak[3]\tokenbox{321}\linebreak[3]\tokenbox{~(}\linebreak[3]\tokenbox{Mobile}\linebreak[3]\tokenbox{)}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{63}\linebreak[3]\tokenbox{15}\linebreak[3]\tokenbox{~Forbes}\linebreak[3]\tokenbox{~Avenue}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{Apart}\linebreak[3]\tokenbox{ment}\linebreak[3]\tokenbox{~\#}\linebreak[3]\tokenbox{~8}\linebreak[3]\tokenbox{09}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{P}\linebreak[3]\tokenbox{itt}\linebreak[3]\tokenbox{s}\linebreak[3]\tokenbox{burgh}\linebreak[3]\tokenbox{~PA}\linebreak[3]\tokenbox{~15}\linebreak[3]\tokenbox{217}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{pn}\linebreak[3]\tokenbox{ar}\linebreak[3]\tokenbox{ayan}\linebreak[3]\tokenbox{@}\linebreak[3]\tokenbox{and}\linebreak[3]\tokenbox{rew}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{c}\linebreak[3]\tokenbox{mu}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{edu}\linebreak[3]
}
\end{tokenized}
\end{minipage}

==> Figures/tokenization/examples_new/EuroParl.tex <==
\begin{minipage}{\textwidth}
\subcaption*{{GPT-2 Tokenization}}
\small\vspace{-0.5\baselineskip}\centering{533 tokens}
\begin{tokenized}
\parbox{\linewidth}{\small
\tokenbox{Let}\linebreak[3]\tokenbox{i}\linebreak[3]\tokenbox{š}\linebreak[3]\tokenbox{tn}\linebreak[3]\tokenbox{í}\linebreak[3]\tokenbox{~pop}\linebreak[3]\tokenbox{lat}\linebreak[3]\tokenbox{ky}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{P}\linebreak[3]\tokenbox{ř}\linebreak[3]\tokenbox{}\linebreak[3]\tokenbox{eds}\linebreak[3]\tokenbox{ed}\linebreak[3]\tokenbox{aj}\linebreak[3]\tokenbox{í}\linebreak[3]\tokenbox{c}\linebreak[3]\tokenbox{í}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{D}\linebreak[3]\tokenbox{al}\linebreak[3]\tokenbox{š}\linebreak[3]\tokenbox{í}\linebreak[3]\tokenbox{~bod}\linebreak[3]\tokenbox{em}\linebreak[3]\tokenbox{~j}\linebreak[3]\tokenbox{ed}\linebreak[3]\tokenbox{n}\linebreak[3]\tokenbox{án}\linebreak[3]\tokenbox{í}\linebreak[3]\tokenbox{~je}\linebreak[3]\tokenbox{~dop}\linebreak[3]\tokenbox{oru}\linebreak[3]\tokenbox{č}\linebreak[3]\tokenbox{en}\linebreak[3]\tokenbox{í}\linebreak[3]\tokenbox{~pro}\linebreak[3]\tokenbox{~dru}\linebreak[3]\tokenbox{h}\linebreak[3]\tokenbox{é}\linebreak[3]\tokenbox{~č}\linebreak[3]\tokenbox{}\linebreak[3]\tokenbox{ten}\linebreak[3]\tokenbox{í}\linebreak[3]\tokenbox{~pod}\linebreak[3]\tokenbox{an}\linebreak[3]\tokenbox{é}\linebreak[3]\tokenbox{~pan}\linebreak[3]\tokenbox{em}\linebreak[3]\tokenbox{~Ul}\linebreak[3]\tokenbox{ric}\linebreak[3]\tokenbox{hem}\linebreak[3]\tokenbox{~Stock}\linebreak[3]\tokenbox{mann}\linebreak[3]\tokenbox{em}\linebreak[3]\tokenbox{~j}\linebreak[3]\tokenbox{m}\linebreak[3]\tokenbox{én}\linebreak[3]\tokenbox{em}\linebreak[3]\tokenbox{~V}\linebreak[3]\tokenbox{ý}\linebreak[3]\tokenbox{}\linebreak[3]\tokenbox{bor}\linebreak[3]\tokenbox{u}\linebreak[3]\tokenbox{~pro}\linebreak[3]\tokenbox{~dop}\linebreak[3]\tokenbox{rav}\linebreak[3]\tokenbox{u}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~c}\linebreak[3]\tokenbox{est}\linebreak[3]\tokenbox{ov}\linebreak[3]\tokenbox{n}\linebreak[3]\tokenbox{í}\linebreak[3]\tokenbox{~r}\linebreak[3]\tokenbox{uch}\linebreak[3]\tokenbox{~o}\linebreak[3]\tokenbox{~let}\linebreak[3]\tokenbox{i}\linebreak[3]\tokenbox{š}\linebreak[3]\tokenbox{tn}\linebreak[3]\tokenbox{í}\linebreak[3]\tokenbox{ch}\linebreak[3]\tokenbox{~pop}\linebreak[3]\tokenbox{lat}\linebreak[3]\tokenbox{c}\linebreak[3]\tokenbox{í}\linebreak[3]\tokenbox{ch}\linebreak[3]\tokenbox{~(}\linebreak[3]\tokenbox{08}\linebreak[3]\tokenbox{332}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{2}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{2008}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~C}\linebreak[3]\tokenbox{6}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{0}\linebreak[3]\tokenbox{259}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{2008}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{Ul}\linebreak[3]\tokenbox{rich}\linebreak[3]\tokenbox{~Stock}\linebreak[3]\tokenbox{mann}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{z}\linebreak[3]\tokenbox{p}\linebreak[3]\tokenbox{rav}\linebreak[3]\tokenbox{od}\linebreak[3]\tokenbox{aj}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~(}\linebreak[3]\tokenbox{DE}\linebreak[3]\tokenbox{)}\linebreak[3]\tokenbox{~Pan}\linebreak[3]\tokenbox{í}\linebreak[3]\tokenbox{~p}\linebreak[3]\tokenbox{ř}\linebreak[3]\tokenbox{}\linebreak[3]\tokenbox{eds}\linebreak[3]\tokenbox{ed}\linebreak[3]\tokenbox{aj}\linebreak[3]\tokenbox{í}\linebreak[3]\tokenbox{c}\linebreak[3]\tokenbox{í}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~pane}\linebreak[3]\tokenbox{~k}\linebreak[3]\tokenbox{om}\linebreak[3]\tokenbox{isa}\linebreak[3]\tokenbox{ř}\linebreak[3]\tokenbox{}\linebreak[3]\tokenbox{i}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~d}\linebreak[3]\tokenbox{á}\linebreak[3]\tokenbox{my}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~p}\linebreak[3]\tokenbox{án}\linebreak[3]\tokenbox{ov}\linebreak[3]\tokenbox{é}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~po}\linebreak[3]\tokenbox{~tom}\linebreak[3]\tokenbox{to}\linebreak[3]\tokenbox{~vel}\linebreak[3]\tokenbox{mi}\linebreak[3]\tokenbox{~do}\linebreak[3]\tokenbox{j}\linebreak[3]\tokenbox{emn}\linebreak[3]\tokenbox{é}\linebreak[3]\tokenbox{m}\linebreak[3]\tokenbox{~t}\linebreak[3]\tokenbox{é}\linebreak[3]\tokenbox{mat}\linebreak[3]\tokenbox{u}\linebreak[3]\tokenbox{~se}\linebreak[3]\tokenbox{~n}\linebreak[3]\tokenbox{yn}\linebreak[3]\tokenbox{í}\linebreak[3]\tokenbox{~p}\linebreak[3]\tokenbox{ř}\linebreak[3]\tokenbox{}\linebreak[3]\tokenbox{es}\linebreak[3]\tokenbox{un}\linebreak[3]\tokenbox{eme}\linebreak[3]\tokenbox{~k}\linebreak[3]\tokenbox{~techn}\linebreak[3]\tokenbox{i}\linebreak[3]\tokenbox{č}\linebreak[3]\tokenbox{t}\linebreak[3]\tokenbox{ě}\linebreak[3]\tokenbox{}\linebreak[3]\tokenbox{j}\linebreak[3]\tokenbox{š}\linebreak[3]\tokenbox{í}\linebreak[3]\tokenbox{m}\linebreak[3]\tokenbox{~z}\linebreak[3]\tokenbox{á}\linebreak[3]\tokenbox{le}\linebreak[3]\tokenbox{ž}\linebreak[3]\tokenbox{}\linebreak[3]\tokenbox{it}\linebreak[3]\tokenbox{ost}\linebreak[3]\tokenbox{em}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~Z}\linebreak[3]\tokenbox{í}\linebreak[3]\tokenbox{tra}\linebreak[3]\tokenbox{~na}\linebreak[3]\tokenbox{~dru}\linebreak[3]\tokenbox{h}\linebreak[3]\tokenbox{é}\linebreak[3]\tokenbox{m}\linebreak[3]\tokenbox{~č}\linebreak[3]\tokenbox{}\linebreak[3]\tokenbox{ten}\linebreak[3]\tokenbox{í}\linebreak[3]\tokenbox{~ch}\linebreak[3]\tokenbox{ce}\linebreak[3]\tokenbox{me}\linebreak[3]\tokenbox{~od}\linebreak[3]\tokenbox{hl}\linebreak[3]\tokenbox{as}\linebreak[3]\tokenbox{ov}\linebreak[3]\tokenbox{at}\linebreak[3]\tokenbox{~sm}\linebreak[3]\tokenbox{ě}\linebreak[3]\tokenbox{}\linebreak[3]\tokenbox{r}\linebreak[3]\tokenbox{nic}\linebreak[3]\tokenbox{i}\linebreak[3]\tokenbox{~o}\linebreak[3]\tokenbox{~let}\linebreak[3]\tokenbox{i}\linebreak[3]\tokenbox{š}\linebreak[3]\tokenbox{tn}\linebreak[3]\tokenbox{í}\linebreak[3]\tokenbox{ch}\linebreak[3]\tokenbox{~pop}\linebreak[3]\tokenbox{lat}\linebreak[3]\tokenbox{c}\linebreak[3]\tokenbox{í}\linebreak[3]\tokenbox{ch}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~po}\linebreak[3]\tokenbox{~j}\linebreak[3]\tokenbox{ed}\linebreak[3]\tokenbox{no}\linebreak[3]\tokenbox{z}\linebreak[3]\tokenbox{na}\linebreak[3]\tokenbox{č}\linebreak[3]\tokenbox{n}\linebreak[3]\tokenbox{é}\linebreak[3]\tokenbox{m}\linebreak[3]\tokenbox{~v}\linebreak[3]\tokenbox{ý}\linebreak[3]\tokenbox{}\linebreak[3]\tokenbox{s}\linebreak[3]\tokenbox{led}\linebreak[3]\tokenbox{ku}\linebreak[3]\tokenbox{~h}\linebreak[3]\tokenbox{las}\linebreak[3]\tokenbox{ov}\linebreak[3]\tokenbox{án}\linebreak[3]\tokenbox{í}\linebreak[3]\tokenbox{~ve}\linebreak[3]\tokenbox{~V}\linebreak[3]\tokenbox{ý}\linebreak[3]\tokenbox{}\linebreak[3]\tokenbox{bor}\linebreak[3]\tokenbox{u}\linebreak[3]\tokenbox{~pro}\linebreak[3]\tokenbox{~dop}\linebreak[3]\tokenbox{rav}\linebreak[3]\tokenbox{u}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~c}\linebreak[3]\tokenbox{est}\linebreak[3]\tokenbox{ov}\linebreak[3]\tokenbox{n}\linebreak[3]\tokenbox{í}\linebreak[3]\tokenbox{~r}\linebreak[3]\tokenbox{uch}\linebreak[3]\tokenbox{~j}\linebreak[3]\tokenbox{sem}\linebreak[3]\tokenbox{~si}\linebreak[3]\tokenbox{~j}\linebreak[3]\tokenbox{ist}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~ž}\linebreak[3]\tokenbox{}\linebreak[3]\tokenbox{e}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{ho}\linebreak[3]\tokenbox{~bud}\linebreak[3]\tokenbox{eme}\linebreak[3]\tokenbox{~t}\linebreak[3]\tokenbox{ak}\linebreak[3]\tokenbox{é}\linebreak[3]\tokenbox{~sch}\linebreak[3]\tokenbox{op}\linebreak[3]\tokenbox{ni}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{Č}\linebreak[3]\tokenbox{}\linebreak[3]\tokenbox{í}\linebreak[3]\tokenbox{m}\linebreak[3]\tokenbox{~se}\linebreak[3]\tokenbox{~t}\linebreak[3]\tokenbox{ato}\linebreak[3]\tokenbox{~sm}\linebreak[3]\tokenbox{ě}\linebreak[3]\tokenbox{}\linebreak[3]\tokenbox{rn}\linebreak[3]\tokenbox{ice}\linebreak[3]\tokenbox{~z}\linebreak[3]\tokenbox{ab}\linebreak[3]\tokenbox{ý}\linebreak[3]\tokenbox{}\linebreak[3]\tokenbox{v}\linebreak[3]\tokenbox{á}\linebreak[3]\tokenbox{?}\linebreak[3]\tokenbox{~Z}\linebreak[3]\tokenbox{av}\linebreak[3]\tokenbox{á}\linebreak[3]\tokenbox{d}\linebreak[3]\tokenbox{í}\linebreak[3]\tokenbox{~j}\linebreak[3]\tokenbox{ed}\linebreak[3]\tokenbox{not}\linebreak[3]\tokenbox{n}\linebreak[3]\tokenbox{é}\linebreak[3]\tokenbox{~z}\linebreak[3]\tokenbox{ás}\linebreak[3]\tokenbox{ady}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~post}\linebreak[3]\tokenbox{up}\linebreak[3]\tokenbox{y}\linebreak[3]\tokenbox{~v}\linebreak[3]\tokenbox{y}\linebreak[3]\tokenbox{b}\linebreak[3]\tokenbox{í}\linebreak[3]\tokenbox{r}\linebreak[3]\tokenbox{án}\linebreak[3]\tokenbox{í}\linebreak[3]\tokenbox{~let}\linebreak[3]\tokenbox{i}\linebreak[3]\tokenbox{š}\linebreak[3]\tokenbox{tn}\linebreak[3]\tokenbox{í}\linebreak[3]\tokenbox{ch}\linebreak[3]\tokenbox{~pop}\linebreak[3]\tokenbox{lat}\linebreak[3]\tokenbox{k}\linebreak[3]\tokenbox{ů}\linebreak[3]\tokenbox{}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~plat}\linebreak[3]\tokenbox{n}\linebreak[3]\tokenbox{é}\linebreak[3]\tokenbox{~pro}\linebreak[3]\tokenbox{~cel}\linebreak[3]\tokenbox{ou}\linebreak[3]\tokenbox{~Ev}\linebreak[3]\tokenbox{rop}\linebreak[3]\tokenbox{u}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~To}\linebreak[3]\tokenbox{~z}\linebreak[3]\tokenbox{nam}\linebreak[3]\tokenbox{en}\linebreak[3]\tokenbox{á}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~ž}\linebreak[3]\tokenbox{}\linebreak[3]\tokenbox{e}\linebreak[3]\tokenbox{~se}\linebreak[3]\tokenbox{~j}\linebreak[3]\tokenbox{ed}\linebreak[3]\tokenbox{n}\linebreak[3]\tokenbox{á}\linebreak[3]\tokenbox{~o}\linebreak[3]\tokenbox{~transparent}\linebreak[3]\tokenbox{n}\linebreak[3]\tokenbox{í}\linebreak[3]\tokenbox{~v}\linebreak[3]\tokenbox{ý}\linebreak[3]\tokenbox{}\linebreak[3]\tokenbox{ch}\linebreak[3]\tokenbox{od}\linebreak[3]\tokenbox{isk}\linebreak[3]\tokenbox{a}\linebreak[3]\tokenbox{~pro}\linebreak[3]\tokenbox{~v}\linebreak[3]\tokenbox{ý}\linebreak[3]\tokenbox{}\linebreak[3]\tokenbox{po}\linebreak[3]\tokenbox{č}\linebreak[3]\tokenbox{et}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~n}\linebreak[3]\tokenbox{ed}\linebreak[3]\tokenbox{isk}\linebreak[3]\tokenbox{rim}\linebreak[3]\tokenbox{in}\linebreak[3]\tokenbox{aci}\linebreak[3]\tokenbox{~le}\linebreak[3]\tokenbox{te}\linebreak[3]\tokenbox{ck}\linebreak[3]\tokenbox{ý}\linebreak[3]\tokenbox{}\linebreak[3]\tokenbox{ch}\linebreak[3]\tokenbox{~sp}\linebreak[3]\tokenbox{ole}\linebreak[3]\tokenbox{č}\linebreak[3]\tokenbox{n}\linebreak[3]\tokenbox{ost}\linebreak[3]\tokenbox{í}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~ur}\linebreak[3]\tokenbox{č}\linebreak[3]\tokenbox{en}\linebreak[3]\tokenbox{ý}\linebreak[3]\tokenbox{}\linebreak[3]\tokenbox{~post}\linebreak[3]\tokenbox{up}\linebreak[3]\tokenbox{~k}\linebreak[3]\tokenbox{onz}\linebreak[3]\tokenbox{ult}\linebreak[3]\tokenbox{ace}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~sl}\linebreak[3]\tokenbox{ou}\linebreak[3]\tokenbox{ž}\linebreak[3]\tokenbox{}\linebreak[3]\tokenbox{í}\linebreak[3]\tokenbox{c}\linebreak[3]\tokenbox{í}\linebreak[3]\tokenbox{~j}\linebreak[3]\tokenbox{ako}\linebreak[3]\tokenbox{~f}\linebreak[3]\tokenbox{ak}\linebreak[3]\tokenbox{t}\linebreak[3]\tokenbox{ory}\linebreak[3]\tokenbox{~p}\linebreak[3]\tokenbox{ou}\linebreak[3]\tokenbox{ž}\linebreak[3]\tokenbox{}\linebreak[3]\tokenbox{ité}\linebreak[3]\tokenbox{~sp}\linebreak[3]\tokenbox{ol}\linebreak[3]\tokenbox{u}\linebreak[3]\tokenbox{~s}\linebreak[3]\tokenbox{~n}\linebreak[3]\tokenbox{ě}\linebreak[3]\tokenbox{}\linebreak[3]\tokenbox{k}\linebreak[3]\tokenbox{ter}\linebreak[3]\tokenbox{ý}\linebreak[3]\tokenbox{}\linebreak[3]\tokenbox{mi}\linebreak[3]\tokenbox{~d}\linebreak[3]\tokenbox{al}\linebreak[3]\tokenbox{š}\linebreak[3]\tokenbox{í}\linebreak[3]\tokenbox{mi}\linebreak[3]\tokenbox{~ke}\linebreak[3]\tokenbox{~st}\linebreak[3]\tokenbox{ano}\linebreak[3]\tokenbox{ven}\linebreak[3]\tokenbox{í}\linebreak[3]\tokenbox{~sp}\linebreak[3]\tokenbox{raved}\linebreak[3]\tokenbox{liv}\linebreak[3]\tokenbox{ý}\linebreak[3]\tokenbox{}\linebreak[3]\tokenbox{ch}\linebreak[3]\tokenbox{~let}\linebreak[3]\tokenbox{i}\linebreak[3]\tokenbox{š}\linebreak[3]\tokenbox{tn}\linebreak[3]\tokenbox{í}\linebreak[3]\tokenbox{ch}\linebreak[3]\tokenbox{~pop}\linebreak[3]\tokenbox{lat}\linebreak[3]\tokenbox{k}\linebreak[3]\tokenbox{ů}\linebreak[3]\tokenbox{}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~Kon}\linebreak[3]\tokenbox{fl}\linebreak[3]\tokenbox{ik}\linebreak[3]\tokenbox{ty}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~k}\linebreak[3]\tokenbox{ter}\linebreak[3]\tokenbox{é}\linebreak[3]\tokenbox{~v}\linebreak[3]\tokenbox{z}\linebreak[3]\tokenbox{nik}\linebreak[3]\tokenbox{ly}\linebreak[3]\tokenbox{~na}\linebreak[3]\tokenbox{~z}\linebreak[3]\tokenbox{á}\linebreak[3]\tokenbox{k}\linebreak[3]\tokenbox{lad}\linebreak[3]\tokenbox{ě}\linebreak[3]\tokenbox{}\linebreak[3]\tokenbox{~t}\linebreak[3]\tokenbox{ě}\linebreak[3]\tokenbox{}\linebreak[3]\tokenbox{ch}\linebreak[3]\tokenbox{to}\linebreak[3]\tokenbox{~j}\linebreak[3]\tokenbox{as}\linebreak[3]\tokenbox{n}\linebreak[3]\tokenbox{ý}\linebreak[3]\tokenbox{}\linebreak[3]\tokenbox{ch}\linebreak[3]\tokenbox{~p}\linebreak[3]\tokenbox{rav}\linebreak[3]\tokenbox{idel}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~m}\linebreak[3]\tokenbox{ů}\linebreak[3]\tokenbox{}\linebreak[3]\tokenbox{ž}\linebreak[3]\tokenbox{}\linebreak[3]\tokenbox{e}\linebreak[3]\tokenbox{~ř}\linebreak[3]\tokenbox{}\linebreak[3]\tokenbox{e}\linebreak[3]\tokenbox{š}\linebreak[3]\tokenbox{it}\linebreak[3]\tokenbox{~ne}\linebreak[3]\tokenbox{z}\linebreak[3]\tokenbox{á}\linebreak[3]\tokenbox{v}\linebreak[3]\tokenbox{isl}\linebreak[3]\tokenbox{ý}\linebreak[3]\tokenbox{}\linebreak[3]\tokenbox{~d}\linebreak[3]
}
\end{tokenized}
\end{minipage}
\vskip1.5em
\begin{minipage}{\textwidth}
\subcaption*{{\model{} Tokenization}}
\small\vspace{-0.5\baselineskip}\centering{457 tokens}
\begin{tokenized}
\parbox{\linewidth}{\small
\tokenbox{Let}\linebreak[3]\tokenbox{i}\linebreak[3]\tokenbox{š}\linebreak[3]\tokenbox{tn}\linebreak[3]\tokenbox{í}\linebreak[3]\tokenbox{~pop}\linebreak[3]\tokenbox{lat}\linebreak[3]\tokenbox{ky}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{P}\linebreak[3]\tokenbox{ř}\linebreak[3]\tokenbox{eds}\linebreak[3]\tokenbox{ed}\linebreak[3]\tokenbox{aj}\linebreak[3]\tokenbox{íc}\linebreak[3]\tokenbox{í}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{D}\linebreak[3]\tokenbox{al}\linebreak[3]\tokenbox{ší}\linebreak[3]\tokenbox{~bod}\linebreak[3]\tokenbox{em}\linebreak[3]\tokenbox{~jed}\linebreak[3]\tokenbox{n}\linebreak[3]\tokenbox{án}\linebreak[3]\tokenbox{í}\linebreak[3]\tokenbox{~je}\linebreak[3]\tokenbox{~dop}\linebreak[3]\tokenbox{or}\linebreak[3]\tokenbox{u}\linebreak[3]\tokenbox{č}\linebreak[3]\tokenbox{ení}\linebreak[3]\tokenbox{~pro}\linebreak[3]\tokenbox{~dru}\linebreak[3]\tokenbox{h}\linebreak[3]\tokenbox{é}\linebreak[3]\tokenbox{~č}\linebreak[3]\tokenbox{ten}\linebreak[3]\tokenbox{í}\linebreak[3]\tokenbox{~pod}\linebreak[3]\tokenbox{an}\linebreak[3]\tokenbox{é}\linebreak[3]\tokenbox{~pan}\linebreak[3]\tokenbox{em}\linebreak[3]\tokenbox{~Ul}\linebreak[3]\tokenbox{ric}\linebreak[3]\tokenbox{hem}\linebreak[3]\tokenbox{~Stock}\linebreak[3]\tokenbox{mann}\linebreak[3]\tokenbox{em}\linebreak[3]\tokenbox{~j}\linebreak[3]\tokenbox{m}\linebreak[3]\tokenbox{én}\linebreak[3]\tokenbox{em}\linebreak[3]\tokenbox{~V}\linebreak[3]\tokenbox{ý}\linebreak[3]\tokenbox{bor}\linebreak[3]\tokenbox{u}\linebreak[3]\tokenbox{~pro}\linebreak[3]\tokenbox{~dop}\linebreak[3]\tokenbox{rav}\linebreak[3]\tokenbox{u}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~c}\linebreak[3]\tokenbox{est}\linebreak[3]\tokenbox{ov}\linebreak[3]\tokenbox{ní}\linebreak[3]\tokenbox{~r}\linebreak[3]\tokenbox{uch}\linebreak[3]\tokenbox{~o}\linebreak[3]\tokenbox{~let}\linebreak[3]\tokenbox{i}\linebreak[3]\tokenbox{š}\linebreak[3]\tokenbox{tn}\linebreak[3]\tokenbox{í}\linebreak[3]\tokenbox{ch}\linebreak[3]\tokenbox{~pop}\linebreak[3]\tokenbox{lat}\linebreak[3]\tokenbox{c}\linebreak[3]\tokenbox{í}\linebreak[3]\tokenbox{ch}\linebreak[3]\tokenbox{~(}\linebreak[3]\tokenbox{08}\linebreak[3]\tokenbox{332}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{2}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{2008}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~C}\linebreak[3]\tokenbox{6}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{025}\linebreak[3]\tokenbox{9}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{2008}\linebreak[3]\tokenbox{~-.}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{Ul}\linebreak[3]\tokenbox{rich}\linebreak[3]\tokenbox{~Stock}\linebreak[3]\tokenbox{mann}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{z}\linebreak[3]\tokenbox{p}\linebreak[3]\tokenbox{rav}\linebreak[3]\tokenbox{od}\linebreak[3]\tokenbox{aj}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~(}\linebreak[3]\tokenbox{DE}\linebreak[3]\tokenbox{)}\linebreak[3]\tokenbox{~Pan}\linebreak[3]\tokenbox{í}\linebreak[3]\tokenbox{~př}\linebreak[3]\tokenbox{eds}\linebreak[3]\tokenbox{ed}\linebreak[3]\tokenbox{aj}\linebreak[3]\tokenbox{íc}\linebreak[3]\tokenbox{í}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~pane}\linebreak[3]\tokenbox{~kom}\linebreak[3]\tokenbox{isa}\linebreak[3]\tokenbox{ř}\linebreak[3]\tokenbox{i}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~d}\linebreak[3]\tokenbox{á}\linebreak[3]\tokenbox{my}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~p}\linebreak[3]\tokenbox{án}\linebreak[3]\tokenbox{ov}\linebreak[3]\tokenbox{é}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~po}\linebreak[3]\tokenbox{~tom}\linebreak[3]\tokenbox{to}\linebreak[3]\tokenbox{~vel}\linebreak[3]\tokenbox{mi}\linebreak[3]\tokenbox{~do}\linebreak[3]\tokenbox{j}\linebreak[3]\tokenbox{emn}\linebreak[3]\tokenbox{ém}\linebreak[3]\tokenbox{~té}\linebreak[3]\tokenbox{mat}\linebreak[3]\tokenbox{u}\linebreak[3]\tokenbox{~se}\linebreak[3]\tokenbox{~n}\linebreak[3]\tokenbox{yn}\linebreak[3]\tokenbox{í}\linebreak[3]\tokenbox{~př}\linebreak[3]\tokenbox{es}\linebreak[3]\tokenbox{un}\linebreak[3]\tokenbox{eme}\linebreak[3]\tokenbox{~k}\linebreak[3]\tokenbox{~techn}\linebreak[3]\tokenbox{i}\linebreak[3]\tokenbox{č}\linebreak[3]\tokenbox{t}\linebreak[3]\tokenbox{ě}\linebreak[3]\tokenbox{j}\linebreak[3]\tokenbox{š}\linebreak[3]\tokenbox{ím}\linebreak[3]\tokenbox{~z}\linebreak[3]\tokenbox{á}\linebreak[3]\tokenbox{le}\linebreak[3]\tokenbox{ž}\linebreak[3]\tokenbox{it}\linebreak[3]\tokenbox{ost}\linebreak[3]\tokenbox{em}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~Z}\linebreak[3]\tokenbox{í}\linebreak[3]\tokenbox{tra}\linebreak[3]\tokenbox{~na}\linebreak[3]\tokenbox{~dru}\linebreak[3]\tokenbox{h}\linebreak[3]\tokenbox{ém}\linebreak[3]\tokenbox{~č}\linebreak[3]\tokenbox{ten}\linebreak[3]\tokenbox{í}\linebreak[3]\tokenbox{~ch}\linebreak[3]\tokenbox{ce}\linebreak[3]\tokenbox{me}\linebreak[3]\tokenbox{~od}\linebreak[3]\tokenbox{h}\linebreak[3]\tokenbox{las}\linebreak[3]\tokenbox{ov}\linebreak[3]\tokenbox{at}\linebreak[3]\tokenbox{~sm}\linebreak[3]\tokenbox{ě}\linebreak[3]\tokenbox{r}\linebreak[3]\tokenbox{nic}\linebreak[3]\tokenbox{i}\linebreak[3]\tokenbox{~o}\linebreak[3]\tokenbox{~let}\linebreak[3]\tokenbox{i}\linebreak[3]\tokenbox{š}\linebreak[3]\tokenbox{tn}\linebreak[3]\tokenbox{í}\linebreak[3]\tokenbox{ch}\linebreak[3]\tokenbox{~pop}\linebreak[3]\tokenbox{lat}\linebreak[3]\tokenbox{c}\linebreak[3]\tokenbox{í}\linebreak[3]\tokenbox{ch}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~po}\linebreak[3]\tokenbox{~jed}\linebreak[3]\tokenbox{no}\linebreak[3]\tokenbox{z}\linebreak[3]\tokenbox{na}\linebreak[3]\tokenbox{č}\linebreak[3]\tokenbox{n}\linebreak[3]\tokenbox{ém}\linebreak[3]\tokenbox{~vý}\linebreak[3]\tokenbox{s}\linebreak[3]\tokenbox{led}\linebreak[3]\tokenbox{ku}\linebreak[3]\tokenbox{~h}\linebreak[3]\tokenbox{las}\linebreak[3]\tokenbox{ov}\linebreak[3]\tokenbox{án}\linebreak[3]\tokenbox{í}\linebreak[3]\tokenbox{~ve}\linebreak[3]\tokenbox{~V}\linebreak[3]\tokenbox{ý}\linebreak[3]\tokenbox{bor}\linebreak[3]\tokenbox{u}\linebreak[3]\tokenbox{~pro}\linebreak[3]\tokenbox{~dop}\linebreak[3]\tokenbox{rav}\linebreak[3]\tokenbox{u}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~c}\linebreak[3]\tokenbox{est}\linebreak[3]\tokenbox{ov}\linebreak[3]\tokenbox{ní}\linebreak[3]\tokenbox{~r}\linebreak[3]\tokenbox{uch}\linebreak[3]\tokenbox{~j}\linebreak[3]\tokenbox{sem}\linebreak[3]\tokenbox{~si}\linebreak[3]\tokenbox{~j}\linebreak[3]\tokenbox{ist}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~že}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{ho}\linebreak[3]\tokenbox{~bud}\linebreak[3]\tokenbox{eme}\linebreak[3]\tokenbox{~tak}\linebreak[3]\tokenbox{é}\linebreak[3]\tokenbox{~sch}\linebreak[3]\tokenbox{op}\linebreak[3]\tokenbox{ni}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{Č}\linebreak[3]\tokenbox{}\linebreak[3]\tokenbox{ím}\linebreak[3]\tokenbox{~se}\linebreak[3]\tokenbox{~t}\linebreak[3]\tokenbox{ato}\linebreak[3]\tokenbox{~sm}\linebreak[3]\tokenbox{ě}\linebreak[3]\tokenbox{rn}\linebreak[3]\tokenbox{ice}\linebreak[3]\tokenbox{~z}\linebreak[3]\tokenbox{ab}\linebreak[3]\tokenbox{ý}\linebreak[3]\tokenbox{v}\linebreak[3]\tokenbox{á}\linebreak[3]\tokenbox{?}\linebreak[3]\tokenbox{~Z}\linebreak[3]\tokenbox{av}\linebreak[3]\tokenbox{ád}\linebreak[3]\tokenbox{í}\linebreak[3]\tokenbox{~jed}\linebreak[3]\tokenbox{not}\linebreak[3]\tokenbox{né}\linebreak[3]\tokenbox{~z}\linebreak[3]\tokenbox{ás}\linebreak[3]\tokenbox{ady}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~post}\linebreak[3]\tokenbox{up}\linebreak[3]\tokenbox{y}\linebreak[3]\tokenbox{~vy}\linebreak[3]\tokenbox{b}\linebreak[3]\tokenbox{í}\linebreak[3]\tokenbox{r}\linebreak[3]\tokenbox{án}\linebreak[3]\tokenbox{í}\linebreak[3]\tokenbox{~let}\linebreak[3]\tokenbox{i}\linebreak[3]\tokenbox{š}\linebreak[3]\tokenbox{tn}\linebreak[3]\tokenbox{í}\linebreak[3]\tokenbox{ch}\linebreak[3]\tokenbox{~pop}\linebreak[3]\tokenbox{lat}\linebreak[3]\tokenbox{k}\linebreak[3]\tokenbox{ů}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~plat}\linebreak[3]\tokenbox{né}\linebreak[3]\tokenbox{~pro}\linebreak[3]\tokenbox{~cel}\linebreak[3]\tokenbox{ou}\linebreak[3]\tokenbox{~Ev}\linebreak[3]\tokenbox{rop}\linebreak[3]\tokenbox{u}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~To}\linebreak[3]\tokenbox{~z}\linebreak[3]\tokenbox{nam}\linebreak[3]\tokenbox{en}\linebreak[3]\tokenbox{á}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~že}\linebreak[3]\tokenbox{~se}\linebreak[3]\tokenbox{~jed}\linebreak[3]\tokenbox{n}\linebreak[3]\tokenbox{á}\linebreak[3]\tokenbox{~o}\linebreak[3]\tokenbox{~transparent}\linebreak[3]\tokenbox{ní}\linebreak[3]\tokenbox{~v}\linebreak[3]\tokenbox{ých}\linebreak[3]\tokenbox{od}\linebreak[3]\tokenbox{iska}\linebreak[3]\tokenbox{~pro}\linebreak[3]\tokenbox{~vý}\linebreak[3]\tokenbox{po}\linebreak[3]\tokenbox{č}\linebreak[3]\tokenbox{et}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~ned}\linebreak[3]\tokenbox{isk}\linebreak[3]\tokenbox{rimin}\linebreak[3]\tokenbox{aci}\linebreak[3]\tokenbox{~le}\linebreak[3]\tokenbox{te}\linebreak[3]\tokenbox{ck}\linebreak[3]\tokenbox{ých}\linebreak[3]\tokenbox{~sp}\linebreak[3]\tokenbox{ole}\linebreak[3]\tokenbox{č}\linebreak[3]\tokenbox{nost}\linebreak[3]\tokenbox{í}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~ur}\linebreak[3]\tokenbox{č}\linebreak[3]\tokenbox{en}\linebreak[3]\tokenbox{ý}\linebreak[3]\tokenbox{~post}\linebreak[3]\tokenbox{up}\linebreak[3]\tokenbox{~k}\linebreak[3]\tokenbox{onz}\linebreak[3]\tokenbox{ult}\linebreak[3]\tokenbox{ace}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~sl}\linebreak[3]\tokenbox{ou}\linebreak[3]\tokenbox{ž}\linebreak[3]\tokenbox{íc}\linebreak[3]\tokenbox{í}\linebreak[3]\tokenbox{~j}\linebreak[3]\tokenbox{ako}\linebreak[3]\tokenbox{~f}\linebreak[3]\tokenbox{akt}\linebreak[3]\tokenbox{ory}\linebreak[3]\tokenbox{~pou}\linebreak[3]\tokenbox{ž}\linebreak[3]\tokenbox{ité}\linebreak[3]\tokenbox{~sp}\linebreak[3]\tokenbox{olu}\linebreak[3]\tokenbox{~s}\linebreak[3]\tokenbox{~n}\linebreak[3]\tokenbox{ě}\linebreak[3]\tokenbox{k}\linebreak[3]\tokenbox{ter}\linebreak[3]\tokenbox{ý}\linebreak[3]\tokenbox{mi}\linebreak[3]\tokenbox{~dal}\linebreak[3]\tokenbox{ší}\linebreak[3]\tokenbox{mi}\linebreak[3]\tokenbox{~ke}\linebreak[3]\tokenbox{~st}\linebreak[3]\tokenbox{an}\linebreak[3]\tokenbox{oven}\linebreak[3]\tokenbox{í}\linebreak[3]\tokenbox{~sp}\linebreak[3]\tokenbox{ra}\linebreak[3]\tokenbox{ved}\linebreak[3]\tokenbox{liv}\linebreak[3]\tokenbox{ých}\linebreak[3]\tokenbox{~let}\linebreak[3]\tokenbox{i}\linebreak[3]\tokenbox{š}\linebreak[3]\tokenbox{tn}\linebreak[3]\tokenbox{í}\linebreak[3]\tokenbox{ch}\linebreak[3]\tokenbox{~pop}\linebreak[3]\tokenbox{lat}\linebreak[3]\tokenbox{k}\linebreak[3]\tokenbox{ů}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~Kon}\linebreak[3]\tokenbox{f}\linebreak[3]\tokenbox{lik}\linebreak[3]\tokenbox{ty}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~k}\linebreak[3]\tokenbox{ter}\linebreak[3]\tokenbox{é}\linebreak[3]\tokenbox{~v}\linebreak[3]\tokenbox{z}\linebreak[3]\tokenbox{nik}\linebreak[3]\tokenbox{ly}\linebreak[3]\tokenbox{~na}\linebreak[3]\tokenbox{~z}\linebreak[3]\tokenbox{á}\linebreak[3]\tokenbox{kl}\linebreak[3]\tokenbox{ad}\linebreak[3]\tokenbox{ě}\linebreak[3]\tokenbox{~t}\linebreak[3]\tokenbox{ě}\linebreak[3]\tokenbox{ch}\linebreak[3]\tokenbox{to}\linebreak[3]\tokenbox{~j}\linebreak[3]\tokenbox{as}\linebreak[3]\tokenbox{n}\linebreak[3]\tokenbox{ých}\linebreak[3]\tokenbox{~p}\linebreak[3]\tokenbox{rav}\linebreak[3]\tokenbox{idel}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~m}\linebreak[3]\tokenbox{ů}\linebreak[3]\tokenbox{že}\linebreak[3]\tokenbox{~ř}\linebreak[3]\tokenbox{}\linebreak[3]\tokenbox{e}\linebreak[3]\tokenbox{š}\linebreak[3]\tokenbox{it}\linebreak[3]\tokenbox{~ne}\linebreak[3]\tokenbox{z}\linebreak[3]\tokenbox{á}\linebreak[3]\tokenbox{vis}\linebreak[3]\tokenbox{l}\linebreak[3]\tokenbox{ý}\linebreak[3]\tokenbox{~d}\linebreak[3]
}
\end{tokenized}
\end{minipage}

==> Figures/tokenization/examples_new/FreeLaw.tex <==
\begin{minipage}{\textwidth}
\subcaption*{{GPT-2 Tokenization}}
\small\vspace{-0.5\baselineskip}\centering{252 tokens}
\begin{tokenized}
\parbox{\linewidth}{\small
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{274}\linebreak[3]\tokenbox{~Kan}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~9}\linebreak[3]\tokenbox{39}\linebreak[3]\tokenbox{~(}\linebreak[3]\tokenbox{2002}\linebreak[3]\tokenbox{)}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{58}\linebreak[3]\tokenbox{~P}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{3}\linebreak[3]\tokenbox{d}\linebreak[3]\tokenbox{~7}\linebreak[3]\tokenbox{16}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{STATE}\linebreak[3]\tokenbox{~OF}\linebreak[3]\tokenbox{~K}\linebreak[3]\tokenbox{ANS}\linebreak[3]\tokenbox{AS}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~App}\linebreak[3]\tokenbox{el}\linebreak[3]\tokenbox{lee}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{v}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{J}\linebreak[3]\tokenbox{AMES}\linebreak[3]\tokenbox{~Mc}\linebreak[3]\tokenbox{INT}\linebreak[3]\tokenbox{OSH}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~App}\linebreak[3]\tokenbox{ell}\linebreak[3]\tokenbox{ant}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{No}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~86}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{386}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{Sup}\linebreak[3]\tokenbox{reme}\linebreak[3]\tokenbox{~Court}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~Kansas}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{O}\linebreak[3]\tokenbox{pin}\linebreak[3]\tokenbox{ion}\linebreak[3]\tokenbox{~filed}\linebreak[3]\tokenbox{~December}\linebreak[3]\tokenbox{~6}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~2002}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{*}\linebreak[3]\tokenbox{940}\linebreak[3]\tokenbox{~Paige}\linebreak[3]\tokenbox{~A}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~Nichols}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~assistant}\linebreak[3]\tokenbox{~appellate}\linebreak[3]\tokenbox{~defender}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~argued}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~cause}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~Reid}\linebreak[3]\tokenbox{~T}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~Nelson}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~assistant}\linebreak[3]\tokenbox{~appellate}\linebreak[3]\tokenbox{~defender}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~Steven}\linebreak[3]\tokenbox{~R}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~Z}\linebreak[3]\tokenbox{inn}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~deputy}\linebreak[3]\tokenbox{~appellate}\linebreak[3]\tokenbox{~defender}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~Jessica}\linebreak[3]\tokenbox{~R}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~Kun}\linebreak[3]\tokenbox{en}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~chief}\linebreak[3]\tokenbox{~appellate}\linebreak[3]\tokenbox{~defender}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~were}\linebreak[3]\tokenbox{~with}\linebreak[3]\tokenbox{~her}\linebreak[3]\tokenbox{~on}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~briefs}\linebreak[3]\tokenbox{~for}\linebreak[3]\tokenbox{~appellant}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{Keith}\linebreak[3]\tokenbox{~E}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~Schro}\linebreak[3]\tokenbox{eder}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~district}\linebreak[3]\tokenbox{~attorney}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~argued}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~cause}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~Thomas}\linebreak[3]\tokenbox{~R}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~Stanton}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~deputy}\linebreak[3]\tokenbox{~district}\linebreak[3]\tokenbox{~attorney}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~Car}\linebreak[3]\tokenbox{la}\linebreak[3]\tokenbox{~J}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~St}\linebreak[3]\tokenbox{ov}\linebreak[3]\tokenbox{all}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~attorney}\linebreak[3]\tokenbox{~general}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~were}\linebreak[3]\tokenbox{~with}\linebreak[3]\tokenbox{~him}\linebreak[3]\tokenbox{~on}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~briefs}\linebreak[3]\tokenbox{~for}\linebreak[3]\tokenbox{~app}\linebreak[3]\tokenbox{el}\linebreak[3]\tokenbox{lee}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{The}\linebreak[3]\tokenbox{~opinion}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~court}\linebreak[3]\tokenbox{~was}\linebreak[3]\tokenbox{~delivered}\linebreak[3]\tokenbox{~by}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{LOCK}\linebreak[3]\tokenbox{ET}\linebreak[3]\tokenbox{T}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~J}\linebreak[3]\tokenbox{.:}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{Def}\linebreak[3]\tokenbox{endant}\linebreak[3]\tokenbox{~petitions}\linebreak[3]\tokenbox{~for}\linebreak[3]\tokenbox{~review}\linebreak[3]\tokenbox{~from}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~Court}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~Appeals}\linebreak[3]\tokenbox{'}\linebreak[3]\tokenbox{~affirm}\linebreak[3]\tokenbox{ance}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~his}\linebreak[3]\tokenbox{~convictions}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~rape}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~aggravated}\linebreak[3]\tokenbox{~indecent}\linebreak[3]\tokenbox{~liberties}\linebreak[3]\tokenbox{~with}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~child}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~two}\linebreak[3]\tokenbox{~counts}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~aggravated}\linebreak[3]\tokenbox{~criminal}\linebreak[3]\tokenbox{~sod}\linebreak[3]\tokenbox{omy}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~his}\linebreak[3]\tokenbox{~sentence}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~316}\linebreak[3]\tokenbox{~months}\linebreak[3]\tokenbox{'}\linebreak[3]\tokenbox{~imprisonment}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~Defendant}\linebreak[3]\tokenbox{~claims}\linebreak[3]\tokenbox{~(}\linebreak[3]\tokenbox{1}\linebreak[3]\tokenbox{)}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~trial}\linebreak[3]\tokenbox{~court}\linebreak[3]\tokenbox{~er}\linebreak[3]\tokenbox{red}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~finding}\linebreak[3]\tokenbox{~that}\linebreak[3]\tokenbox{~he}\linebreak[3]\tokenbox{~failed}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~establish}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~compelling}\linebreak[3]\tokenbox{~reason}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~requ}\linebreak[3]\tokenbox{ir}\linebreak[3]
}
\end{tokenized}
\end{minipage}
\vskip1.5em
\begin{minipage}{\textwidth}
\subcaption*{{\model{} Tokenization}}
\small\vspace{-0.5\baselineskip}\centering{248 tokens}
\begin{tokenized}
\parbox{\linewidth}{\small
\tokenbox{}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{274}\linebreak[3]\tokenbox{~Kan}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~9}\linebreak[3]\tokenbox{39}\linebreak[3]\tokenbox{~(}\linebreak[3]\tokenbox{2002}\linebreak[3]\tokenbox{)}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{58}\linebreak[3]\tokenbox{~P}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{3}\linebreak[3]\tokenbox{d}\linebreak[3]\tokenbox{~7}\linebreak[3]\tokenbox{16}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{STATE}\linebreak[3]\tokenbox{~OF}\linebreak[3]\tokenbox{~K}\linebreak[3]\tokenbox{ANS}\linebreak[3]\tokenbox{AS}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~Appellee}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{v}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{J}\linebreak[3]\tokenbox{AMES}\linebreak[3]\tokenbox{~Mc}\linebreak[3]\tokenbox{INT}\linebreak[3]\tokenbox{OS}\linebreak[3]\tokenbox{H}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~Appellant}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{No}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~86}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{386}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{Supreme}\linebreak[3]\tokenbox{~Court}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~Kansas}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{O}\linebreak[3]\tokenbox{pinion}\linebreak[3]\tokenbox{~filed}\linebreak[3]\tokenbox{~December}\linebreak[3]\tokenbox{~6}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~2002}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{*}\linebreak[3]\tokenbox{940}\linebreak[3]\tokenbox{~Pa}\linebreak[3]\tokenbox{ige}\linebreak[3]\tokenbox{~A}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~Nichols}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~assistant}\linebreak[3]\tokenbox{~appellate}\linebreak[3]\tokenbox{~defender}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~argued}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~cause}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~Reid}\linebreak[3]\tokenbox{~T}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~Nelson}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~assistant}\linebreak[3]\tokenbox{~appellate}\linebreak[3]\tokenbox{~defender}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~Steven}\linebreak[3]\tokenbox{~R}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~Z}\linebreak[3]\tokenbox{inn}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~deputy}\linebreak[3]\tokenbox{~appellate}\linebreak[3]\tokenbox{~defender}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~Jessica}\linebreak[3]\tokenbox{~R}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~Kun}\linebreak[3]\tokenbox{en}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~chief}\linebreak[3]\tokenbox{~appellate}\linebreak[3]\tokenbox{~defender}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~were}\linebreak[3]\tokenbox{~with}\linebreak[3]\tokenbox{~her}\linebreak[3]\tokenbox{~on}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~briefs}\linebreak[3]\tokenbox{~for}\linebreak[3]\tokenbox{~appellant}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{Ke}\linebreak[3]\tokenbox{ith}\linebreak[3]\tokenbox{~E}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~Sch}\linebreak[3]\tokenbox{ro}\linebreak[3]\tokenbox{eder}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~district}\linebreak[3]\tokenbox{~attorney}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~argued}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~cause}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~Thomas}\linebreak[3]\tokenbox{~R}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~Stanton}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~deputy}\linebreak[3]\tokenbox{~district}\linebreak[3]\tokenbox{~attorney}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~Car}\linebreak[3]\tokenbox{la}\linebreak[3]\tokenbox{~J}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~St}\linebreak[3]\tokenbox{ov}\linebreak[3]\tokenbox{all}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~attorney}\linebreak[3]\tokenbox{~general}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~were}\linebreak[3]\tokenbox{~with}\linebreak[3]\tokenbox{~him}\linebreak[3]\tokenbox{~on}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~briefs}\linebreak[3]\tokenbox{~for}\linebreak[3]\tokenbox{~appellee}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{The}\linebreak[3]\tokenbox{~opinion}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~court}\linebreak[3]\tokenbox{~was}\linebreak[3]\tokenbox{~delivered}\linebreak[3]\tokenbox{~by}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{LOCK}\linebreak[3]\tokenbox{ET}\linebreak[3]\tokenbox{T}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~J}\linebreak[3]\tokenbox{.:}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{Defendant}\linebreak[3]\tokenbox{~petitions}\linebreak[3]\tokenbox{~for}\linebreak[3]\tokenbox{~review}\linebreak[3]\tokenbox{~from}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~Court}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~Appeals}\linebreak[3]\tokenbox{'}\linebreak[3]\tokenbox{~affirm}\linebreak[3]\tokenbox{ance}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~his}\linebreak[3]\tokenbox{~convictions}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~rape}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~aggravated}\linebreak[3]\tokenbox{~inde}\linebreak[3]\tokenbox{cent}\linebreak[3]\tokenbox{~liberties}\linebreak[3]\tokenbox{~with}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~child}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~two}\linebreak[3]\tokenbox{~counts}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~aggravated}\linebreak[3]\tokenbox{~criminal}\linebreak[3]\tokenbox{~sod}\linebreak[3]\tokenbox{omy}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~his}\linebreak[3]\tokenbox{~sentence}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~316}\linebreak[3]\tokenbox{~months}\linebreak[3]\tokenbox{'}\linebreak[3]\tokenbox{~imprisonment}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~Defendant}\linebreak[3]\tokenbox{~claims}\linebreak[3]\tokenbox{~(}\linebreak[3]\tokenbox{1}\linebreak[3]\tokenbox{)}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~trial}\linebreak[3]\tokenbox{~court}\linebreak[3]\tokenbox{~erred}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~finding}\linebreak[3]\tokenbox{~that}\linebreak[3]\tokenbox{~he}\linebreak[3]\tokenbox{~failed}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~establish}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~compelling}\linebreak[3]\tokenbox{~reason}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~requ}\linebreak[3]\tokenbox{ir}\linebreak[3]
}
\end{tokenized}
\end{minipage}

==> Figures/tokenization/examples_new/Gutenberg.tex <==
\begin{minipage}{\textwidth}
\subcaption*{{GPT-2 Tokenization}}
\small\vspace{-0.5\baselineskip}\centering{250 tokens}
\begin{tokenized}
\parbox{\linewidth}{\small
\tokenbox{$\hookleftarrow$$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{Produ}\linebreak[3]\tokenbox{ced}\linebreak[3]\tokenbox{~by}\linebreak[3]\tokenbox{~Anne}\linebreak[3]\tokenbox{~Soul}\linebreak[3]\tokenbox{ard}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~Charles}\linebreak[3]\tokenbox{~Franks}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~Online}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{Dist}\linebreak[3]\tokenbox{ributed}\linebreak[3]\tokenbox{~Proof}\linebreak[3]\tokenbox{reading}\linebreak[3]\tokenbox{~Team}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{The}\linebreak[3]\tokenbox{~Treasure}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~Inc}\linebreak[3]\tokenbox{as}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{A}\linebreak[3]\tokenbox{~Story}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~Adventure}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~Peru}\linebreak[3]\tokenbox{$\hookleftarrow$$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{BY}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{G}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~A}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~H}\linebreak[3]\tokenbox{ENT}\linebreak[3]\tokenbox{Y}\linebreak[3]\tokenbox{$\hookleftarrow$$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{[}\linebreak[3]\tokenbox{Ill}\linebreak[3]\tokenbox{ustration}\linebreak[3]\tokenbox{:}\linebreak[3]\tokenbox{~IT}\linebreak[3]\tokenbox{~DID}\linebreak[3]\tokenbox{~NOT}\linebreak[3]\tokenbox{~TA}\linebreak[3]\tokenbox{KE}\linebreak[3]\tokenbox{~LONG}\linebreak[3]\tokenbox{~TO}\linebreak[3]\tokenbox{~TRANS}\linebreak[3]\tokenbox{FER}\linebreak[3]\tokenbox{~THE}\linebreak[3]\tokenbox{~S}\linebreak[3]\tokenbox{ACK}\linebreak[3]\tokenbox{S}\linebreak[3]\tokenbox{~INTO}\linebreak[3]\tokenbox{~THE}\linebreak[3]\tokenbox{~BO}\linebreak[3]\tokenbox{AT}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{\_}\linebreak[3]\tokenbox{Page}\linebreak[3]\tokenbox{~339}\linebreak[3]\tokenbox{\_}\linebreak[3]\tokenbox{]}\linebreak[3]\tokenbox{$\hookleftarrow$$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{P}\linebreak[3]\tokenbox{REF}\linebreak[3]\tokenbox{ACE}\linebreak[3]\tokenbox{~TO}\linebreak[3]\tokenbox{~THE}\linebreak[3]\tokenbox{~ORIG}\linebreak[3]\tokenbox{INAL}\linebreak[3]\tokenbox{~EDITION}\linebreak[3]\tokenbox{$\hookleftarrow$$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{The}\linebreak[3]\tokenbox{~mysterious}\linebreak[3]\tokenbox{~loss}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~large}\linebreak[3]\tokenbox{~portion}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~treasure}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~Inc}\linebreak[3]\tokenbox{as}\linebreak[3]\tokenbox{~has}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{never}\linebreak[3]\tokenbox{~been}\linebreak[3]\tokenbox{~completely}\linebreak[3]\tokenbox{~cleared}\linebreak[3]\tokenbox{~up}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~By}\linebreak[3]\tokenbox{~tort}\linebreak[3]\tokenbox{uring}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~natives}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~whom}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{secret}\linebreak[3]\tokenbox{~had}\linebreak[3]\tokenbox{~been}\linebreak[3]\tokenbox{~entrusted}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~Spani}\linebreak[3]\tokenbox{ards}\linebreak[3]\tokenbox{~made}\linebreak[3]\tokenbox{~two}\linebreak[3]\tokenbox{~or}\linebreak[3]\tokenbox{~three}\linebreak[3]\tokenbox{~discoveries}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{but}\linebreak[3]\tokenbox{~there}\linebreak[3]\tokenbox{~can}\linebreak[3]\tokenbox{~be}\linebreak[3]\tokenbox{~little}\linebreak[3]\tokenbox{~doubt}\linebreak[3]\tokenbox{~that}\linebreak[3]\tokenbox{~these}\linebreak[3]\tokenbox{~finds}\linebreak[3]\tokenbox{~were}\linebreak[3]\tokenbox{~only}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~small}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{pro}\linebreak[3]\tokenbox{portion}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~total}\linebreak[3]\tokenbox{~amount}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~missing}\linebreak[3]\tokenbox{~ho}\linebreak[3]\tokenbox{ards}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~although}\linebreak[3]\tokenbox{~for}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{years}\linebreak[3]\tokenbox{~after}\linebreak[3]\tokenbox{~their}\linebreak[3]\tokenbox{~occupation}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~country}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~Spani}\linebreak[3]\tokenbox{ards}\linebreak[3]\tokenbox{~spared}\linebreak[3]\tokenbox{~no}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{p}\linebreak[3]\tokenbox{ains}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~hesitated}\linebreak[3]\tokenbox{~at}\linebreak[3]\tokenbox{~no}\linebreak[3]\tokenbox{~cruelty}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~bring}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~light}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~hidden}\linebreak[3]\tokenbox{~wealth}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{The}\linebreak[3]\tokenbox{~story}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~boat}\linebreak[3]\tokenbox{~which}\linebreak[3]\tokenbox{~put}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~sea}\linebreak[3]\tokenbox{~lad}\linebreak[3]\tokenbox{en}\linebreak[3]\tokenbox{~with}\linebreak[3]\tokenbox{~treasure}\linebreak[3]\tokenbox{~is}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{hist}\linebreak[3]\tokenbox{orical}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~it}\linebreak[3]\tokenbox{~was}\linebreak[3]\tokenbox{~generally}\linebreak[3]\tokenbox{~supposed}\linebreak[3]\tokenbox{~that}\linebreak[3]\tokenbox{~she}\linebreak[3]\tokenbox{~was}\linebreak[3]\tokenbox{~lost}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~storm}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{that}\linebreak[3]\tokenbox{~took}\linebreak[3]\tokenbox{~place}\linebreak[3]\tokenbox{~soon}\linebreak[3]\tokenbox{~after}\linebreak[3]\tokenbox{~she}\linebreak[3]\tokenbox{~sailed}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~It}\linebreak[3]\tokenbox{~was}\linebreak[3]\tokenbox{~also}\linebreak[3]\tokenbox{~morally}\linebreak[3]\tokenbox{~certain}\linebreak[3]\tokenbox{~that}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{the}\linebreak[3]\tokenbox{~Per}\linebreak[3]\tokenbox{uv}\linebreak[3]
}
\end{tokenized}
\end{minipage}
\vskip1.5em
\begin{minipage}{\textwidth}
\subcaption*{{\model{} Tokenization}}
\small\vspace{-0.5\baselineskip}\centering{247 tokens}
\begin{tokenized}
\parbox{\linewidth}{\small
\tokenbox{}\linebreak[3]\tokenbox{$\hookleftarrow$$\hookleftarrow$$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{Pro}\linebreak[3]\tokenbox{duced}\linebreak[3]\tokenbox{~by}\linebreak[3]\tokenbox{~Anne}\linebreak[3]\tokenbox{~Soul}\linebreak[3]\tokenbox{ard}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~Charles}\linebreak[3]\tokenbox{~Fr}\linebreak[3]\tokenbox{anks}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~Online}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{Dist}\linebreak[3]\tokenbox{ributed}\linebreak[3]\tokenbox{~Proof}\linebreak[3]\tokenbox{reading}\linebreak[3]\tokenbox{~Team}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$$\hookleftarrow$$\hookleftarrow$$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$$\hookleftarrow$$\hookleftarrow$$\hookleftarrow$$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{The}\linebreak[3]\tokenbox{~Treasure}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~Inc}\linebreak[3]\tokenbox{as}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{A}\linebreak[3]\tokenbox{~Story}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~Adventure}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~Peru}\linebreak[3]\tokenbox{$\hookleftarrow$$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{BY}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{G}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~A}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~H}\linebreak[3]\tokenbox{ENT}\linebreak[3]\tokenbox{Y}\linebreak[3]\tokenbox{$\hookleftarrow$$\hookleftarrow$$\hookleftarrow$$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{[}\linebreak[3]\tokenbox{Illustration}\linebreak[3]\tokenbox{:}\linebreak[3]\tokenbox{~IT}\linebreak[3]\tokenbox{~DID}\linebreak[3]\tokenbox{~NOT}\linebreak[3]\tokenbox{~TA}\linebreak[3]\tokenbox{KE}\linebreak[3]\tokenbox{~LONG}\linebreak[3]\tokenbox{~TO}\linebreak[3]\tokenbox{~TRAN}\linebreak[3]\tokenbox{SF}\linebreak[3]\tokenbox{ER}\linebreak[3]\tokenbox{~THE}\linebreak[3]\tokenbox{~S}\linebreak[3]\tokenbox{ACK}\linebreak[3]\tokenbox{S}\linebreak[3]\tokenbox{~INTO}\linebreak[3]\tokenbox{~THE}\linebreak[3]\tokenbox{~BO}\linebreak[3]\tokenbox{AT}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{\_}\linebreak[3]\tokenbox{Page}\linebreak[3]\tokenbox{~339}\linebreak[3]\tokenbox{\_}\linebreak[3]\tokenbox{]}\linebreak[3]\tokenbox{$\hookleftarrow$$\hookleftarrow$$\hookleftarrow$$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{PRE}\linebreak[3]\tokenbox{FACE}\linebreak[3]\tokenbox{~TO}\linebreak[3]\tokenbox{~THE}\linebreak[3]\tokenbox{~OR}\linebreak[3]\tokenbox{IG}\linebreak[3]\tokenbox{IN}\linebreak[3]\tokenbox{AL}\linebreak[3]\tokenbox{~ED}\linebreak[3]\tokenbox{ITION}\linebreak[3]\tokenbox{$\hookleftarrow$$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{The}\linebreak[3]\tokenbox{~mysterious}\linebreak[3]\tokenbox{~loss}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~large}\linebreak[3]\tokenbox{~portion}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~treasure}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~Inc}\linebreak[3]\tokenbox{as}\linebreak[3]\tokenbox{~has}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{never}\linebreak[3]\tokenbox{~been}\linebreak[3]\tokenbox{~completely}\linebreak[3]\tokenbox{~cleared}\linebreak[3]\tokenbox{~up}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~By}\linebreak[3]\tokenbox{~tort}\linebreak[3]\tokenbox{uring}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~natives}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~whom}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{secret}\linebreak[3]\tokenbox{~had}\linebreak[3]\tokenbox{~been}\linebreak[3]\tokenbox{~entrusted}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~Spani}\linebreak[3]\tokenbox{ards}\linebreak[3]\tokenbox{~made}\linebreak[3]\tokenbox{~two}\linebreak[3]\tokenbox{~or}\linebreak[3]\tokenbox{~three}\linebreak[3]\tokenbox{~discoveries}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{but}\linebreak[3]\tokenbox{~there}\linebreak[3]\tokenbox{~can}\linebreak[3]\tokenbox{~be}\linebreak[3]\tokenbox{~little}\linebreak[3]\tokenbox{~doubt}\linebreak[3]\tokenbox{~that}\linebreak[3]\tokenbox{~these}\linebreak[3]\tokenbox{~finds}\linebreak[3]\tokenbox{~were}\linebreak[3]\tokenbox{~only}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~small}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{proportion}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~total}\linebreak[3]\tokenbox{~amount}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~missing}\linebreak[3]\tokenbox{~ho}\linebreak[3]\tokenbox{ards}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~although}\linebreak[3]\tokenbox{~for}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{years}\linebreak[3]\tokenbox{~after}\linebreak[3]\tokenbox{~their}\linebreak[3]\tokenbox{~occupation}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~country}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~Spani}\linebreak[3]\tokenbox{ards}\linebreak[3]\tokenbox{~spared}\linebreak[3]\tokenbox{~no}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{p}\linebreak[3]\tokenbox{ains}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~hesitated}\linebreak[3]\tokenbox{~at}\linebreak[3]\tokenbox{~no}\linebreak[3]\tokenbox{~cruelty}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~bring}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~light}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~hidden}\linebreak[3]\tokenbox{~wealth}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{The}\linebreak[3]\tokenbox{~story}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~boat}\linebreak[3]\tokenbox{~which}\linebreak[3]\tokenbox{~put}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~sea}\linebreak[3]\tokenbox{~lad}\linebreak[3]\tokenbox{en}\linebreak[3]\tokenbox{~with}\linebreak[3]\tokenbox{~treasure}\linebreak[3]\tokenbox{~is}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{histor}\linebreak[3]\tokenbox{ical}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~it}\linebreak[3]\tokenbox{~was}\linebreak[3]\tokenbox{~generally}\linebreak[3]\tokenbox{~supposed}\linebreak[3]\tokenbox{~that}\linebreak[3]\tokenbox{~she}\linebreak[3]\tokenbox{~was}\linebreak[3]\tokenbox{~lost}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~storm}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{that}\linebreak[3]\tokenbox{~took}\linebreak[3]\tokenbox{~place}\linebreak[3]\tokenbox{~soon}\linebreak[3]\tokenbox{~after}\linebreak[3]\tokenbox{~she}\linebreak[3]\tokenbox{~sailed}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~It}\linebreak[3]\tokenbox{~was}\linebreak[3]\tokenbox{~also}\linebreak[3]\tokenbox{~morally}\linebreak[3]\tokenbox{~certain}\linebreak[3]\tokenbox{~that}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{the}\linebreak[3]\tokenbox{~Per}\linebreak[3]\tokenbox{uv}\linebreak[3]
}
\end{tokenized}
\end{minipage}

==> Figures/tokenization/examples_new/HackerNews.tex <==
\begin{minipage}{\textwidth}
\subcaption*{{GPT-2 Tokenization}}
\small\vspace{-0.5\baselineskip}\centering{152 tokens}
\begin{tokenized}
\parbox{\linewidth}{\small
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{New}\linebreak[3]\tokenbox{~data}\linebreak[3]\tokenbox{~supports}\linebreak[3]\tokenbox{~finding}\linebreak[3]\tokenbox{~that}\linebreak[3]\tokenbox{~30}\linebreak[3]\tokenbox{%}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~servers}\linebreak[3]\tokenbox{~are}\linebreak[3]\tokenbox{~‘}\linebreak[3]\tokenbox{}\linebreak[3]\tokenbox{com}\linebreak[3]\tokenbox{at}\linebreak[3]\tokenbox{ose}\linebreak[3]\tokenbox{’}\linebreak[3]\tokenbox{}\linebreak[3]\tokenbox{~[}\linebreak[3]\tokenbox{pdf}\linebreak[3]\tokenbox{]}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~r}\linebreak[3]\tokenbox{7}\linebreak[3]\tokenbox{21}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{http}\linebreak[3]\tokenbox{://}\linebreak[3]\tokenbox{ant}\linebreak[3]\tokenbox{hesis}\linebreak[3]\tokenbox{group}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{com}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{wp}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{content}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{uploads}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{2015}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{06}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{Case}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{Study}\linebreak[3]\tokenbox{\_}\linebreak[3]\tokenbox{Data}\linebreak[3]\tokenbox{Supp}\linebreak[3]\tokenbox{orts}\linebreak[3]\tokenbox{30}\linebreak[3]\tokenbox{Percent}\linebreak[3]\tokenbox{Com}\linebreak[3]\tokenbox{at}\linebreak[3]\tokenbox{ose}\linebreak[3]\tokenbox{Est}\linebreak[3]\tokenbox{imate}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{F}\linebreak[3]\tokenbox{INAL}\linebreak[3]\tokenbox{\_}\linebreak[3]\tokenbox{0}\linebreak[3]\tokenbox{603}\linebreak[3]\tokenbox{2015}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{pdf}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{======}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{d}\linebreak[3]\tokenbox{ang}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{Url}\linebreak[3]\tokenbox{~changed}\linebreak[3]\tokenbox{~from}\linebreak[3]\tokenbox{~[}\linebreak[3]\tokenbox{http}\linebreak[3]\tokenbox{://}\linebreak[3]\tokenbox{www}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{computer}\linebreak[3]\tokenbox{world}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{com}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{article}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{29}\linebreak[3]\tokenbox{37}\linebreak[3]\tokenbox{408}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{data}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{center}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{1}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{i}\linebreak[3]\tokenbox{...}\linebreak[3]\tokenbox{](}\linebreak[3]\tokenbox{http}\linebreak[3]\tokenbox{://}\linebreak[3]\tokenbox{www}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{computer}\linebreak[3]\tokenbox{world}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{com}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{article}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{29}\linebreak[3]\tokenbox{37}\linebreak[3]\tokenbox{408}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{data}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{center}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{1}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{in}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{3}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{data}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{center}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{ser}\linebreak[3]\tokenbox{vers}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{is}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{a}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{z}\linebreak[3]\tokenbox{ombie}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{html}\linebreak[3]\tokenbox{),}\linebreak[3]\tokenbox{~which}\linebreak[3]\tokenbox{~points}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~this}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$$\hookleftarrow$}\newline

}
\end{tokenized}
\end{minipage}
\vskip1.5em
\begin{minipage}{\textwidth}
\subcaption*{{\model{} Tokenization}}
\small\vspace{-0.5\baselineskip}\centering{150 tokens}
\begin{tokenized}
\parbox{\linewidth}{\small
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{New}\linebreak[3]\tokenbox{~data}\linebreak[3]\tokenbox{~supports}\linebreak[3]\tokenbox{~finding}\linebreak[3]\tokenbox{~that}\linebreak[3]\tokenbox{~30}\linebreak[3]\tokenbox{%}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~servers}\linebreak[3]\tokenbox{~are}\linebreak[3]\tokenbox{~‘}\linebreak[3]\tokenbox{com}\linebreak[3]\tokenbox{at}\linebreak[3]\tokenbox{ose}\linebreak[3]\tokenbox{’}\linebreak[3]\tokenbox{~[}\linebreak[3]\tokenbox{pdf}\linebreak[3]\tokenbox{]}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~r}\linebreak[3]\tokenbox{7}\linebreak[3]\tokenbox{21}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{http}\linebreak[3]\tokenbox{://}\linebreak[3]\tokenbox{ant}\linebreak[3]\tokenbox{hesis}\linebreak[3]\tokenbox{group}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{com}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{wp}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{content}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{uploads}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{2015}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{06}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{Case}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{Study}\linebreak[3]\tokenbox{\_}\linebreak[3]\tokenbox{Data}\linebreak[3]\tokenbox{Supp}\linebreak[3]\tokenbox{orts}\linebreak[3]\tokenbox{30}\linebreak[3]\tokenbox{Percent}\linebreak[3]\tokenbox{Com}\linebreak[3]\tokenbox{at}\linebreak[3]\tokenbox{ose}\linebreak[3]\tokenbox{Est}\linebreak[3]\tokenbox{imate}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{FIN}\linebreak[3]\tokenbox{AL}\linebreak[3]\tokenbox{\_}\linebreak[3]\tokenbox{060}\linebreak[3]\tokenbox{32}\linebreak[3]\tokenbox{015}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{pdf}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{======}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{d}\linebreak[3]\tokenbox{ang}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{Url}\linebreak[3]\tokenbox{~changed}\linebreak[3]\tokenbox{~from}\linebreak[3]\tokenbox{~[}\linebreak[3]\tokenbox{http}\linebreak[3]\tokenbox{://}\linebreak[3]\tokenbox{www}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{computer}\linebreak[3]\tokenbox{world}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{com}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{article}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{29}\linebreak[3]\tokenbox{37}\linebreak[3]\tokenbox{408}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{data}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{center}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{1}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{i}\linebreak[3]\tokenbox{...](}\linebreak[3]\tokenbox{http}\linebreak[3]\tokenbox{://}\linebreak[3]\tokenbox{www}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{computer}\linebreak[3]\tokenbox{world}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{com}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{article}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{29}\linebreak[3]\tokenbox{37}\linebreak[3]\tokenbox{408}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{data}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{center}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{1}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{in}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{3}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{data}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{center}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{ser}\linebreak[3]\tokenbox{vers}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{is}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{a}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{z}\linebreak[3]\tokenbox{omb}\linebreak[3]\tokenbox{ie}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{html}\linebreak[3]\tokenbox{),}\linebreak[3]\tokenbox{~which}\linebreak[3]\tokenbox{~points}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~this}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$$\hookleftarrow$}\newline

}
\end{tokenized}
\end{minipage}

==> Figures/tokenization/examples_new/NIH_ExPorter.tex <==
\begin{minipage}{\textwidth}
\subcaption*{{GPT-2 Tokenization}}
\small\vspace{-0.5\baselineskip}\centering{228 tokens}
\begin{tokenized}
\parbox{\linewidth}{\small
\tokenbox{EX}\linebreak[3]\tokenbox{CE}\linebreak[3]\tokenbox{ED}\linebreak[3]\tokenbox{~THE}\linebreak[3]\tokenbox{~SPACE}\linebreak[3]\tokenbox{~PROV}\linebreak[3]\tokenbox{ID}\linebreak[3]\tokenbox{ED}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~The}\linebreak[3]\tokenbox{~proposed}\linebreak[3]\tokenbox{~research}\linebreak[3]\tokenbox{~is}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~continued}\linebreak[3]\tokenbox{~study}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~mobile}\linebreak[3]\tokenbox{~intr}\linebreak[3]\tokenbox{ons}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~bacteria}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~The}\linebreak[3]\tokenbox{~mobile}\linebreak[3]\tokenbox{~group}\linebreak[3]\tokenbox{~I}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~group}\linebreak[3]\tokenbox{~II}\linebreak[3]\tokenbox{~intr}\linebreak[3]\tokenbox{ons}\linebreak[3]\tokenbox{~are}\linebreak[3]\tokenbox{~both}\linebreak[3]\tokenbox{~self}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{spl}\linebreak[3]\tokenbox{icing}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~but}\linebreak[3]\tokenbox{~their}\linebreak[3]\tokenbox{~RNA}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{spl}\linebreak[3]\tokenbox{icing}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~DNA}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{mob}\linebreak[3]\tokenbox{ility}\linebreak[3]\tokenbox{~pathways}\linebreak[3]\tokenbox{~are}\linebreak[3]\tokenbox{~distinct}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~In}\linebreak[3]\tokenbox{~each}\linebreak[3]\tokenbox{~case}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~int}\linebreak[3]\tokenbox{ron}\linebreak[3]\tokenbox{~typically}\linebreak[3]\tokenbox{~transfers}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~an}\linebreak[3]\tokenbox{~alle}\linebreak[3]\tokenbox{lic}\linebreak[3]\tokenbox{~int}\linebreak[3]\tokenbox{ron}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{less}\linebreak[3]\tokenbox{~site}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~h}\linebreak[3]\tokenbox{oming}\linebreak[3]\tokenbox{process}\linebreak[3]\tokenbox{~initiated}\linebreak[3]\tokenbox{~by}\linebreak[3]\tokenbox{~int}\linebreak[3]\tokenbox{ron}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{enc}\linebreak[3]\tokenbox{oded}\linebreak[3]\tokenbox{~end}\linebreak[3]\tokenbox{on}\linebreak[3]\tokenbox{ucle}\linebreak[3]\tokenbox{ases}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~For}\linebreak[3]\tokenbox{~group}\linebreak[3]\tokenbox{~I}\linebreak[3]\tokenbox{~int}\linebreak[3]\tokenbox{ron}\linebreak[3]\tokenbox{~h}\linebreak[3]\tokenbox{oming}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~recomb}\linebreak[3]\tokenbox{ination}\linebreak[3]\tokenbox{~events}\linebreak[3]\tokenbox{~are}\linebreak[3]\tokenbox{~strictly}\linebreak[3]\tokenbox{~DNA}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{based}\linebreak[3]\tokenbox{~whereas}\linebreak[3]\tokenbox{~for}\linebreak[3]\tokenbox{~group}\linebreak[3]\tokenbox{~II}\linebreak[3]\tokenbox{~int}\linebreak[3]\tokenbox{ron}\linebreak[3]\tokenbox{~h}\linebreak[3]\tokenbox{oming}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~also}\linebreak[3]\tokenbox{~termed}\linebreak[3]\tokenbox{~retro}\linebreak[3]\tokenbox{h}\linebreak[3]\tokenbox{oming}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~RNA}\linebreak[3]\tokenbox{~is}\linebreak[3]\tokenbox{~involved}\linebreak[3]\tokenbox{~at}\linebreak[3]\tokenbox{~levels}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~both}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~int}\linebreak[3]\tokenbox{ron}\linebreak[3]\tokenbox{~template}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~cle}\linebreak[3]\tokenbox{avage}\linebreak[3]\tokenbox{~enzyme}\linebreak[3]\tokenbox{~for}\linebreak[3]\tokenbox{~mobility}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~Trans}\linebreak[3]\tokenbox{position}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~ect}\linebreak[3]\tokenbox{opic}\linebreak[3]\tokenbox{~sites}\linebreak[3]\tokenbox{~also}\linebreak[3]\tokenbox{~occurs}\linebreak[3]\tokenbox{~at}\linebreak[3]\tokenbox{~low}\linebreak[3]\tokenbox{~frequency}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~is}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~process}\linebreak[3]\tokenbox{~responsible}\linebreak[3]\tokenbox{~for}\linebreak[3]\tokenbox{~int}\linebreak[3]\tokenbox{ron}\linebreak[3]\tokenbox{~dissemination}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~nature}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~During}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~current}\linebreak[3]\tokenbox{~funding}\linebreak[3]\tokenbox{~period}\linebreak[3]\tokenbox{~we}\linebreak[3]\tokenbox{~showed}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~following}\linebreak[3]\tokenbox{:}\linebreak[3]\tokenbox{~H}\linebreak[3]\tokenbox{oming}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~group}\linebreak[3]\tokenbox{~I}\linebreak[3]\tokenbox{~td}\linebreak[3]\tokenbox{~int}\linebreak[3]\tokenbox{ron}\linebreak[3]\tokenbox{~is}\linebreak[3]\tokenbox{~regulated}\linebreak[3]\tokenbox{~by}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~very}\linebreak[3]\tokenbox{~end}\linebreak[3]\tokenbox{on}\linebreak[3]\tokenbox{uc}\linebreak[3]\tokenbox{lease}\linebreak[3]\tokenbox{~that}\linebreak[3]\tokenbox{~promotes}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~process}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~by}\linebreak[3]\tokenbox{~acting}\linebreak[3]\tokenbox{~as}\linebreak[3]\tokenbox{~an}\linebreak[3]\tokenbox{~aut}\linebreak[3]\tokenbox{ore}\linebreak[3]\tokenbox{press}\linebreak[3]\tokenbox{or}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~Also}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~retro}\linebreak[3]\tokenbox{h}\linebreak[3]\tokenbox{oming}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~group}\linebreak[3]\tokenbox{~II}\linebreak[3]\tokenbox{~intr}\linebreak[3]\tokenbox{ons}\linebreak[3]\tokenbox{~is}\linebreak[3]\tokenbox{~dependent}\linebreak[3]\tokenbox{~on}\linebreak[3]\tokenbox{~host}\linebreak[3]\tokenbox{~polymer}\linebreak[3]\tokenbox{ases}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~way}\linebreak[3]\tokenbox{~that}\linebreak[3]\tokenbox{~suggests}\linebreak[3]\tokenbox{~}\linebreak[3]
}
\end{tokenized}
\end{minipage}
\vskip1.5em
\begin{minipage}{\textwidth}
\subcaption*{{\model{} Tokenization}}
\small\vspace{-0.5\baselineskip}\centering{214 tokens}
\begin{tokenized}
\parbox{\linewidth}{\small
\tokenbox{EX}\linebreak[3]\tokenbox{CE}\linebreak[3]\tokenbox{ED}\linebreak[3]\tokenbox{~THE}\linebreak[3]\tokenbox{~SP}\linebreak[3]\tokenbox{ACE}\linebreak[3]\tokenbox{~PROVIDED}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~The}\linebreak[3]\tokenbox{~proposed}\linebreak[3]\tokenbox{~research}\linebreak[3]\tokenbox{~is}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~continued}\linebreak[3]\tokenbox{~study}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~mobile}\linebreak[3]\tokenbox{~intr}\linebreak[3]\tokenbox{ons}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~bacteria}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~The}\linebreak[3]\tokenbox{~mobile}\linebreak[3]\tokenbox{~group}\linebreak[3]\tokenbox{~I}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~group}\linebreak[3]\tokenbox{~II}\linebreak[3]\tokenbox{~intr}\linebreak[3]\tokenbox{ons}\linebreak[3]\tokenbox{~are}\linebreak[3]\tokenbox{~both}\linebreak[3]\tokenbox{~self}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{s}\linebreak[3]\tokenbox{plic}\linebreak[3]\tokenbox{ing}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~but}\linebreak[3]\tokenbox{~their}\linebreak[3]\tokenbox{~RNA}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{s}\linebreak[3]\tokenbox{plic}\linebreak[3]\tokenbox{ing}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~DNA}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{mob}\linebreak[3]\tokenbox{ility}\linebreak[3]\tokenbox{~pathways}\linebreak[3]\tokenbox{~are}\linebreak[3]\tokenbox{~distinct}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~In}\linebreak[3]\tokenbox{~each}\linebreak[3]\tokenbox{~case}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~intron}\linebreak[3]\tokenbox{~typically}\linebreak[3]\tokenbox{~transfers}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~an}\linebreak[3]\tokenbox{~alle}\linebreak[3]\tokenbox{lic}\linebreak[3]\tokenbox{~intron}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{less}\linebreak[3]\tokenbox{~site}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~hom}\linebreak[3]\tokenbox{ing}\linebreak[3]\tokenbox{process}\linebreak[3]\tokenbox{~initiated}\linebreak[3]\tokenbox{~by}\linebreak[3]\tokenbox{~intron}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{encoded}\linebreak[3]\tokenbox{~end}\linebreak[3]\tokenbox{onucle}\linebreak[3]\tokenbox{ases}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~For}\linebreak[3]\tokenbox{~group}\linebreak[3]\tokenbox{~I}\linebreak[3]\tokenbox{~intron}\linebreak[3]\tokenbox{~hom}\linebreak[3]\tokenbox{ing}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~recombination}\linebreak[3]\tokenbox{~events}\linebreak[3]\tokenbox{~are}\linebreak[3]\tokenbox{~strictly}\linebreak[3]\tokenbox{~DNA}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{based}\linebreak[3]\tokenbox{~whereas}\linebreak[3]\tokenbox{~for}\linebreak[3]\tokenbox{~group}\linebreak[3]\tokenbox{~II}\linebreak[3]\tokenbox{~intron}\linebreak[3]\tokenbox{~hom}\linebreak[3]\tokenbox{ing}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~also}\linebreak[3]\tokenbox{~termed}\linebreak[3]\tokenbox{~retro}\linebreak[3]\tokenbox{hom}\linebreak[3]\tokenbox{ing}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~RNA}\linebreak[3]\tokenbox{~is}\linebreak[3]\tokenbox{~involved}\linebreak[3]\tokenbox{~at}\linebreak[3]\tokenbox{~levels}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~both}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~intron}\linebreak[3]\tokenbox{~template}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~cleavage}\linebreak[3]\tokenbox{~enzyme}\linebreak[3]\tokenbox{~for}\linebreak[3]\tokenbox{~mobility}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~Trans}\linebreak[3]\tokenbox{position}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~ectopic}\linebreak[3]\tokenbox{~sites}\linebreak[3]\tokenbox{~also}\linebreak[3]\tokenbox{~occurs}\linebreak[3]\tokenbox{~at}\linebreak[3]\tokenbox{~low}\linebreak[3]\tokenbox{~frequency}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~is}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~process}\linebreak[3]\tokenbox{~responsible}\linebreak[3]\tokenbox{~for}\linebreak[3]\tokenbox{~intron}\linebreak[3]\tokenbox{~dissemination}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~nature}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~During}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~current}\linebreak[3]\tokenbox{~funding}\linebreak[3]\tokenbox{~period}\linebreak[3]\tokenbox{~we}\linebreak[3]\tokenbox{~showed}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~following}\linebreak[3]\tokenbox{:}\linebreak[3]\tokenbox{~Hom}\linebreak[3]\tokenbox{ing}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~group}\linebreak[3]\tokenbox{~I}\linebreak[3]\tokenbox{~td}\linebreak[3]\tokenbox{~intron}\linebreak[3]\tokenbox{~is}\linebreak[3]\tokenbox{~regulated}\linebreak[3]\tokenbox{~by}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~very}\linebreak[3]\tokenbox{~end}\linebreak[3]\tokenbox{onucle}\linebreak[3]\tokenbox{ase}\linebreak[3]\tokenbox{~that}\linebreak[3]\tokenbox{~promotes}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~process}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~by}\linebreak[3]\tokenbox{~acting}\linebreak[3]\tokenbox{~as}\linebreak[3]\tokenbox{~an}\linebreak[3]\tokenbox{~autore}\linebreak[3]\tokenbox{press}\linebreak[3]\tokenbox{or}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~Also}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~retro}\linebreak[3]\tokenbox{hom}\linebreak[3]\tokenbox{ing}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~group}\linebreak[3]\tokenbox{~II}\linebreak[3]\tokenbox{~intr}\linebreak[3]\tokenbox{ons}\linebreak[3]\tokenbox{~is}\linebreak[3]\tokenbox{~dependent}\linebreak[3]\tokenbox{~on}\linebreak[3]\tokenbox{~host}\linebreak[3]\tokenbox{~polymer}\linebreak[3]\tokenbox{ases}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~way}\linebreak[3]\tokenbox{~that}\linebreak[3]\tokenbox{~suggests}\linebreak[3]\tokenbox{~}\linebreak[3]
}
\end{tokenized}
\end{minipage}

==> Figures/tokenization/examples_new/OpenSubtitles.tex <==
\begin{minipage}{\textwidth}
\subcaption*{{GPT-2 Tokenization}}
\small\vspace{-0.5\baselineskip}\centering{257 tokens}
\begin{tokenized}
\parbox{\linewidth}{\small
\tokenbox{"}\linebreak[3]\tokenbox{Once}\linebreak[3]\tokenbox{~upon}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~time}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~village}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~ancient}\linebreak[3]\tokenbox{~India}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~there}\linebreak[3]\tokenbox{~was}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~little}\linebreak[3]\tokenbox{~goat}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~priest}\linebreak[3]\tokenbox{."}\linebreak[3]\tokenbox{~"}\linebreak[3]\tokenbox{The}\linebreak[3]\tokenbox{~priest}\linebreak[3]\tokenbox{~wanted}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~sacrifice}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~goat}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~gods}\linebreak[3]\tokenbox{."}\linebreak[3]\tokenbox{~"}\linebreak[3]\tokenbox{He}\linebreak[3]\tokenbox{~raised}\linebreak[3]\tokenbox{~his}\linebreak[3]\tokenbox{~arm}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~cut}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~goat}\linebreak[3]\tokenbox{'s}\linebreak[3]\tokenbox{~throat}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~when}\linebreak[3]\tokenbox{~suddenly}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~goat}\linebreak[3]\tokenbox{~began}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~laugh}\linebreak[3]\tokenbox{."}\linebreak[3]\tokenbox{~"}\linebreak[3]\tokenbox{The}\linebreak[3]\tokenbox{~priest}\linebreak[3]\tokenbox{~stopped}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~amazed}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~asked}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~goat}\linebreak[3]\tokenbox{,"}\linebreak[3]\tokenbox{~""}\linebreak[3]\tokenbox{Why}\linebreak[3]\tokenbox{~do}\linebreak[3]\tokenbox{~you}\linebreak[3]\tokenbox{~laugh}\linebreak[3]\tokenbox{?"}\linebreak[3]\tokenbox{~"}\linebreak[3]\tokenbox{Don}\linebreak[3]\tokenbox{'t}\linebreak[3]\tokenbox{~you}\linebreak[3]\tokenbox{~know}\linebreak[3]\tokenbox{~I}\linebreak[3]\tokenbox{'m}\linebreak[3]\tokenbox{~about}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~cut}\linebreak[3]\tokenbox{~your}\linebreak[3]\tokenbox{~throat}\linebreak[3]\tokenbox{?"}\linebreak[3]\tokenbox{"}\linebreak[3]\tokenbox{~""}\linebreak[3]\tokenbox{Oh}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~yes}\linebreak[3]\tokenbox{,"}\linebreak[3]\tokenbox{~said}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~goat}\linebreak[3]\tokenbox{."}\linebreak[3]\tokenbox{~""}\linebreak[3]\tokenbox{After}\linebreak[3]\tokenbox{~499}\linebreak[3]\tokenbox{~times}\linebreak[3]\tokenbox{~dying}\linebreak[3]\tokenbox{...}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~being}\linebreak[3]\tokenbox{~reborn}\linebreak[3]\tokenbox{~as}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~goat}\linebreak[3]\tokenbox{,"}\linebreak[3]\tokenbox{~"}\linebreak[3]\tokenbox{I}\linebreak[3]\tokenbox{~will}\linebreak[3]\tokenbox{~be}\linebreak[3]\tokenbox{~reborn}\linebreak[3]\tokenbox{~as}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~human}\linebreak[3]\tokenbox{~being}\linebreak[3]\tokenbox{.""}\linebreak[3]\tokenbox{~"}\linebreak[3]\tokenbox{Then}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~little}\linebreak[3]\tokenbox{~goat}\linebreak[3]\tokenbox{~began}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~cry}\linebreak[3]\tokenbox{."}\linebreak[3]\tokenbox{~"}\linebreak[3]\tokenbox{The}\linebreak[3]\tokenbox{~high}\linebreak[3]\tokenbox{~priest}\linebreak[3]\tokenbox{~said}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~"}\linebreak[3]\tokenbox{Why}\linebreak[3]\tokenbox{~now}\linebreak[3]\tokenbox{~are}\linebreak[3]\tokenbox{~you}\linebreak[3]\tokenbox{~crying}\linebreak[3]\tokenbox{?"}\linebreak[3]\tokenbox{"}\linebreak[3]\tokenbox{~"}\linebreak[3]\tokenbox{And}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~goat}\linebreak[3]\tokenbox{~replied}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~"}\linebreak[3]\tokenbox{For}\linebreak[3]\tokenbox{~you}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~poor}\linebreak[3]\tokenbox{~priest}\linebreak[3]\tokenbox{."}\linebreak[3]\tokenbox{~"}\linebreak[3]\tokenbox{500}\linebreak[3]\tokenbox{~lives}\linebreak[3]\tokenbox{~ago}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~I}\linebreak[3]\tokenbox{~too}\linebreak[3]\tokenbox{~was}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~high}\linebreak[3]\tokenbox{~priest}\linebreak[3]\tokenbox{...}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~sacrificed}\linebreak[3]\tokenbox{~goats}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~gods}\linebreak[3]\tokenbox{.""}\linebreak[3]\tokenbox{~"}\linebreak[3]\tokenbox{The}\linebreak[3]\tokenbox{~priest}\linebreak[3]\tokenbox{~dropped}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~his}\linebreak[3]\tokenbox{~knees}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~saying}\linebreak[3]\tokenbox{,"}\linebreak[3]\tokenbox{~""}\linebreak[3]\tokenbox{For}\linebreak[3]\tokenbox{give}\linebreak[3]\tokenbox{~me}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~I}\linebreak[3]\tokenbox{~beg}\linebreak[3]\tokenbox{~you}\linebreak[3]\tokenbox{."}\linebreak[3]\tokenbox{~"}\linebreak[3]\tokenbox{From}\linebreak[3]\tokenbox{~now}\linebreak[3]\tokenbox{~on}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~I}\linebreak[3]\tokenbox{~will}\linebreak[3]\tokenbox{~be}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~guardian}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~protector}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~every}\linebreak[3]\tokenbox{~goat}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~land}\linebreak[3]\tokenbox{.""}\linebreak[3]\tokenbox{~"}\linebreak[3]\tokenbox{Now}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~then}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~what}\linebreak[3]\tokenbox{~does}\linebreak[3]\tokenbox{~this}\linebreak[3]\tokenbox{~ancient}\linebreak[3]\tokenbox{~tale}\linebreak[3]\tokenbox{~teach}\linebreak[3]\tokenbox{~us}\linebreak[3]\tokenbox{?"}\linebreak[3]\tokenbox{~"}\linebreak[3]\tokenbox{That}\linebreak[3]\tokenbox{~no}\linebreak[3]\tokenbox{~living}\linebreak[3]\tokenbox{~creature}\linebreak[3]\tokenbox{...}\linebreak[3]\tokenbox{~must}\linebreak[3]\tokenbox{~ever}\linebreak[3]\tokenbox{~be}\linebreak[3]\tokenbox{~sacrificed}\linebreak[3]\tokenbox{."}\linebreak[3]\tokenbox{~"}\linebreak[3]\tokenbox{What}\linebreak[3]\tokenbox{~happened}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~goat}\linebreak[3]\tokenbox{?"}\linebreak[3]\tokenbox{~"}\linebreak[3]\tokenbox{Ah}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~yes}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~goat}\linebreak[3]\tokenbox{."}\linebreak[3]\tokenbox{~"}\linebreak[3]\tokenbox{M}\linebreak[3]\tokenbox{mm}\linebreak[3]\tokenbox{."}\linebreak[3]\tokenbox{~"}\linebreak[3]\tokenbox{Th}\linebreak[3]
}
\end{tokenized}
\end{minipage}
\vskip1.5em
\begin{minipage}{\textwidth}
\subcaption*{{\model{} Tokenization}}
\small\vspace{-0.5\baselineskip}\centering{259 tokens}
\begin{tokenized}
\parbox{\linewidth}{\small
\tokenbox{"}\linebreak[3]\tokenbox{Once}\linebreak[3]\tokenbox{~upon}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~time}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~village}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~ancient}\linebreak[3]\tokenbox{~India}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~there}\linebreak[3]\tokenbox{~was}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~little}\linebreak[3]\tokenbox{~goat}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~priest}\linebreak[3]\tokenbox{."}\linebreak[3]\tokenbox{~"}\linebreak[3]\tokenbox{The}\linebreak[3]\tokenbox{~priest}\linebreak[3]\tokenbox{~wanted}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~sacrifice}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~goat}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~gods}\linebreak[3]\tokenbox{."}\linebreak[3]\tokenbox{~"}\linebreak[3]\tokenbox{He}\linebreak[3]\tokenbox{~raised}\linebreak[3]\tokenbox{~his}\linebreak[3]\tokenbox{~arm}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~cut}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~goat}\linebreak[3]\tokenbox{'s}\linebreak[3]\tokenbox{~throat}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~when}\linebreak[3]\tokenbox{~suddenly}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~goat}\linebreak[3]\tokenbox{~began}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~laugh}\linebreak[3]\tokenbox{."}\linebreak[3]\tokenbox{~"}\linebreak[3]\tokenbox{The}\linebreak[3]\tokenbox{~priest}\linebreak[3]\tokenbox{~stopped}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~amazed}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~asked}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~goat}\linebreak[3]\tokenbox{,"}\linebreak[3]\tokenbox{~""}\linebreak[3]\tokenbox{Why}\linebreak[3]\tokenbox{~do}\linebreak[3]\tokenbox{~you}\linebreak[3]\tokenbox{~laugh}\linebreak[3]\tokenbox{?"}\linebreak[3]\tokenbox{~"}\linebreak[3]\tokenbox{Don}\linebreak[3]\tokenbox{'t}\linebreak[3]\tokenbox{~you}\linebreak[3]\tokenbox{~know}\linebreak[3]\tokenbox{~I}\linebreak[3]\tokenbox{'m}\linebreak[3]\tokenbox{~about}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~cut}\linebreak[3]\tokenbox{~your}\linebreak[3]\tokenbox{~throat}\linebreak[3]\tokenbox{?"}\linebreak[3]\tokenbox{"}\linebreak[3]\tokenbox{~""}\linebreak[3]\tokenbox{Oh}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~yes}\linebreak[3]\tokenbox{,"}\linebreak[3]\tokenbox{~said}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~goat}\linebreak[3]\tokenbox{."}\linebreak[3]\tokenbox{~""}\linebreak[3]\tokenbox{After}\linebreak[3]\tokenbox{~499}\linebreak[3]\tokenbox{~times}\linebreak[3]\tokenbox{~dying}\linebreak[3]\tokenbox{...}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~being}\linebreak[3]\tokenbox{~reb}\linebreak[3]\tokenbox{orn}\linebreak[3]\tokenbox{~as}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~goat}\linebreak[3]\tokenbox{,"}\linebreak[3]\tokenbox{~"}\linebreak[3]\tokenbox{I}\linebreak[3]\tokenbox{~will}\linebreak[3]\tokenbox{~be}\linebreak[3]\tokenbox{~reb}\linebreak[3]\tokenbox{orn}\linebreak[3]\tokenbox{~as}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~human}\linebreak[3]\tokenbox{~being}\linebreak[3]\tokenbox{.""}\linebreak[3]\tokenbox{~"}\linebreak[3]\tokenbox{Then}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~little}\linebreak[3]\tokenbox{~goat}\linebreak[3]\tokenbox{~began}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~cry}\linebreak[3]\tokenbox{."}\linebreak[3]\tokenbox{~"}\linebreak[3]\tokenbox{The}\linebreak[3]\tokenbox{~high}\linebreak[3]\tokenbox{~priest}\linebreak[3]\tokenbox{~said}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~"}\linebreak[3]\tokenbox{Why}\linebreak[3]\tokenbox{~now}\linebreak[3]\tokenbox{~are}\linebreak[3]\tokenbox{~you}\linebreak[3]\tokenbox{~crying}\linebreak[3]\tokenbox{?"}\linebreak[3]\tokenbox{"}\linebreak[3]\tokenbox{~"}\linebreak[3]\tokenbox{And}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~goat}\linebreak[3]\tokenbox{~replied}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~"}\linebreak[3]\tokenbox{For}\linebreak[3]\tokenbox{~you}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~poor}\linebreak[3]\tokenbox{~priest}\linebreak[3]\tokenbox{."}\linebreak[3]\tokenbox{~"}\linebreak[3]\tokenbox{500}\linebreak[3]\tokenbox{~lives}\linebreak[3]\tokenbox{~ago}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~I}\linebreak[3]\tokenbox{~too}\linebreak[3]\tokenbox{~was}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~high}\linebreak[3]\tokenbox{~priest}\linebreak[3]\tokenbox{...}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~sacrificed}\linebreak[3]\tokenbox{~goats}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~gods}\linebreak[3]\tokenbox{.""}\linebreak[3]\tokenbox{~"}\linebreak[3]\tokenbox{The}\linebreak[3]\tokenbox{~priest}\linebreak[3]\tokenbox{~dropped}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~his}\linebreak[3]\tokenbox{~knees}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~saying}\linebreak[3]\tokenbox{,"}\linebreak[3]\tokenbox{~""}\linebreak[3]\tokenbox{Forg}\linebreak[3]\tokenbox{ive}\linebreak[3]\tokenbox{~me}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~I}\linebreak[3]\tokenbox{~beg}\linebreak[3]\tokenbox{~you}\linebreak[3]\tokenbox{."}\linebreak[3]\tokenbox{~"}\linebreak[3]\tokenbox{From}\linebreak[3]\tokenbox{~now}\linebreak[3]\tokenbox{~on}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~I}\linebreak[3]\tokenbox{~will}\linebreak[3]\tokenbox{~be}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~guardian}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~protector}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~every}\linebreak[3]\tokenbox{~goat}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~land}\linebreak[3]\tokenbox{.""}\linebreak[3]\tokenbox{~"}\linebreak[3]\tokenbox{Now}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~then}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~what}\linebreak[3]\tokenbox{~does}\linebreak[3]\tokenbox{~this}\linebreak[3]\tokenbox{~ancient}\linebreak[3]\tokenbox{~tale}\linebreak[3]\tokenbox{~teach}\linebreak[3]\tokenbox{~us}\linebreak[3]\tokenbox{?"}\linebreak[3]\tokenbox{~"}\linebreak[3]\tokenbox{That}\linebreak[3]\tokenbox{~no}\linebreak[3]\tokenbox{~living}\linebreak[3]\tokenbox{~creature}\linebreak[3]\tokenbox{...}\linebreak[3]\tokenbox{~must}\linebreak[3]\tokenbox{~ever}\linebreak[3]\tokenbox{~be}\linebreak[3]\tokenbox{~sacrificed}\linebreak[3]\tokenbox{."}\linebreak[3]\tokenbox{~"}\linebreak[3]\tokenbox{What}\linebreak[3]\tokenbox{~happened}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~goat}\linebreak[3]\tokenbox{?"}\linebreak[3]\tokenbox{~"}\linebreak[3]\tokenbox{Ah}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~yes}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~goat}\linebreak[3]\tokenbox{."}\linebreak[3]\tokenbox{~"}\linebreak[3]\tokenbox{M}\linebreak[3]\tokenbox{mm}\linebreak[3]\tokenbox{."}\linebreak[3]\tokenbox{~"}\linebreak[3]\tokenbox{Th}\linebreak[3]
}
\end{tokenized}
\end{minipage}

==> Figures/tokenization/examples_new/PhilPapers.tex <==
\begin{minipage}{\textwidth}
\subcaption*{{GPT-2 Tokenization}}
\small\vspace{-0.5\baselineskip}\centering{224 tokens}
\begin{tokenized}
\parbox{\linewidth}{\small
\tokenbox{Raw}\linebreak[3]\tokenbox{ls}\linebreak[3]\tokenbox{ian}\linebreak[3]\tokenbox{~Self}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{Res}\linebreak[3]\tokenbox{pect}\linebreak[3]\tokenbox{1}\linebreak[3]\tokenbox{~cyn}\linebreak[3]\tokenbox{thia}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~stark}\linebreak[3]\tokenbox{~Self}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{respect}\linebreak[3]\tokenbox{~is}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~good}\linebreak[3]\tokenbox{~whose}\linebreak[3]\tokenbox{~value}\linebreak[3]\tokenbox{~seems}\linebreak[3]\tokenbox{~undeniable}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~As}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~consequence}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~it}\linebreak[3]\tokenbox{~presents}\linebreak[3]\tokenbox{~itself}\linebreak[3]\tokenbox{~as}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~notion}\linebreak[3]\tokenbox{~capable}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~justifying}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~value}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~other}\linebreak[3]\tokenbox{~goods}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~Indeed}\linebreak[3]\tokenbox{~it}\linebreak[3]\tokenbox{~has}\linebreak[3]\tokenbox{~been}\linebreak[3]\tokenbox{~employed}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~this}\linebreak[3]\tokenbox{~way}\linebreak[3]\tokenbox{~by}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~number}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~philosophers}\linebreak[3]\tokenbox{~(}\linebreak[3]\tokenbox{Box}\linebreak[3]\tokenbox{ill}\linebreak[3]\tokenbox{~1976}\linebreak[3]\tokenbox{;}\linebreak[3]\tokenbox{~Held}\linebreak[3]\tokenbox{~1973}\linebreak[3]\tokenbox{;}\linebreak[3]\tokenbox{~Post}\linebreak[3]\tokenbox{ow}\linebreak[3]\tokenbox{~1979}\linebreak[3]\tokenbox{;}\linebreak[3]\tokenbox{~Miller}\linebreak[3]\tokenbox{~1982}\linebreak[3]\tokenbox{;}\linebreak[3]\tokenbox{~Moh}\linebreak[3]\tokenbox{r}\linebreak[3]\tokenbox{~1988}\linebreak[3]\tokenbox{).}\linebreak[3]\tokenbox{~The}\linebreak[3]\tokenbox{~most}\linebreak[3]\tokenbox{~prominent}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~these}\linebreak[3]\tokenbox{~is}\linebreak[3]\tokenbox{~John}\linebreak[3]\tokenbox{~Raw}\linebreak[3]\tokenbox{ls}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~Raw}\linebreak[3]\tokenbox{ls}\linebreak[3]\tokenbox{~appeals}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~good}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~self}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{respect}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~justify}\linebreak[3]\tokenbox{~many}\linebreak[3]\tokenbox{~features}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~"}\linebreak[3]\tokenbox{justice}\linebreak[3]\tokenbox{~as}\linebreak[3]\tokenbox{~fairness}\linebreak[3]\tokenbox{"-}\linebreak[3]\tokenbox{the}\linebreak[3]\tokenbox{~highly}\linebreak[3]\tokenbox{~influential}\linebreak[3]\tokenbox{~account}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~distribut}\linebreak[3]\tokenbox{ive}\linebreak[3]\tokenbox{~justice}\linebreak[3]\tokenbox{~presented}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~A}\linebreak[3]\tokenbox{~Theory}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~Justice}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~Most}\linebreak[3]\tokenbox{~who}\linebreak[3]\tokenbox{~have}\linebreak[3]\tokenbox{~considered}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~role}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~self}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{respect}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~Raw}\linebreak[3]\tokenbox{ls}\linebreak[3]\tokenbox{'s}\linebreak[3]\tokenbox{~theory}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~throughout}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~four}\linebreak[3]\tokenbox{~decades}\linebreak[3]\tokenbox{~since}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~publication}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~A}\linebreak[3]\tokenbox{~Theory}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~Justice}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~have}\linebreak[3]\tokenbox{~agreed}\linebreak[3]\tokenbox{~that}\linebreak[3]\tokenbox{~Raw}\linebreak[3]\tokenbox{ls}\linebreak[3]\tokenbox{'s}\linebreak[3]\tokenbox{~argument}\linebreak[3]\tokenbox{~rests}\linebreak[3]\tokenbox{~upon}\linebreak[3]\tokenbox{~an}\linebreak[3]\tokenbox{~irre}\linebreak[3]\tokenbox{parable}\linebreak[3]\tokenbox{~equ}\linebreak[3]\tokenbox{iv}\linebreak[3]\tokenbox{ocation}\linebreak[3]\tokenbox{~between}\linebreak[3]\tokenbox{~two}\linebreak[3]\tokenbox{~different}\linebreak[3]\tokenbox{~ideals}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~self}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{respect}\linebreak[3]\tokenbox{~(}\linebreak[3]\tokenbox{Do}\linebreak[3]\tokenbox{pp}\linebreak[3]\tokenbox{elt}\linebreak[3]\tokenbox{~2009}\linebreak[3]\tokenbox{;}\linebreak[3]\tokenbox{~Ey}\linebreak[3]\tokenbox{al}\linebreak[3]\tokenbox{~2009}\linebreak[3]\tokenbox{;}\linebreak[3]\tokenbox{~Mori}\linebreak[3]\tokenbox{arty}\linebreak[3]\tokenbox{~2009}\linebreak[3]\tokenbox{;}\linebreak[3]\tokenbox{~Thomas}\linebreak[3]\tokenbox{~1978}\linebreak[3]\tokenbox{a}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~1978}\linebreak[3]\tokenbox{b}\linebreak[3]\tokenbox{).}\linebreak[3]\tokenbox{2}\linebreak[3]\tokenbox{~In}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~face}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~this}\linebreak[3]\tokenbox{~critical}\linebreak[3]\tokenbox{~consensus}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~I}\linebreak[3]\tokenbox{~attempt}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~resurrect}\linebreak[3]\tokenbox{~Raw}\linebreak[3]\tokenbox{ls}\linebreak[3]\tokenbox{'s}\linebreak[3]\tokenbox{~approach}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~I}\linebreak[3]\tokenbox{~show}\linebreak[3]\tokenbox{~first}\linebreak[3]\tokenbox{~that}\linebreak[3]\tokenbox{~Raw}\linebreak[3]\tokenbox{ls}\linebreak[3]\tokenbox{~relies}\linebreak[3]\tokenbox{~upon}\linebreak[3]\tokenbox{~an}\linebreak[3]\tokenbox{~unamb}\linebreak[3]\tokenbox{ig}\linebreak[3]\tokenbox{u}\linebreak[3]\tokenbox{ou}\linebreak[3]
}
\end{tokenized}
\end{minipage}
\vskip1.5em
\begin{minipage}{\textwidth}
\subcaption*{{\model{} Tokenization}}
\small\vspace{-0.5\baselineskip}\centering{228 tokens}
\begin{tokenized}
\parbox{\linewidth}{\small
\tokenbox{Raw}\linebreak[3]\tokenbox{ls}\linebreak[3]\tokenbox{ian}\linebreak[3]\tokenbox{~Self}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{Res}\linebreak[3]\tokenbox{pect}\linebreak[3]\tokenbox{1}\linebreak[3]\tokenbox{~cyn}\linebreak[3]\tokenbox{thia}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~stark}\linebreak[3]\tokenbox{~Self}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{respect}\linebreak[3]\tokenbox{~is}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~good}\linebreak[3]\tokenbox{~whose}\linebreak[3]\tokenbox{~value}\linebreak[3]\tokenbox{~seems}\linebreak[3]\tokenbox{~unden}\linebreak[3]\tokenbox{iable}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~As}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~consequence}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~it}\linebreak[3]\tokenbox{~presents}\linebreak[3]\tokenbox{~itself}\linebreak[3]\tokenbox{~as}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~notion}\linebreak[3]\tokenbox{~capable}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~just}\linebreak[3]\tokenbox{ifying}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~value}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~other}\linebreak[3]\tokenbox{~goods}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~Indeed}\linebreak[3]\tokenbox{~it}\linebreak[3]\tokenbox{~has}\linebreak[3]\tokenbox{~been}\linebreak[3]\tokenbox{~employed}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~this}\linebreak[3]\tokenbox{~way}\linebreak[3]\tokenbox{~by}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~number}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~philosophers}\linebreak[3]\tokenbox{~(}\linebreak[3]\tokenbox{Box}\linebreak[3]\tokenbox{ill}\linebreak[3]\tokenbox{~1976}\linebreak[3]\tokenbox{;}\linebreak[3]\tokenbox{~Hel}\linebreak[3]\tokenbox{d}\linebreak[3]\tokenbox{~1973}\linebreak[3]\tokenbox{;}\linebreak[3]\tokenbox{~Post}\linebreak[3]\tokenbox{ow}\linebreak[3]\tokenbox{~1979}\linebreak[3]\tokenbox{;}\linebreak[3]\tokenbox{~Miller}\linebreak[3]\tokenbox{~1982}\linebreak[3]\tokenbox{;}\linebreak[3]\tokenbox{~Moh}\linebreak[3]\tokenbox{r}\linebreak[3]\tokenbox{~1988}\linebreak[3]\tokenbox{).}\linebreak[3]\tokenbox{~The}\linebreak[3]\tokenbox{~most}\linebreak[3]\tokenbox{~prominent}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~these}\linebreak[3]\tokenbox{~is}\linebreak[3]\tokenbox{~John}\linebreak[3]\tokenbox{~Raw}\linebreak[3]\tokenbox{ls}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~Raw}\linebreak[3]\tokenbox{ls}\linebreak[3]\tokenbox{~appeals}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~good}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~self}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{respect}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~justify}\linebreak[3]\tokenbox{~many}\linebreak[3]\tokenbox{~features}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~"}\linebreak[3]\tokenbox{just}\linebreak[3]\tokenbox{ice}\linebreak[3]\tokenbox{~as}\linebreak[3]\tokenbox{~fairness}\linebreak[3]\tokenbox{"-}\linebreak[3]\tokenbox{the}\linebreak[3]\tokenbox{~highly}\linebreak[3]\tokenbox{~influential}\linebreak[3]\tokenbox{~account}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~distribut}\linebreak[3]\tokenbox{ive}\linebreak[3]\tokenbox{~justice}\linebreak[3]\tokenbox{~presented}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~A}\linebreak[3]\tokenbox{~Theory}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~Justice}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~Most}\linebreak[3]\tokenbox{~who}\linebreak[3]\tokenbox{~have}\linebreak[3]\tokenbox{~considered}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~role}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~self}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{respect}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~Raw}\linebreak[3]\tokenbox{ls}\linebreak[3]\tokenbox{'s}\linebreak[3]\tokenbox{~theory}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~throughout}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~four}\linebreak[3]\tokenbox{~decades}\linebreak[3]\tokenbox{~since}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~publication}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~A}\linebreak[3]\tokenbox{~Theory}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~Justice}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~have}\linebreak[3]\tokenbox{~agreed}\linebreak[3]\tokenbox{~that}\linebreak[3]\tokenbox{~Raw}\linebreak[3]\tokenbox{ls}\linebreak[3]\tokenbox{'s}\linebreak[3]\tokenbox{~argument}\linebreak[3]\tokenbox{~rests}\linebreak[3]\tokenbox{~upon}\linebreak[3]\tokenbox{~an}\linebreak[3]\tokenbox{~irre}\linebreak[3]\tokenbox{parable}\linebreak[3]\tokenbox{~equiv}\linebreak[3]\tokenbox{ocation}\linebreak[3]\tokenbox{~between}\linebreak[3]\tokenbox{~two}\linebreak[3]\tokenbox{~different}\linebreak[3]\tokenbox{~ideals}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~self}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{respect}\linebreak[3]\tokenbox{~(}\linebreak[3]\tokenbox{Do}\linebreak[3]\tokenbox{pp}\linebreak[3]\tokenbox{elt}\linebreak[3]\tokenbox{~2009}\linebreak[3]\tokenbox{;}\linebreak[3]\tokenbox{~Ey}\linebreak[3]\tokenbox{al}\linebreak[3]\tokenbox{~2009}\linebreak[3]\tokenbox{;}\linebreak[3]\tokenbox{~Mor}\linebreak[3]\tokenbox{i}\linebreak[3]\tokenbox{arty}\linebreak[3]\tokenbox{~2009}\linebreak[3]\tokenbox{;}\linebreak[3]\tokenbox{~Thomas}\linebreak[3]\tokenbox{~1978}\linebreak[3]\tokenbox{a}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~1978}\linebreak[3]\tokenbox{b}\linebreak[3]\tokenbox{).}\linebreak[3]\tokenbox{2}\linebreak[3]\tokenbox{~In}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~face}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~this}\linebreak[3]\tokenbox{~critical}\linebreak[3]\tokenbox{~consensus}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~I}\linebreak[3]\tokenbox{~attempt}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~resur}\linebreak[3]\tokenbox{rect}\linebreak[3]\tokenbox{~Raw}\linebreak[3]\tokenbox{ls}\linebreak[3]\tokenbox{'s}\linebreak[3]\tokenbox{~approach}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~I}\linebreak[3]\tokenbox{~show}\linebreak[3]\tokenbox{~first}\linebreak[3]\tokenbox{~that}\linebreak[3]\tokenbox{~Raw}\linebreak[3]\tokenbox{ls}\linebreak[3]\tokenbox{~relies}\linebreak[3]\tokenbox{~upon}\linebreak[3]\tokenbox{~an}\linebreak[3]\tokenbox{~unambig}\linebreak[3]\tokenbox{u}\linebreak[3]\tokenbox{ou}\linebreak[3]
}
\end{tokenized}
\end{minipage}

==> Figures/tokenization/examples_new/Pile-CC.tex <==
\begin{minipage}{\textwidth}
\subcaption*{{GPT-2 Tokenization}}
\small\vspace{-0.5\baselineskip}\centering{303 tokens}
\begin{tokenized}
\parbox{\linewidth}{\small
\tokenbox{Pages}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{Wednesday}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~November}\linebreak[3]\tokenbox{~23}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~2011}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{Watch}\linebreak[3]\tokenbox{~fireworks}\linebreak[3]\tokenbox{~reflect}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~Long}\linebreak[3]\tokenbox{view}\linebreak[3]\tokenbox{Lake}\linebreak[3]\tokenbox{~at}\linebreak[3]\tokenbox{~99}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{7}\linebreak[3]\tokenbox{~The}\linebreak[3]\tokenbox{~Point}\linebreak[3]\tokenbox{’}\linebreak[3]\tokenbox{}\linebreak[3]\tokenbox{s}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~Jackson}\linebreak[3]\tokenbox{Count}\linebreak[3]\tokenbox{y}\linebreak[3]\tokenbox{’}\linebreak[3]\tokenbox{}\linebreak[3]\tokenbox{s}\linebreak[3]\tokenbox{~Christmas}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~Sky}\linebreak[3]\tokenbox{~event}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~At}\linebreak[3]\tokenbox{~6}\linebreak[3]\tokenbox{pm}\linebreak[3]\tokenbox{~today}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~enjoy}\linebreak[3]\tokenbox{~holiday}\linebreak[3]\tokenbox{~stage}\linebreak[3]\tokenbox{~productions}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~A}\linebreak[3]\tokenbox{~fireworks}\linebreak[3]\tokenbox{~display}\linebreak[3]\tokenbox{~synchronized}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~your}\linebreak[3]\tokenbox{~favorite}\linebreak[3]\tokenbox{~holiday}\linebreak[3]\tokenbox{~music}\linebreak[3]\tokenbox{~begins}\linebreak[3]\tokenbox{~at}\linebreak[3]\tokenbox{~7}\linebreak[3]\tokenbox{:}\linebreak[3]\tokenbox{30}\linebreak[3]\tokenbox{pm}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~For}\linebreak[3]\tokenbox{~more}\linebreak[3]\tokenbox{~info}\linebreak[3]\tokenbox{~call}\linebreak[3]\tokenbox{~(}\linebreak[3]\tokenbox{8}\linebreak[3]\tokenbox{16}\linebreak[3]\tokenbox{)}\linebreak[3]\tokenbox{~503}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{48}\linebreak[3]\tokenbox{00}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{R}\linebreak[3]\tokenbox{US}\linebreak[3]\tokenbox{K}\linebreak[3]\tokenbox{IN}\linebreak[3]\tokenbox{~CHO}\linebreak[3]\tokenbox{IR}\linebreak[3]\tokenbox{~PER}\linebreak[3]\tokenbox{F}\linebreak[3]\tokenbox{OM}\linebreak[3]\tokenbox{S}\linebreak[3]\tokenbox{~AT}\linebreak[3]\tokenbox{~PL}\linebreak[3]\tokenbox{AZ}\linebreak[3]\tokenbox{A}\linebreak[3]\tokenbox{~L}\linebreak[3]\tokenbox{IGHT}\linebreak[3]\tokenbox{ING}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{R}\linebreak[3]\tokenbox{HS}\linebreak[3]\tokenbox{’}\linebreak[3]\tokenbox{}\linebreak[3]\tokenbox{~Advanced}\linebreak[3]\tokenbox{~Cho}\linebreak[3]\tokenbox{ir}\linebreak[3]\tokenbox{~will}\linebreak[3]\tokenbox{~perform}\linebreak[3]\tokenbox{~at}\linebreak[3]\tokenbox{~this}\linebreak[3]\tokenbox{~year}\linebreak[3]\tokenbox{’}\linebreak[3]\tokenbox{}\linebreak[3]\tokenbox{s}\linebreak[3]\tokenbox{~Plaza}\linebreak[3]\tokenbox{~Lighting}\linebreak[3]\tokenbox{~Cere}\linebreak[3]\tokenbox{mony}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~Thanksgiving}\linebreak[3]\tokenbox{~Day}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~Nov}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~24}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~Rus}\linebreak[3]\tokenbox{kin}\linebreak[3]\tokenbox{~will}\linebreak[3]\tokenbox{~perform}\linebreak[3]\tokenbox{~at}\linebreak[3]\tokenbox{~5}\linebreak[3]\tokenbox{:}\linebreak[3]\tokenbox{20}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{5}\linebreak[3]\tokenbox{:}\linebreak[3]\tokenbox{45}\linebreak[3]\tokenbox{~pm}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~then}\linebreak[3]\tokenbox{~join}\linebreak[3]\tokenbox{~other}\linebreak[3]\tokenbox{~cho}\linebreak[3]\tokenbox{irs}\linebreak[3]\tokenbox{~for}\linebreak[3]\tokenbox{~two}\linebreak[3]\tokenbox{~opening}\linebreak[3]\tokenbox{~numbers}\linebreak[3]\tokenbox{~before}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~actual}\linebreak[3]\tokenbox{~lighting}\linebreak[3]\tokenbox{~ceremony}\linebreak[3]\tokenbox{~at}\linebreak[3]\tokenbox{~7}\linebreak[3]\tokenbox{pm}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{KC}\linebreak[3]\tokenbox{~Mayor}\linebreak[3]\tokenbox{’}\linebreak[3]\tokenbox{}\linebreak[3]\tokenbox{s}\linebreak[3]\tokenbox{~Christmas}\linebreak[3]\tokenbox{~Tree}\linebreak[3]\tokenbox{~Lighting}\linebreak[3]\tokenbox{~Cere}\linebreak[3]\tokenbox{mony}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{On}\linebreak[3]\tokenbox{~Friday}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~November}\linebreak[3]\tokenbox{~25}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~at}\linebreak[3]\tokenbox{~5}\linebreak[3]\tokenbox{:}\linebreak[3]\tokenbox{30}\linebreak[3]\tokenbox{pm}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~join}\linebreak[3]\tokenbox{~Mayor}\linebreak[3]\tokenbox{~Sly}\linebreak[3]\tokenbox{~James}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~R}\linebreak[3]\tokenbox{&}\linebreak[3]\tokenbox{B}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{s}\linebreak[3]\tokenbox{oul}\linebreak[3]\tokenbox{~sensation}\linebreak[3]\tokenbox{~Jan}\linebreak[3]\tokenbox{elle}\linebreak[3]\tokenbox{~Mon}\linebreak[3]\tokenbox{ae}\linebreak[3]\tokenbox{~light}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~100}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{foot}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{tall}\linebreak[3]\tokenbox{~Mayor}\linebreak[3]\tokenbox{’}\linebreak[3]\tokenbox{}\linebreak[3]\tokenbox{s}\linebreak[3]\tokenbox{~Christmas}\linebreak[3]\tokenbox{~Tree}\linebreak[3]\tokenbox{~at}\linebreak[3]\tokenbox{~Crown}\linebreak[3]\tokenbox{Center}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~The}\linebreak[3]\tokenbox{~tree}\linebreak[3]\tokenbox{~is}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~symbol}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~Mayor}\linebreak[3]\tokenbox{’}\linebreak[3]\tokenbox{}\linebreak[3]\tokenbox{s}\linebreak[3]\tokenbox{~Christmas}\linebreak[3]\tokenbox{~Tree}\linebreak[3]\tokenbox{~Fund}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~which}\linebreak[3]\tokenbox{~assists}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~city}\linebreak[3]\tokenbox{’}\linebreak[3]\tokenbox{}\linebreak[3]\tokenbox{s}\linebreak[3]\tokenbox{~less}\linebreak[3]\tokenbox{~fortunate}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~For}\linebreak[3]\tokenbox{~more}\linebreak[3]\tokenbox{~info}\linebreak[3]\tokenbox{~call}\linebreak[3]\tokenbox{~8}\linebreak[3]\tokenbox{16}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{2}\linebreak[3]
}
\end{tokenized}
\end{minipage}
\vskip1.5em
\begin{minipage}{\textwidth}
\subcaption*{{\model{} Tokenization}}
\small\vspace{-0.5\baselineskip}\centering{299 tokens}
\begin{tokenized}
\parbox{\linewidth}{\small
\tokenbox{Pages}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{Wednesday}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~November}\linebreak[3]\tokenbox{~23}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~2011}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{Watch}\linebreak[3]\tokenbox{~fireworks}\linebreak[3]\tokenbox{~reflect}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~Long}\linebreak[3]\tokenbox{view}\linebreak[3]\tokenbox{L}\linebreak[3]\tokenbox{ake}\linebreak[3]\tokenbox{~at}\linebreak[3]\tokenbox{~99}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{7}\linebreak[3]\tokenbox{~The}\linebreak[3]\tokenbox{~Point}\linebreak[3]\tokenbox{’}\linebreak[3]\tokenbox{s}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~Jackson}\linebreak[3]\tokenbox{County}\linebreak[3]\tokenbox{’}\linebreak[3]\tokenbox{s}\linebreak[3]\tokenbox{~Christmas}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~Sky}\linebreak[3]\tokenbox{~event}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~At}\linebreak[3]\tokenbox{~6}\linebreak[3]\tokenbox{pm}\linebreak[3]\tokenbox{~today}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~enjoy}\linebreak[3]\tokenbox{~holiday}\linebreak[3]\tokenbox{~stage}\linebreak[3]\tokenbox{~productions}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~A}\linebreak[3]\tokenbox{~fireworks}\linebreak[3]\tokenbox{~display}\linebreak[3]\tokenbox{~synchronized}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~your}\linebreak[3]\tokenbox{~favorite}\linebreak[3]\tokenbox{~holiday}\linebreak[3]\tokenbox{~music}\linebreak[3]\tokenbox{~begins}\linebreak[3]\tokenbox{~at}\linebreak[3]\tokenbox{~7}\linebreak[3]\tokenbox{:}\linebreak[3]\tokenbox{30}\linebreak[3]\tokenbox{pm}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~For}\linebreak[3]\tokenbox{~more}\linebreak[3]\tokenbox{~info}\linebreak[3]\tokenbox{~call}\linebreak[3]\tokenbox{~(}\linebreak[3]\tokenbox{816}\linebreak[3]\tokenbox{)}\linebreak[3]\tokenbox{~503}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{48}\linebreak[3]\tokenbox{00}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{R}\linebreak[3]\tokenbox{US}\linebreak[3]\tokenbox{K}\linebreak[3]\tokenbox{IN}\linebreak[3]\tokenbox{~CHO}\linebreak[3]\tokenbox{IR}\linebreak[3]\tokenbox{~PER}\linebreak[3]\tokenbox{F}\linebreak[3]\tokenbox{OM}\linebreak[3]\tokenbox{S}\linebreak[3]\tokenbox{~AT}\linebreak[3]\tokenbox{~PLA}\linebreak[3]\tokenbox{ZA}\linebreak[3]\tokenbox{~L}\linebreak[3]\tokenbox{IGHT}\linebreak[3]\tokenbox{ING}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{R}\linebreak[3]\tokenbox{HS}\linebreak[3]\tokenbox{’}\linebreak[3]\tokenbox{~Advanced}\linebreak[3]\tokenbox{~Ch}\linebreak[3]\tokenbox{oir}\linebreak[3]\tokenbox{~will}\linebreak[3]\tokenbox{~perform}\linebreak[3]\tokenbox{~at}\linebreak[3]\tokenbox{~this}\linebreak[3]\tokenbox{~year}\linebreak[3]\tokenbox{’}\linebreak[3]\tokenbox{s}\linebreak[3]\tokenbox{~Plaza}\linebreak[3]\tokenbox{~Light}\linebreak[3]\tokenbox{ing}\linebreak[3]\tokenbox{~Ce}\linebreak[3]\tokenbox{rem}\linebreak[3]\tokenbox{ony}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~Thanksgiving}\linebreak[3]\tokenbox{~Day}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~Nov}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~24}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~Rus}\linebreak[3]\tokenbox{kin}\linebreak[3]\tokenbox{~will}\linebreak[3]\tokenbox{~perform}\linebreak[3]\tokenbox{~at}\linebreak[3]\tokenbox{~5}\linebreak[3]\tokenbox{:}\linebreak[3]\tokenbox{20}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{5}\linebreak[3]\tokenbox{:}\linebreak[3]\tokenbox{45}\linebreak[3]\tokenbox{~pm}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~then}\linebreak[3]\tokenbox{~join}\linebreak[3]\tokenbox{~other}\linebreak[3]\tokenbox{~cho}\linebreak[3]\tokenbox{irs}\linebreak[3]\tokenbox{~for}\linebreak[3]\tokenbox{~two}\linebreak[3]\tokenbox{~opening}\linebreak[3]\tokenbox{~numbers}\linebreak[3]\tokenbox{~before}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~actual}\linebreak[3]\tokenbox{~lighting}\linebreak[3]\tokenbox{~ceremony}\linebreak[3]\tokenbox{~at}\linebreak[3]\tokenbox{~7}\linebreak[3]\tokenbox{pm}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{KC}\linebreak[3]\tokenbox{~Mayor}\linebreak[3]\tokenbox{’}\linebreak[3]\tokenbox{s}\linebreak[3]\tokenbox{~Christmas}\linebreak[3]\tokenbox{~Tree}\linebreak[3]\tokenbox{~Light}\linebreak[3]\tokenbox{ing}\linebreak[3]\tokenbox{~Ce}\linebreak[3]\tokenbox{rem}\linebreak[3]\tokenbox{ony}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{On}\linebreak[3]\tokenbox{~Friday}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~November}\linebreak[3]\tokenbox{~25}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~at}\linebreak[3]\tokenbox{~5}\linebreak[3]\tokenbox{:}\linebreak[3]\tokenbox{30}\linebreak[3]\tokenbox{pm}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~join}\linebreak[3]\tokenbox{~Mayor}\linebreak[3]\tokenbox{~S}\linebreak[3]\tokenbox{ly}\linebreak[3]\tokenbox{~James}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~R}\linebreak[3]\tokenbox{&}\linebreak[3]\tokenbox{B}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{s}\linebreak[3]\tokenbox{oul}\linebreak[3]\tokenbox{~sensation}\linebreak[3]\tokenbox{~Jan}\linebreak[3]\tokenbox{elle}\linebreak[3]\tokenbox{~Mon}\linebreak[3]\tokenbox{ae}\linebreak[3]\tokenbox{~light}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~100}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{foot}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{t}\linebreak[3]\tokenbox{all}\linebreak[3]\tokenbox{~Mayor}\linebreak[3]\tokenbox{’}\linebreak[3]\tokenbox{s}\linebreak[3]\tokenbox{~Christmas}\linebreak[3]\tokenbox{~Tree}\linebreak[3]\tokenbox{~at}\linebreak[3]\tokenbox{~Crown}\linebreak[3]\tokenbox{Center}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~The}\linebreak[3]\tokenbox{~tree}\linebreak[3]\tokenbox{~is}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~symbol}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~Mayor}\linebreak[3]\tokenbox{’}\linebreak[3]\tokenbox{s}\linebreak[3]\tokenbox{~Christmas}\linebreak[3]\tokenbox{~Tree}\linebreak[3]\tokenbox{~Fund}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~which}\linebreak[3]\tokenbox{~assists}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~city}\linebreak[3]\tokenbox{’}\linebreak[3]\tokenbox{s}\linebreak[3]\tokenbox{~less}\linebreak[3]\tokenbox{~fortunate}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~For}\linebreak[3]\tokenbox{~more}\linebreak[3]\tokenbox{~info}\linebreak[3]\tokenbox{~call}\linebreak[3]\tokenbox{~8}\linebreak[3]\tokenbox{16}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{2}\linebreak[3]
}
\end{tokenized}
\end{minipage}

==> Figures/tokenization/examples_new/PubMed_Central.tex <==
\begin{minipage}{\textwidth}
\subcaption*{{GPT-2 Tokenization}}
\small\vspace{-0.5\baselineskip}\centering{303 tokens}
\begin{tokenized}
\parbox{\linewidth}{\small
\tokenbox{1}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~Introduction}\linebreak[3]\tokenbox{~{}\linebreak[3]\tokenbox{\#}\linebreak[3]\tokenbox{sec}\linebreak[3]\tokenbox{1}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{j}\linebreak[3]\tokenbox{cm}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{08}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{020}\linebreak[3]\tokenbox{39}\linebreak[3]\tokenbox{}}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{============}\linebreak[3]\tokenbox{===}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{Ven}\linebreak[3]\tokenbox{ous}\linebreak[3]\tokenbox{~th}\linebreak[3]\tokenbox{rom}\linebreak[3]\tokenbox{bo}\linebreak[3]\tokenbox{emb}\linebreak[3]\tokenbox{ol}\linebreak[3]\tokenbox{ism}\linebreak[3]\tokenbox{~(}\linebreak[3]\tokenbox{V}\linebreak[3]\tokenbox{TE}\linebreak[3]\tokenbox{)}\linebreak[3]\tokenbox{~is}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~common}\linebreak[3]\tokenbox{~cause}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~morbid}\linebreak[3]\tokenbox{ity}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~mortality}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~hospitalized}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~non}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{hospital}\linebreak[3]\tokenbox{ized}\linebreak[3]\tokenbox{~patients}\linebreak[3]\tokenbox{~\textbackslash}\linebreak[3]\tokenbox{[[}\linebreak[3]\tokenbox{@}\linebreak[3]\tokenbox{B}\linebreak[3]\tokenbox{1}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{j}\linebreak[3]\tokenbox{cm}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{08}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{020}\linebreak[3]\tokenbox{39}\linebreak[3]\tokenbox{]}\linebreak[3]\tokenbox{\textbackslash}\linebreak[3]\tokenbox{].}\linebreak[3]\tokenbox{~The}\linebreak[3]\tokenbox{~American}\linebreak[3]\tokenbox{~Society}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~Hem}\linebreak[3]\tokenbox{at}\linebreak[3]\tokenbox{ology}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~American}\linebreak[3]\tokenbox{~College}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~Chest}\linebreak[3]\tokenbox{~Physicians}\linebreak[3]\tokenbox{~guidelines}\linebreak[3]\tokenbox{~recommend}\linebreak[3]\tokenbox{~low}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{m}\linebreak[3]\tokenbox{ole}\linebreak[3]\tokenbox{cular}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{weight}\linebreak[3]\tokenbox{~he}\linebreak[3]\tokenbox{par}\linebreak[3]\tokenbox{in}\linebreak[3]\tokenbox{~(}\linebreak[3]\tokenbox{LM}\linebreak[3]\tokenbox{WH}\linebreak[3]\tokenbox{)}\linebreak[3]\tokenbox{~as}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~first}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{line}\linebreak[3]\tokenbox{~pharmac}\linebreak[3]\tokenbox{ological}\linebreak[3]\tokenbox{~option}\linebreak[3]\tokenbox{~for}\linebreak[3]\tokenbox{~most}\linebreak[3]\tokenbox{~patients}\linebreak[3]\tokenbox{~at}\linebreak[3]\tokenbox{~risk}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~V}\linebreak[3]\tokenbox{TE}\linebreak[3]\tokenbox{~\textbackslash}\linebreak[3]\tokenbox{[[}\linebreak[3]\tokenbox{@}\linebreak[3]\tokenbox{B}\linebreak[3]\tokenbox{2}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{j}\linebreak[3]\tokenbox{cm}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{08}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{020}\linebreak[3]\tokenbox{39}\linebreak[3]\tokenbox{],[}\linebreak[3]\tokenbox{@}\linebreak[3]\tokenbox{B}\linebreak[3]\tokenbox{3}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{j}\linebreak[3]\tokenbox{cm}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{08}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{020}\linebreak[3]\tokenbox{39}\linebreak[3]\tokenbox{]}\linebreak[3]\tokenbox{\textbackslash}\linebreak[3]\tokenbox{].}\linebreak[3]\tokenbox{~Several}\linebreak[3]\tokenbox{~pro}\linebreak[3]\tokenbox{ph}\linebreak[3]\tokenbox{yl}\linebreak[3]\tokenbox{actic}\linebreak[3]\tokenbox{~doses}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~types}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~LM}\linebreak[3]\tokenbox{WH}\linebreak[3]\tokenbox{~are}\linebreak[3]\tokenbox{~used}\linebreak[3]\tokenbox{~worldwide}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~which}\linebreak[3]\tokenbox{~is}\linebreak[3]\tokenbox{~reflected}\linebreak[3]\tokenbox{~by}\linebreak[3]\tokenbox{~differences}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~national}\linebreak[3]\tokenbox{~summ}\linebreak[3]\tokenbox{aries}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~product}\linebreak[3]\tokenbox{~characteristics}\linebreak[3]\tokenbox{~(}\linebreak[3]\tokenbox{SP}\linebreak[3]\tokenbox{Cs}\linebreak[3]\tokenbox{)}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~d}\linebreak[3]\tokenbox{osing}\linebreak[3]\tokenbox{~reg}\linebreak[3]\tokenbox{imens}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~randomized}\linebreak[3]\tokenbox{~controlled}\linebreak[3]\tokenbox{~trials}\linebreak[3]\tokenbox{~(}\linebreak[3]\tokenbox{R}\linebreak[3]\tokenbox{CT}\linebreak[3]\tokenbox{s}\linebreak[3]\tokenbox{).}\linebreak[3]\tokenbox{~There}\linebreak[3]\tokenbox{~is}\linebreak[3]\tokenbox{~no}\linebreak[3]\tokenbox{~high}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{quality}\linebreak[3]\tokenbox{~evidence}\linebreak[3]\tokenbox{~or}\linebreak[3]\tokenbox{~guidance}\linebreak[3]\tokenbox{~on}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~optimal}\linebreak[3]\tokenbox{~pro}\linebreak[3]\tokenbox{ph}\linebreak[3]\tokenbox{yl}\linebreak[3]\tokenbox{actic}\linebreak[3]\tokenbox{~LM}\linebreak[3]\tokenbox{WH}\linebreak[3]\tokenbox{~dose}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~Pre}\linebreak[3]\tokenbox{ced}\linebreak[3]\tokenbox{ing}\linebreak[3]\tokenbox{~systematic}\linebreak[3]\tokenbox{~reviews}\linebreak[3]\tokenbox{~on}\linebreak[3]\tokenbox{~th}\linebreak[3]\tokenbox{rom}\linebreak[3]\tokenbox{b}\linebreak[3]\tokenbox{osis}\linebreak[3]\tokenbox{~pro}\linebreak[3]\tokenbox{ph}\linebreak[3]\tokenbox{yl}\linebreak[3]\tokenbox{axis}\linebreak[3]\tokenbox{~have}\linebreak[3]\tokenbox{~not}\linebreak[3]\tokenbox{~specifically}\linebreak[3]\tokenbox{~assessed}\linebreak[3]\tokenbox{~benefits}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~harms}\linebreak[3]\tokenbox{~associated}\linebreak[3]\tokenbox{~with}\linebreak[3]\tokenbox{~different}\linebreak[3]\tokenbox{~LM}\linebreak[3]\tokenbox{WH}\linebreak[3]\tokenbox{~doses}\linebreak[3]\tokenbox{~\textbackslash}\linebreak[3]\tokenbox{[[}\linebreak[3]\tokenbox{@}\linebreak[3]\tokenbox{B}\linebreak[3]\tokenbox{4}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{j}\linebreak[3]\tokenbox{cm}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{08}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{020}\linebreak[3]\tokenbox{39}\linebreak[3]\tokenbox{],[}\linebreak[3]\tokenbox{@}\linebreak[3]\tokenbox{B}\linebreak[3]\tokenbox{5}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{j}\linebreak[3]\tokenbox{cm}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{08}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{020}\linebreak[3]\tokenbox{39}\linebreak[3]\tokenbox{],[}\linebreak[3]\tokenbox{@}\linebreak[3]\tokenbox{B}\linebreak[3]\tokenbox{6}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{j}\linebreak[3]\tokenbox{cm}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{08}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{020}\linebreak[3]\tokenbox{39}\linebreak[3]\tokenbox{],[}\linebreak[3]\tokenbox{@}\linebreak[3]\tokenbox{B}\linebreak[3]\tokenbox{7}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{j}\linebreak[3]\tokenbox{cm}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{08}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{020}\linebreak[3]\tokenbox{39}\linebreak[3]\tokenbox{],[}\linebreak[3]\tokenbox{@}\linebreak[3]\tokenbox{B}\linebreak[3]\tokenbox{8}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{j}\linebreak[3]\tokenbox{cm}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{08}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{020}\linebreak[3]\tokenbox{39}\linebreak[3]\tokenbox{],[}\linebreak[3]\tokenbox{@}\linebreak[3]\tokenbox{B}\linebreak[3]\tokenbox{9}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{j}\linebreak[3]\tokenbox{cm}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{08}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{020}\linebreak[3]
}
\end{tokenized}
\end{minipage}
\vskip1.5em
\begin{minipage}{\textwidth}
\subcaption*{{\model{} Tokenization}}
\small\vspace{-0.5\baselineskip}\centering{256 tokens}
\begin{tokenized}
\parbox{\linewidth}{\small
\tokenbox{1}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~Introduction}\linebreak[3]\tokenbox{~{\#}\linebreak[3]\tokenbox{sec}\linebreak[3]\tokenbox{1}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{jcm}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{08}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{020}\linebreak[3]\tokenbox{39}\linebreak[3]\tokenbox{}}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{===============}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{Ven}\linebreak[3]\tokenbox{ous}\linebreak[3]\tokenbox{~throm}\linebreak[3]\tokenbox{bo}\linebreak[3]\tokenbox{emb}\linebreak[3]\tokenbox{ol}\linebreak[3]\tokenbox{ism}\linebreak[3]\tokenbox{~(}\linebreak[3]\tokenbox{V}\linebreak[3]\tokenbox{TE}\linebreak[3]\tokenbox{)}\linebreak[3]\tokenbox{~is}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~common}\linebreak[3]\tokenbox{~cause}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~morbidity}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~mortality}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~hospitalized}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~non}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{hospital}\linebreak[3]\tokenbox{ized}\linebreak[3]\tokenbox{~patients}\linebreak[3]\tokenbox{~\textbackslash[[@}\linebreak[3]\tokenbox{B}\linebreak[3]\tokenbox{1}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{jcm}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{08}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{020}\linebreak[3]\tokenbox{39}\linebreak[3]\tokenbox{]\textbackslash].}\linebreak[3]\tokenbox{~The}\linebreak[3]\tokenbox{~American}\linebreak[3]\tokenbox{~Society}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~H}\linebreak[3]\tokenbox{emat}\linebreak[3]\tokenbox{ology}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~American}\linebreak[3]\tokenbox{~College}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~Chest}\linebreak[3]\tokenbox{~Phys}\linebreak[3]\tokenbox{icians}\linebreak[3]\tokenbox{~guidelines}\linebreak[3]\tokenbox{~recommend}\linebreak[3]\tokenbox{~low}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{molecular}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{weight}\linebreak[3]\tokenbox{~heparin}\linebreak[3]\tokenbox{~(}\linebreak[3]\tokenbox{LM}\linebreak[3]\tokenbox{WH}\linebreak[3]\tokenbox{)}\linebreak[3]\tokenbox{~as}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~first}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{line}\linebreak[3]\tokenbox{~pharmacological}\linebreak[3]\tokenbox{~option}\linebreak[3]\tokenbox{~for}\linebreak[3]\tokenbox{~most}\linebreak[3]\tokenbox{~patients}\linebreak[3]\tokenbox{~at}\linebreak[3]\tokenbox{~risk}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~V}\linebreak[3]\tokenbox{TE}\linebreak[3]\tokenbox{~\textbackslash[[@}\linebreak[3]\tokenbox{B}\linebreak[3]\tokenbox{2}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{jcm}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{08}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{020}\linebreak[3]\tokenbox{39}\linebreak[3]\tokenbox{],[@}\linebreak[3]\tokenbox{B}\linebreak[3]\tokenbox{3}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{jcm}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{08}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{020}\linebreak[3]\tokenbox{39}\linebreak[3]\tokenbox{]\textbackslash].}\linebreak[3]\tokenbox{~Several}\linebreak[3]\tokenbox{~prophylactic}\linebreak[3]\tokenbox{~doses}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~types}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~LM}\linebreak[3]\tokenbox{WH}\linebreak[3]\tokenbox{~are}\linebreak[3]\tokenbox{~used}\linebreak[3]\tokenbox{~worldwide}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~which}\linebreak[3]\tokenbox{~is}\linebreak[3]\tokenbox{~reflected}\linebreak[3]\tokenbox{~by}\linebreak[3]\tokenbox{~differences}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~national}\linebreak[3]\tokenbox{~summ}\linebreak[3]\tokenbox{aries}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~product}\linebreak[3]\tokenbox{~characteristics}\linebreak[3]\tokenbox{~(}\linebreak[3]\tokenbox{SP}\linebreak[3]\tokenbox{Cs}\linebreak[3]\tokenbox{)}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~dosing}\linebreak[3]\tokenbox{~regimens}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~randomized}\linebreak[3]\tokenbox{~controlled}\linebreak[3]\tokenbox{~trials}\linebreak[3]\tokenbox{~(}\linebreak[3]\tokenbox{R}\linebreak[3]\tokenbox{CT}\linebreak[3]\tokenbox{s}\linebreak[3]\tokenbox{).}\linebreak[3]\tokenbox{~There}\linebreak[3]\tokenbox{~is}\linebreak[3]\tokenbox{~no}\linebreak[3]\tokenbox{~high}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{quality}\linebreak[3]\tokenbox{~evidence}\linebreak[3]\tokenbox{~or}\linebreak[3]\tokenbox{~guidance}\linebreak[3]\tokenbox{~on}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~optimal}\linebreak[3]\tokenbox{~prophylactic}\linebreak[3]\tokenbox{~LM}\linebreak[3]\tokenbox{WH}\linebreak[3]\tokenbox{~dose}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~Pre}\linebreak[3]\tokenbox{ced}\linebreak[3]\tokenbox{ing}\linebreak[3]\tokenbox{~systematic}\linebreak[3]\tokenbox{~reviews}\linebreak[3]\tokenbox{~on}\linebreak[3]\tokenbox{~thrombosis}\linebreak[3]\tokenbox{~prophylaxis}\linebreak[3]\tokenbox{~have}\linebreak[3]\tokenbox{~not}\linebreak[3]\tokenbox{~specifically}\linebreak[3]\tokenbox{~assessed}\linebreak[3]\tokenbox{~benefits}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~har}\linebreak[3]\tokenbox{ms}\linebreak[3]\tokenbox{~associated}\linebreak[3]\tokenbox{~with}\linebreak[3]\tokenbox{~different}\linebreak[3]\tokenbox{~LM}\linebreak[3]\tokenbox{WH}\linebreak[3]\tokenbox{~doses}\linebreak[3]\tokenbox{~\textbackslash[[@}\linebreak[3]\tokenbox{B}\linebreak[3]\tokenbox{4}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{jcm}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{08}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{020}\linebreak[3]\tokenbox{39}\linebreak[3]\tokenbox{],[@}\linebreak[3]\tokenbox{B}\linebreak[3]\tokenbox{5}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{jcm}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{08}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{020}\linebreak[3]\tokenbox{39}\linebreak[3]\tokenbox{],[@}\linebreak[3]\tokenbox{B}\linebreak[3]\tokenbox{6}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{jcm}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{08}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{020}\linebreak[3]\tokenbox{39}\linebreak[3]\tokenbox{],[@}\linebreak[3]\tokenbox{B}\linebreak[3]\tokenbox{7}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{jcm}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{08}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{020}\linebreak[3]\tokenbox{39}\linebreak[3]\tokenbox{],[@}\linebreak[3]\tokenbox{B}\linebreak[3]\tokenbox{8}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{jcm}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{08}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{020}\linebreak[3]\tokenbox{39}\linebreak[3]\tokenbox{],[@}\linebreak[3]\tokenbox{B}\linebreak[3]\tokenbox{9}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{jcm}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{08}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{020}\linebreak[3]
}
\end{tokenized}
\end{minipage}

==> Figures/tokenization/examples_new/StackExchange.tex <==
\begin{minipage}{\textwidth}
\subcaption*{{GPT-2 Tokenization}}
\small\vspace{-0.5\baselineskip}\centering{229 tokens}
\begin{tokenized}
\parbox{\linewidth}{\small
\tokenbox{Q}\linebreak[3]\tokenbox{:}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{Get}\linebreak[3]\tokenbox{~URL}\linebreak[3]\tokenbox{~segment}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~Lara}\linebreak[3]\tokenbox{vel}\linebreak[3]\tokenbox{~5}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{For}\linebreak[3]\tokenbox{~accessing}\linebreak[3]\tokenbox{~previous}\linebreak[3]\tokenbox{~URL}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~l}\linebreak[3]\tokenbox{ara}\linebreak[3]\tokenbox{vel}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~I}\linebreak[3]\tokenbox{~am}\linebreak[3]\tokenbox{~using}\linebreak[3]\tokenbox{~this}\linebreak[3]\tokenbox{~code}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~my}\linebreak[3]\tokenbox{~controller}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{\$}\linebreak[3]\tokenbox{current}\linebreak[3]\tokenbox{\_}\linebreak[3]\tokenbox{url}\linebreak[3]\tokenbox{~=}\linebreak[3]\tokenbox{~Request}\linebreak[3]\tokenbox{::}\linebreak[3]\tokenbox{url}\linebreak[3]\tokenbox{();}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{\$}\linebreak[3]\tokenbox{back}\linebreak[3]\tokenbox{\_}\linebreak[3]\tokenbox{url}\linebreak[3]\tokenbox{~=}\linebreak[3]\tokenbox{~redirect}\linebreak[3]\tokenbox{()}\linebreak[3]\tokenbox{->}\linebreak[3]\tokenbox{back}\linebreak[3]\tokenbox{()}\linebreak[3]\tokenbox{->}\linebreak[3]\tokenbox{get}\linebreak[3]\tokenbox{Target}\linebreak[3]\tokenbox{Url}\linebreak[3]\tokenbox{();}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{if}\linebreak[3]\tokenbox{~(\$}\linebreak[3]\tokenbox{current}\linebreak[3]\tokenbox{\_}\linebreak[3]\tokenbox{url}\linebreak[3]\tokenbox{~!=}\linebreak[3]\tokenbox{~\$}\linebreak[3]\tokenbox{back}\linebreak[3]\tokenbox{\_}\linebreak[3]\tokenbox{url}\linebreak[3]\tokenbox{)}\linebreak[3]\tokenbox{~{}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{~}\linebreak[3]\tokenbox{~Session}\linebreak[3]\tokenbox{::}\linebreak[3]\tokenbox{put}\linebreak[3]\tokenbox{('}\linebreak[3]\tokenbox{pre}\linebreak[3]\tokenbox{vious}\linebreak[3]\tokenbox{\_}\linebreak[3]\tokenbox{url}\linebreak[3]\tokenbox{',}\linebreak[3]\tokenbox{~redirect}\linebreak[3]\tokenbox{()}\linebreak[3]\tokenbox{->}\linebreak[3]\tokenbox{back}\linebreak[3]\tokenbox{()}\linebreak[3]\tokenbox{->}\linebreak[3]\tokenbox{get}\linebreak[3]\tokenbox{Target}\linebreak[3]\tokenbox{Url}\linebreak[3]\tokenbox{());}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{}}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{This}\linebreak[3]\tokenbox{~method}\linebreak[3]\tokenbox{~helps}\linebreak[3]\tokenbox{~main}\linebreak[3]\tokenbox{ta}\linebreak[3]\tokenbox{inging}\linebreak[3]\tokenbox{~previous}\linebreak[3]\tokenbox{~url}\linebreak[3]\tokenbox{~even}\linebreak[3]\tokenbox{~when}\linebreak[3]\tokenbox{~server}\linebreak[3]\tokenbox{~side}\linebreak[3]\tokenbox{~validation}\linebreak[3]\tokenbox{~fails}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{In}\linebreak[3]\tokenbox{~my}\linebreak[3]\tokenbox{~blade}\linebreak[3]\tokenbox{~I}\linebreak[3]\tokenbox{~access}\linebreak[3]\tokenbox{~previous}\linebreak[3]\tokenbox{~url}\linebreak[3]\tokenbox{~like}\linebreak[3]\tokenbox{~this}\linebreak[3]\tokenbox{~{{}\linebreak[3]\tokenbox{~Session}\linebreak[3]\tokenbox{::}\linebreak[3]\tokenbox{get}\linebreak[3]\tokenbox{('}\linebreak[3]\tokenbox{pre}\linebreak[3]\tokenbox{vious}\linebreak[3]\tokenbox{\_}\linebreak[3]\tokenbox{url}\linebreak[3]\tokenbox{')}\linebreak[3]\tokenbox{~}}\linebreak[3]\tokenbox{}.}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{I}\linebreak[3]\tokenbox{~need}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~find}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~second}\linebreak[3]\tokenbox{~segment}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~my}\linebreak[3]\tokenbox{~previous}\linebreak[3]\tokenbox{~url}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{Thanks}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{A}\linebreak[3]\tokenbox{:}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{You}\linebreak[3]\tokenbox{~can}\linebreak[3]\tokenbox{~do}\linebreak[3]\tokenbox{~it}\linebreak[3]\tokenbox{~this}\linebreak[3]\tokenbox{~way}\linebreak[3]\tokenbox{:}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{request}\linebreak[3]\tokenbox{()}\linebreak[3]\tokenbox{->}\linebreak[3]\tokenbox{se}\linebreak[3]\tokenbox{gment}\linebreak[3]\tokenbox{(}\linebreak[3]\tokenbox{2}\linebreak[3]\tokenbox{);}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{request}\linebreak[3]\tokenbox{()}\linebreak[3]\tokenbox{~is}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~helper}\linebreak[3]\tokenbox{~function}\linebreak[3]\tokenbox{~that}\linebreak[3]\tokenbox{~returns}\linebreak[3]\tokenbox{~Illum}\linebreak[3]\tokenbox{inate}\linebreak[3]\tokenbox{\textbackslash}\linebreak[3]\tokenbox{Http}\linebreak[3]\tokenbox{\textbackslash}\linebreak[3]\tokenbox{Request}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~but}\linebreak[3]\tokenbox{~you}\linebreak[3]\tokenbox{~can}\linebreak[3]\tokenbox{~also}\linebreak[3]\tokenbox{~use}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~facade}\linebreak[3]\tokenbox{~Request}\linebreak[3]\tokenbox{~or}\linebreak[3]\tokenbox{~inject}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~class}\linebreak[3]\tokenbox{~as}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~dependency}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~your}\linebreak[3]\tokenbox{~method}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{EDIT}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{with}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~redirect}\linebreak[3]\tokenbox{~back}\linebreak[3]\tokenbox{:}\linebreak[3]\tokenbox{~redirect}\linebreak[3]\tokenbox{()}\linebreak[3]\tokenbox{->}\linebreak[3]\tokenbox{back}\linebreak[3]\tokenbox{()}\linebreak[3]\tokenbox{->}\linebreak[3]\tokenbox{get}\linebreak[3]\tokenbox{Request}\linebreak[3]\tokenbox{()}\linebreak[3]\tokenbox{->}\linebreak[3]\tokenbox{se}\linebreak[3]\tokenbox{gment}\linebreak[3]\tokenbox{(}\linebreak[3]\tokenbox{2}\linebreak[3]\tokenbox{);}\linebreak[3]\tokenbox{$\hookleftarrow$$\hookleftarrow$}\newline

}
\end{tokenized}
\end{minipage}
\vskip1.5em
\begin{minipage}{\textwidth}
\subcaption*{{\model{} Tokenization}}
\small\vspace{-0.5\baselineskip}\centering{218 tokens}
\begin{tokenized}
\parbox{\linewidth}{\small
\tokenbox{Q}\linebreak[3]\tokenbox{:}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{Get}\linebreak[3]\tokenbox{~URL}\linebreak[3]\tokenbox{~segment}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~Lar}\linebreak[3]\tokenbox{avel}\linebreak[3]\tokenbox{~5}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{For}\linebreak[3]\tokenbox{~accessing}\linebreak[3]\tokenbox{~previous}\linebreak[3]\tokenbox{~URL}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~lar}\linebreak[3]\tokenbox{avel}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~I}\linebreak[3]\tokenbox{~am}\linebreak[3]\tokenbox{~using}\linebreak[3]\tokenbox{~this}\linebreak[3]\tokenbox{~code}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~my}\linebreak[3]\tokenbox{~controller}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{\$}\linebreak[3]\tokenbox{current}\linebreak[3]\tokenbox{\_}\linebreak[3]\tokenbox{url}\linebreak[3]\tokenbox{~=}\linebreak[3]\tokenbox{~Request}\linebreak[3]\tokenbox{::}\linebreak[3]\tokenbox{url}\linebreak[3]\tokenbox{();}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{\$}\linebreak[3]\tokenbox{back}\linebreak[3]\tokenbox{\_}\linebreak[3]\tokenbox{url}\linebreak[3]\tokenbox{~=}\linebreak[3]\tokenbox{~redirect}\linebreak[3]\tokenbox{()->}\linebreak[3]\tokenbox{back}\linebreak[3]\tokenbox{()->}\linebreak[3]\tokenbox{get}\linebreak[3]\tokenbox{Target}\linebreak[3]\tokenbox{Url}\linebreak[3]\tokenbox{();}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{if}\linebreak[3]\tokenbox{~(\$}\linebreak[3]\tokenbox{current}\linebreak[3]\tokenbox{\_}\linebreak[3]\tokenbox{url}\linebreak[3]\tokenbox{~!=}\linebreak[3]\tokenbox{~\$}\linebreak[3]\tokenbox{back}\linebreak[3]\tokenbox{\_}\linebreak[3]\tokenbox{url}\linebreak[3]\tokenbox{)}\linebreak[3]\tokenbox{~{}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{~~}\linebreak[3]\tokenbox{Session}\linebreak[3]\tokenbox{::}\linebreak[3]\tokenbox{put}\linebreak[3]\tokenbox{('}\linebreak[3]\tokenbox{previous}\linebreak[3]\tokenbox{\_}\linebreak[3]\tokenbox{url}\linebreak[3]\tokenbox{',}\linebreak[3]\tokenbox{~redirect}\linebreak[3]\tokenbox{()->}\linebreak[3]\tokenbox{back}\linebreak[3]\tokenbox{()->}\linebreak[3]\tokenbox{get}\linebreak[3]\tokenbox{Target}\linebreak[3]\tokenbox{Url}\linebreak[3]\tokenbox{());}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{}}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{This}\linebreak[3]\tokenbox{~method}\linebreak[3]\tokenbox{~helps}\linebreak[3]\tokenbox{~main}\linebreak[3]\tokenbox{ta}\linebreak[3]\tokenbox{inging}\linebreak[3]\tokenbox{~previous}\linebreak[3]\tokenbox{~url}\linebreak[3]\tokenbox{~even}\linebreak[3]\tokenbox{~when}\linebreak[3]\tokenbox{~server}\linebreak[3]\tokenbox{~side}\linebreak[3]\tokenbox{~validation}\linebreak[3]\tokenbox{~fails}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{In}\linebreak[3]\tokenbox{~my}\linebreak[3]\tokenbox{~blade}\linebreak[3]\tokenbox{~I}\linebreak[3]\tokenbox{~access}\linebreak[3]\tokenbox{~previous}\linebreak[3]\tokenbox{~url}\linebreak[3]\tokenbox{~like}\linebreak[3]\tokenbox{~this}\linebreak[3]\tokenbox{~{{}\linebreak[3]\tokenbox{~Session}\linebreak[3]\tokenbox{::}\linebreak[3]\tokenbox{get}\linebreak[3]\tokenbox{('}\linebreak[3]\tokenbox{previous}\linebreak[3]\tokenbox{\_}\linebreak[3]\tokenbox{url}\linebreak[3]\tokenbox{')}\linebreak[3]\tokenbox{~}}}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{I}\linebreak[3]\tokenbox{~need}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~find}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~second}\linebreak[3]\tokenbox{~segment}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~my}\linebreak[3]\tokenbox{~previous}\linebreak[3]\tokenbox{~url}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{Thanks}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{A}\linebreak[3]\tokenbox{:}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{You}\linebreak[3]\tokenbox{~can}\linebreak[3]\tokenbox{~do}\linebreak[3]\tokenbox{~it}\linebreak[3]\tokenbox{~this}\linebreak[3]\tokenbox{~way}\linebreak[3]\tokenbox{:}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{request}\linebreak[3]\tokenbox{()->}\linebreak[3]\tokenbox{segment}\linebreak[3]\tokenbox{(}\linebreak[3]\tokenbox{2}\linebreak[3]\tokenbox{);}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{request}\linebreak[3]\tokenbox{()}\linebreak[3]\tokenbox{~is}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~helper}\linebreak[3]\tokenbox{~function}\linebreak[3]\tokenbox{~that}\linebreak[3]\tokenbox{~returns}\linebreak[3]\tokenbox{~Ill}\linebreak[3]\tokenbox{um}\linebreak[3]\tokenbox{inate}\linebreak[3]\tokenbox{\textbackslash}\linebreak[3]\tokenbox{Http}\linebreak[3]\tokenbox{\textbackslash}\linebreak[3]\tokenbox{Request}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~but}\linebreak[3]\tokenbox{~you}\linebreak[3]\tokenbox{~can}\linebreak[3]\tokenbox{~also}\linebreak[3]\tokenbox{~use}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~fac}\linebreak[3]\tokenbox{ade}\linebreak[3]\tokenbox{~Request}\linebreak[3]\tokenbox{~or}\linebreak[3]\tokenbox{~inject}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~class}\linebreak[3]\tokenbox{~as}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~dependency}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~your}\linebreak[3]\tokenbox{~method}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{EDIT}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{with}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~redirect}\linebreak[3]\tokenbox{~back}\linebreak[3]\tokenbox{:}\linebreak[3]\tokenbox{~redirect}\linebreak[3]\tokenbox{()->}\linebreak[3]\tokenbox{back}\linebreak[3]\tokenbox{()->}\linebreak[3]\tokenbox{get}\linebreak[3]\tokenbox{Request}\linebreak[3]\tokenbox{()->}\linebreak[3]\tokenbox{segment}\linebreak[3]\tokenbox{(}\linebreak[3]\tokenbox{2}\linebreak[3]\tokenbox{);}\linebreak[3]\tokenbox{$\hookleftarrow$$\hookleftarrow$}\newline

}
\end{tokenized}
\end{minipage}

==> Figures/tokenization/examples_new/USPTO_Backgrounds.tex <==
\begin{minipage}{\textwidth}
\subcaption*{{GPT-2 Tokenization}}
\small\vspace{-0.5\baselineskip}\centering{216 tokens}
\begin{tokenized}
\parbox{\linewidth}{\small
\tokenbox{1}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~Field}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~Invention}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{The}\linebreak[3]\tokenbox{~present}\linebreak[3]\tokenbox{~invention}\linebreak[3]\tokenbox{~relates}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~medical}\linebreak[3]\tokenbox{~instruments}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~more}\linebreak[3]\tokenbox{~particularly}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~an}\linebreak[3]\tokenbox{~end}\linebreak[3]\tokenbox{oscope}\linebreak[3]\tokenbox{~having}\linebreak[3]\tokenbox{~flexible}\linebreak[3]\tokenbox{~tubes}\linebreak[3]\tokenbox{~within}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~passive}\linebreak[3]\tokenbox{~def}\linebreak[3]\tokenbox{lection}\linebreak[3]\tokenbox{~section}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{2}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~Prior}\linebreak[3]\tokenbox{~Art}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{End}\linebreak[3]\tokenbox{osc}\linebreak[3]\tokenbox{opes}\linebreak[3]\tokenbox{~with}\linebreak[3]\tokenbox{~passive}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~active}\linebreak[3]\tokenbox{~def}\linebreak[3]\tokenbox{lection}\linebreak[3]\tokenbox{~sections}\linebreak[3]\tokenbox{~are}\linebreak[3]\tokenbox{~known}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~art}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~U}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{S}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~Pat}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~No}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~4}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{580}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{551}\linebreak[3]\tokenbox{~shows}\linebreak[3]\tokenbox{~an}\linebreak[3]\tokenbox{~end}\linebreak[3]\tokenbox{oscope}\linebreak[3]\tokenbox{~with}\linebreak[3]\tokenbox{~an}\linebreak[3]\tokenbox{~elong}\linebreak[3]\tokenbox{ated}\linebreak[3]\tokenbox{~flexible}\linebreak[3]\tokenbox{~plastic}\linebreak[3]\tokenbox{~tube}\linebreak[3]\tokenbox{~comprising}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~continuous}\linebreak[3]\tokenbox{~sequence}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~connected}\linebreak[3]\tokenbox{~verte}\linebreak[3]\tokenbox{bra}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{like}\linebreak[3]\tokenbox{~elements}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~U}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{S}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~Pat}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~No}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~3}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{162}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{214}\linebreak[3]\tokenbox{~discl}\linebreak[3]\tokenbox{oses}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~thin}\linebreak[3]\tokenbox{~wall}\linebreak[3]\tokenbox{ed}\linebreak[3]\tokenbox{~tube}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~elastic}\linebreak[3]\tokenbox{~material}\linebreak[3]\tokenbox{~internally}\linebreak[3]\tokenbox{~supported}\linebreak[3]\tokenbox{~throughout}\linebreak[3]\tokenbox{~its}\linebreak[3]\tokenbox{~length}\linebreak[3]\tokenbox{~by}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~series}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~tub}\linebreak[3]\tokenbox{ular}\linebreak[3]\tokenbox{~rigid}\linebreak[3]\tokenbox{~rings}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~In}\linebreak[3]\tokenbox{~one}\linebreak[3]\tokenbox{~prior}\linebreak[3]\tokenbox{~art}\linebreak[3]\tokenbox{~embodiment}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~control}\linebreak[3]\tokenbox{~wires}\linebreak[3]\tokenbox{~from}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~def}\linebreak[3]\tokenbox{lection}\linebreak[3]\tokenbox{~control}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~dist}\linebreak[3]\tokenbox{al}\linebreak[3]\tokenbox{~tip}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~active}\linebreak[3]\tokenbox{~def}\linebreak[3]\tokenbox{lection}\linebreak[3]\tokenbox{~are}\linebreak[3]\tokenbox{~provided}\linebreak[3]\tokenbox{~with}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~wire}\linebreak[3]\tokenbox{~she}\linebreak[3]\tokenbox{ath}\linebreak[3]\tokenbox{~along}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~passive}\linebreak[3]\tokenbox{~def}\linebreak[3]\tokenbox{lection}\linebreak[3]\tokenbox{~section}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~The}\linebreak[3]\tokenbox{~wire}\linebreak[3]\tokenbox{~she}\linebreak[3]\tokenbox{ath}\linebreak[3]\tokenbox{~comprises}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~co}\linebreak[3]\tokenbox{iled}\linebreak[3]\tokenbox{~wire}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~form}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~flexible}\linebreak[3]\tokenbox{~tube}\linebreak[3]\tokenbox{~around}\linebreak[3]\tokenbox{~each}\linebreak[3]\tokenbox{~control}\linebreak[3]\tokenbox{~wire}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~A}\linebreak[3]\tokenbox{~problem}\linebreak[3]\tokenbox{~exists}\linebreak[3]\tokenbox{~with}\linebreak[3]\tokenbox{~these}\linebreak[3]\tokenbox{~coil}\linebreak[3]\tokenbox{~wire}\linebreak[3]\tokenbox{~she}\linebreak[3]\tokenbox{aths}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~that}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~coil}\linebreak[3]\tokenbox{~shape}\linebreak[3]\tokenbox{~can}\linebreak[3]\tokenbox{~expand}\linebreak[3]\tokenbox{~during}\linebreak[3]\tokenbox{~compression}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~This}\linebreak[3]\tokenbox{~can}\linebreak[3]\tokenbox{~result}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~loss}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~def}\linebreak[3]\tokenbox{lection}\linebreak[3]\tokenbox{~at}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~active}\linebreak[3]\tokenbox{~def}\linebreak[3]
}
\end{tokenized}
\end{minipage}
\vskip1.5em
\begin{minipage}{\textwidth}
\subcaption*{{\model{} Tokenization}}
\small\vspace{-0.5\baselineskip}\centering{203 tokens}
\begin{tokenized}
\parbox{\linewidth}{\small
\tokenbox{1}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~Field}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~Invention}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{The}\linebreak[3]\tokenbox{~present}\linebreak[3]\tokenbox{~invention}\linebreak[3]\tokenbox{~relates}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~medical}\linebreak[3]\tokenbox{~instruments}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~more}\linebreak[3]\tokenbox{~particularly}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~an}\linebreak[3]\tokenbox{~end}\linebreak[3]\tokenbox{oscope}\linebreak[3]\tokenbox{~having}\linebreak[3]\tokenbox{~flexible}\linebreak[3]\tokenbox{~tubes}\linebreak[3]\tokenbox{~within}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~passive}\linebreak[3]\tokenbox{~deflection}\linebreak[3]\tokenbox{~section}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{2}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~Prior}\linebreak[3]\tokenbox{~Art}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{End}\linebreak[3]\tokenbox{osc}\linebreak[3]\tokenbox{opes}\linebreak[3]\tokenbox{~with}\linebreak[3]\tokenbox{~passive}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~active}\linebreak[3]\tokenbox{~deflection}\linebreak[3]\tokenbox{~sections}\linebreak[3]\tokenbox{~are}\linebreak[3]\tokenbox{~known}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~art}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~U}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{S}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~Pat}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~No}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~4}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{580}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{551}\linebreak[3]\tokenbox{~shows}\linebreak[3]\tokenbox{~an}\linebreak[3]\tokenbox{~end}\linebreak[3]\tokenbox{oscope}\linebreak[3]\tokenbox{~with}\linebreak[3]\tokenbox{~an}\linebreak[3]\tokenbox{~elongated}\linebreak[3]\tokenbox{~flexible}\linebreak[3]\tokenbox{~plastic}\linebreak[3]\tokenbox{~tube}\linebreak[3]\tokenbox{~comprising}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~continuous}\linebreak[3]\tokenbox{~sequence}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~connected}\linebreak[3]\tokenbox{~vertebra}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{like}\linebreak[3]\tokenbox{~elements}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~U}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{S}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~Pat}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~No}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~3}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{162}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{214}\linebreak[3]\tokenbox{~discloses}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~thin}\linebreak[3]\tokenbox{~wall}\linebreak[3]\tokenbox{ed}\linebreak[3]\tokenbox{~tube}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~elastic}\linebreak[3]\tokenbox{~material}\linebreak[3]\tokenbox{~internally}\linebreak[3]\tokenbox{~supported}\linebreak[3]\tokenbox{~throughout}\linebreak[3]\tokenbox{~its}\linebreak[3]\tokenbox{~length}\linebreak[3]\tokenbox{~by}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~series}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~tubular}\linebreak[3]\tokenbox{~rigid}\linebreak[3]\tokenbox{~rings}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~In}\linebreak[3]\tokenbox{~one}\linebreak[3]\tokenbox{~prior}\linebreak[3]\tokenbox{~art}\linebreak[3]\tokenbox{~embodiment}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~control}\linebreak[3]\tokenbox{~wires}\linebreak[3]\tokenbox{~from}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~deflection}\linebreak[3]\tokenbox{~control}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~distal}\linebreak[3]\tokenbox{~tip}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~active}\linebreak[3]\tokenbox{~deflection}\linebreak[3]\tokenbox{~are}\linebreak[3]\tokenbox{~provided}\linebreak[3]\tokenbox{~with}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~wire}\linebreak[3]\tokenbox{~sheath}\linebreak[3]\tokenbox{~along}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~passive}\linebreak[3]\tokenbox{~deflection}\linebreak[3]\tokenbox{~section}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~The}\linebreak[3]\tokenbox{~wire}\linebreak[3]\tokenbox{~sheath}\linebreak[3]\tokenbox{~comprises}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~co}\linebreak[3]\tokenbox{iled}\linebreak[3]\tokenbox{~wire}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~form}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~flexible}\linebreak[3]\tokenbox{~tube}\linebreak[3]\tokenbox{~around}\linebreak[3]\tokenbox{~each}\linebreak[3]\tokenbox{~control}\linebreak[3]\tokenbox{~wire}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~A}\linebreak[3]\tokenbox{~problem}\linebreak[3]\tokenbox{~exists}\linebreak[3]\tokenbox{~with}\linebreak[3]\tokenbox{~these}\linebreak[3]\tokenbox{~coil}\linebreak[3]\tokenbox{~wire}\linebreak[3]\tokenbox{~sheath}\linebreak[3]\tokenbox{s}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~that}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~coil}\linebreak[3]\tokenbox{~shape}\linebreak[3]\tokenbox{~can}\linebreak[3]\tokenbox{~expand}\linebreak[3]\tokenbox{~during}\linebreak[3]\tokenbox{~compression}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~This}\linebreak[3]\tokenbox{~can}\linebreak[3]\tokenbox{~result}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~loss}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~deflection}\linebreak[3]\tokenbox{~at}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~active}\linebreak[3]\tokenbox{~def}\linebreak[3]
}
\end{tokenized}
\end{minipage}

==> Figures/tokenization/examples_new/Ubuntu_IRC.tex <==
\begin{minipage}{\textwidth}
\subcaption*{{GPT-2 Tokenization}}
\small\vspace{-0.5\baselineskip}\centering{406 tokens}
\begin{tokenized}
\parbox{\linewidth}{\small
\tokenbox{\#}\linebreak[3]\tokenbox{ju}\linebreak[3]\tokenbox{ju}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{dev}\linebreak[3]\tokenbox{~2012}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{10}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{29}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{<}\linebreak[3]\tokenbox{rog}\linebreak[3]\tokenbox{>}\linebreak[3]\tokenbox{~n}\linebreak[3]\tokenbox{iem}\linebreak[3]\tokenbox{ey}\linebreak[3]\tokenbox{er}\linebreak[3]\tokenbox{:}\linebreak[3]\tokenbox{~mind}\linebreak[3]\tokenbox{~works}\linebreak[3]\tokenbox{~find}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~i}\linebreak[3]\tokenbox{~*}\linebreak[3]\tokenbox{think}\linebreak[3]\tokenbox{*}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{<}\linebreak[3]\tokenbox{rog}\linebreak[3]\tokenbox{>}\linebreak[3]\tokenbox{~s}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{mind}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{mine}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{<}\linebreak[3]\tokenbox{rog}\linebreak[3]\tokenbox{>}\linebreak[3]\tokenbox{~s}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{find}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{fine}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{~:-)}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{<}\linebreak[3]\tokenbox{A}\linebreak[3]\tokenbox{ram}\linebreak[3]\tokenbox{>}\linebreak[3]\tokenbox{~rog}\linebreak[3]\tokenbox{:}\linebreak[3]\tokenbox{~any}\linebreak[3]\tokenbox{~idea}\linebreak[3]\tokenbox{~how}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~rewrite}\linebreak[3]\tokenbox{~code}\linebreak[3]\tokenbox{~that}\linebreak[3]\tokenbox{~uses}\linebreak[3]\tokenbox{~/}\linebreak[3]\tokenbox{sr}\linebreak[3]\tokenbox{v}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~Plan}\linebreak[3]\tokenbox{~9}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~run}\linebreak[3]\tokenbox{~under}\linebreak[3]\tokenbox{~plan}\linebreak[3]\tokenbox{9}\linebreak[3]\tokenbox{port}\linebreak[3]\tokenbox{?}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{<}\linebreak[3]\tokenbox{A}\linebreak[3]\tokenbox{ram}\linebreak[3]\tokenbox{>}\linebreak[3]\tokenbox{~I}\linebreak[3]\tokenbox{'m}\linebreak[3]\tokenbox{~trying}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~port}\linebreak[3]\tokenbox{~history}\linebreak[3]\tokenbox{(}\linebreak[3]\tokenbox{1}\linebreak[3]\tokenbox{).}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{<}\linebreak[3]\tokenbox{A}\linebreak[3]\tokenbox{ram}\linebreak[3]\tokenbox{>}\linebreak[3]\tokenbox{~d}\linebreak[3]\tokenbox{ave}\linebreak[3]\tokenbox{che}\linebreak[3]\tokenbox{ney}\linebreak[3]\tokenbox{:}\linebreak[3]\tokenbox{~http}\linebreak[3]\tokenbox{://}\linebreak[3]\tokenbox{paste}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{ubuntu}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{com}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{13}\linebreak[3]\tokenbox{15}\linebreak[3]\tokenbox{554}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{<}\linebreak[3]\tokenbox{d}\linebreak[3]\tokenbox{ave}\linebreak[3]\tokenbox{che}\linebreak[3]\tokenbox{ney}\linebreak[3]\tokenbox{>}\linebreak[3]\tokenbox{~Aram}\linebreak[3]\tokenbox{:}\linebreak[3]\tokenbox{~ty}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{<}\linebreak[3]\tokenbox{A}\linebreak[3]\tokenbox{ram}\linebreak[3]\tokenbox{>}\linebreak[3]\tokenbox{~cheers}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{<}\linebreak[3]\tokenbox{ni}\linebreak[3]\tokenbox{em}\linebreak[3]\tokenbox{ey}\linebreak[3]\tokenbox{er}\linebreak[3]\tokenbox{>}\linebreak[3]\tokenbox{~rog}\linebreak[3]\tokenbox{pe}\linebreak[3]\tokenbox{ppe}\linebreak[3]\tokenbox{:}\linebreak[3]\tokenbox{~https}\linebreak[3]\tokenbox{://}\linebreak[3]\tokenbox{cod}\linebreak[3]\tokenbox{ere}\linebreak[3]\tokenbox{view}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{app}\linebreak[3]\tokenbox{spot}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{com}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{67}\linebreak[3]\tokenbox{200}\linebreak[3]\tokenbox{49}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{<}\linebreak[3]\tokenbox{d}\linebreak[3]\tokenbox{ave}\linebreak[3]\tokenbox{che}\linebreak[3]\tokenbox{ney}\linebreak[3]\tokenbox{>}\linebreak[3]\tokenbox{~\$}\linebreak[3]\tokenbox{~ls}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{1}\linebreak[3]\tokenbox{~/}\linebreak[3]\tokenbox{tmp}\linebreak[3]\tokenbox{~|}\linebreak[3]\tokenbox{~w}\linebreak[3]\tokenbox{c}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{l}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{<}\linebreak[3]\tokenbox{d}\linebreak[3]\tokenbox{ave}\linebreak[3]\tokenbox{che}\linebreak[3]\tokenbox{ney}\linebreak[3]\tokenbox{>}\linebreak[3]\tokenbox{~2017}\linebreak[3]\tokenbox{6}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{<}\linebreak[3]\tokenbox{d}\linebreak[3]\tokenbox{ave}\linebreak[3]\tokenbox{che}\linebreak[3]\tokenbox{ney}\linebreak[3]\tokenbox{>}\linebreak[3]\tokenbox{~prot}\linebreak[3]\tokenbox{ip}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~don}\linebreak[3]\tokenbox{'t}\linebreak[3]\tokenbox{~leave}\linebreak[3]\tokenbox{~tests}\linebreak[3]\tokenbox{~running}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~loop}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{<}\linebreak[3]\tokenbox{d}\linebreak[3]\tokenbox{ave}\linebreak[3]\tokenbox{che}\linebreak[3]\tokenbox{ney}\linebreak[3]\tokenbox{>}\linebreak[3]\tokenbox{~http}\linebreak[3]\tokenbox{://}\linebreak[3]\tokenbox{paste}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{ubuntu}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{com}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{13}\linebreak[3]\tokenbox{157}\linebreak[3]\tokenbox{24}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{~<<}\linebreak[3]\tokenbox{~24}\linebreak[3]\tokenbox{~hour}\linebreak[3]\tokenbox{~stress}\linebreak[3]\tokenbox{~test}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{<}\linebreak[3]\tokenbox{d}\linebreak[3]\tokenbox{ave}\linebreak[3]\tokenbox{che}\linebreak[3]\tokenbox{ney}\linebreak[3]\tokenbox{>}\linebreak[3]\tokenbox{~no}\linebreak[3]\tokenbox{~G}\linebreak[3]\tokenbox{OM}\linebreak[3]\tokenbox{AX}\linebreak[3]\tokenbox{PR}\linebreak[3]\tokenbox{OC}\linebreak[3]\tokenbox{S}\linebreak[3]\tokenbox{~tom}\linebreak[3]\tokenbox{f}\linebreak[3]\tokenbox{ool}\linebreak[3]\tokenbox{ery}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{<}\linebreak[3]\tokenbox{d}\linebreak[3]\tokenbox{ave}\linebreak[3]\tokenbox{che}\linebreak[3]\tokenbox{ney}\linebreak[3]\tokenbox{>}\linebreak[3]\tokenbox{~just}\linebreak[3]\tokenbox{~while}\linebreak[3]\tokenbox{~true}\linebreak[3]\tokenbox{~;}\linebreak[3]\tokenbox{~do}\linebreak[3]\tokenbox{~go}\linebreak[3]\tokenbox{~test}\linebreak[3]\tokenbox{~./}\linebreak[3]\tokenbox{...}\linebreak[3]\tokenbox{~;}\linebreak[3]\tokenbox{~done}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{\#}\linebreak[3]\tokenbox{ju}\linebreak[3]\tokenbox{ju}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{dev}\linebreak[3]\tokenbox{~2012}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{10}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{30}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{<}\linebreak[3]\tokenbox{Sp}\linebreak[3]\tokenbox{am}\linebreak[3]\tokenbox{ap}\linebreak[3]\tokenbox{S}\linebreak[3]\tokenbox{>}\linebreak[3]\tokenbox{~Hey}\linebreak[3]\tokenbox{~can}\linebreak[3]\tokenbox{~somebody}\linebreak[3]\tokenbox{~from}\linebreak[3]\tokenbox{~ju}\linebreak[3]\tokenbox{ju}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{core}\linebreak[3]\tokenbox{~please}\linebreak[3]\tokenbox{~come}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~this}\linebreak[3]\tokenbox{~session}\linebreak[3]\tokenbox{~at}\linebreak[3]\tokenbox{~11}\linebreak[3]\tokenbox{:}\linebreak[3]\tokenbox{00}\linebreak[3]\tokenbox{:}\linebreak[3]\tokenbox{~}\linebreak[3]\tokenbox{~http}\linebreak[3]\tokenbox{://}\linebreak[3]\tokenbox{sum}\linebreak[3]\tokenbox{mit}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{ubuntu}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{com}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{uds}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{r}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{me}\linebreak[3]\tokenbox{eting}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{213}\linebreak[3]\tokenbox{26}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{server}\linebreak[3]\tokenbox{cloud}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{r}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{ju}\linebreak[3]\tokenbox{ju}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{ci}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{<}\linebreak[3]\tokenbox{rog}\linebreak[3]\tokenbox{pe}\linebreak[3]\tokenbox{ppe}\linebreak[3]\tokenbox{>}\linebreak[3]\tokenbox{~Sp}\linebreak[3]\tokenbox{am}\linebreak[3]\tokenbox{ap}\linebreak[3]\tokenbox{S}\linebreak[3]\tokenbox{:}\linebreak[3]\tokenbox{~will}\linebreak[3]\tokenbox{~do}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{<}\linebreak[3]\tokenbox{Sp}\linebreak[3]\tokenbox{am}\linebreak[3]\tokenbox{ap}\linebreak[3]\tokenbox{S}\linebreak[3]\tokenbox{>}\linebreak[3]\tokenbox{~rog}\linebreak[3]\tokenbox{pe}\linebreak[3]\tokenbox{ppe}\linebreak[3]\tokenbox{:}\linebreak[3]\tokenbox{~ty}\linebreak[3]\tokenbox{!}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{<}\linebreak[3]\tokenbox{Sp}\linebreak[3]\tokenbox{am}\linebreak[3]\tokenbox{ap}\linebreak[3]\tokenbox{S}\linebreak[3]\tokenbox{>}\linebreak[3]\tokenbox{~anybody}\linebreak[3]\tokenbox{~from}\linebreak[3]\tokenbox{~go}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{aware}\linebreak[3]\tokenbox{~team}\linebreak[3]\tokenbox{~please}\linebreak[3]\tokenbox{~join}\linebreak[3]\tokenbox{~us}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~B}\linebreak[3]\tokenbox{3}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{M}\linebreak[3]\tokenbox{1}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{<}\linebreak[3]\tokenbox{Sp}\linebreak[3]\tokenbox{am}\linebreak[3]\tokenbox{ap}\linebreak[3]\tokenbox{S}\linebreak[3]\tokenbox{>}\linebreak[3]\tokenbox{~d}\linebreak[3]\tokenbox{ave}\linebreak[3]\tokenbox{che}\linebreak[3]\tokenbox{ney}\linebreak[3]\tokenbox{:}\linebreak[3]\tokenbox{~around}\linebreak[3]\tokenbox{?}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{<}\linebreak[3]\tokenbox{Sp}\linebreak[3]\tokenbox{am}\linebreak[3]\tokenbox{ap}\linebreak[3]\tokenbox{S}\linebreak[3]\tokenbox{>}\linebreak[3]\tokenbox{~rog}\linebreak[3]\tokenbox{pe}\linebreak[3]\tokenbox{ppe}\linebreak[3]\tokenbox{:}\linebreak[3]\tokenbox{~?}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{<}\linebreak[3]\tokenbox{Sp}\linebreak[3]\tokenbox{am}\linebreak[3]\tokenbox{ap}\linebreak[3]\tokenbox{S}\linebreak[3]\tokenbox{>}\linebreak[3]
}
\end{tokenized}
\end{minipage}
\vskip1.5em
\begin{minipage}{\textwidth}
\subcaption*{{\model{} Tokenization}}
\small\vspace{-0.5\baselineskip}\centering{412 tokens}
\begin{tokenized}
\parbox{\linewidth}{\small
\tokenbox{\#}\linebreak[3]\tokenbox{ju}\linebreak[3]\tokenbox{ju}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{dev}\linebreak[3]\tokenbox{~2012}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{10}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{29}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{<}\linebreak[3]\tokenbox{rog}\linebreak[3]\tokenbox{>}\linebreak[3]\tokenbox{~n}\linebreak[3]\tokenbox{iem}\linebreak[3]\tokenbox{eyer}\linebreak[3]\tokenbox{:}\linebreak[3]\tokenbox{~mind}\linebreak[3]\tokenbox{~works}\linebreak[3]\tokenbox{~find}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~i}\linebreak[3]\tokenbox{~*}\linebreak[3]\tokenbox{think}\linebreak[3]\tokenbox{*}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{<}\linebreak[3]\tokenbox{rog}\linebreak[3]\tokenbox{>}\linebreak[3]\tokenbox{~s}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{mind}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{mine}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{<}\linebreak[3]\tokenbox{rog}\linebreak[3]\tokenbox{>}\linebreak[3]\tokenbox{~s}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{find}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{fine}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{~:-)}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{<}\linebreak[3]\tokenbox{Ar}\linebreak[3]\tokenbox{am}\linebreak[3]\tokenbox{>}\linebreak[3]\tokenbox{~ro}\linebreak[3]\tokenbox{g}\linebreak[3]\tokenbox{:}\linebreak[3]\tokenbox{~any}\linebreak[3]\tokenbox{~idea}\linebreak[3]\tokenbox{~how}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~rewrite}\linebreak[3]\tokenbox{~code}\linebreak[3]\tokenbox{~that}\linebreak[3]\tokenbox{~uses}\linebreak[3]\tokenbox{~/}\linebreak[3]\tokenbox{sr}\linebreak[3]\tokenbox{v}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~Plan}\linebreak[3]\tokenbox{~9}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~run}\linebreak[3]\tokenbox{~under}\linebreak[3]\tokenbox{~plan}\linebreak[3]\tokenbox{9}\linebreak[3]\tokenbox{port}\linebreak[3]\tokenbox{?}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{<}\linebreak[3]\tokenbox{Ar}\linebreak[3]\tokenbox{am}\linebreak[3]\tokenbox{>}\linebreak[3]\tokenbox{~I}\linebreak[3]\tokenbox{'m}\linebreak[3]\tokenbox{~trying}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~port}\linebreak[3]\tokenbox{~history}\linebreak[3]\tokenbox{(}\linebreak[3]\tokenbox{1}\linebreak[3]\tokenbox{).}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{<}\linebreak[3]\tokenbox{Ar}\linebreak[3]\tokenbox{am}\linebreak[3]\tokenbox{>}\linebreak[3]\tokenbox{~d}\linebreak[3]\tokenbox{ave}\linebreak[3]\tokenbox{che}\linebreak[3]\tokenbox{ney}\linebreak[3]\tokenbox{:}\linebreak[3]\tokenbox{~http}\linebreak[3]\tokenbox{://}\linebreak[3]\tokenbox{paste}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{ubuntu}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{com}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{13}\linebreak[3]\tokenbox{15}\linebreak[3]\tokenbox{554}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{<}\linebreak[3]\tokenbox{d}\linebreak[3]\tokenbox{ave}\linebreak[3]\tokenbox{che}\linebreak[3]\tokenbox{ney}\linebreak[3]\tokenbox{>}\linebreak[3]\tokenbox{~Ar}\linebreak[3]\tokenbox{am}\linebreak[3]\tokenbox{:}\linebreak[3]\tokenbox{~ty}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{<}\linebreak[3]\tokenbox{Ar}\linebreak[3]\tokenbox{am}\linebreak[3]\tokenbox{>}\linebreak[3]\tokenbox{~che}\linebreak[3]\tokenbox{ers}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{<}\linebreak[3]\tokenbox{ni}\linebreak[3]\tokenbox{em}\linebreak[3]\tokenbox{eyer}\linebreak[3]\tokenbox{>}\linebreak[3]\tokenbox{~ro}\linebreak[3]\tokenbox{g}\linebreak[3]\tokenbox{pe}\linebreak[3]\tokenbox{p}\linebreak[3]\tokenbox{pe}\linebreak[3]\tokenbox{:}\linebreak[3]\tokenbox{~https}\linebreak[3]\tokenbox{://}\linebreak[3]\tokenbox{code}\linebreak[3]\tokenbox{review}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{app}\linebreak[3]\tokenbox{spot}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{com}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{67}\linebreak[3]\tokenbox{200}\linebreak[3]\tokenbox{49}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{<}\linebreak[3]\tokenbox{d}\linebreak[3]\tokenbox{ave}\linebreak[3]\tokenbox{che}\linebreak[3]\tokenbox{ney}\linebreak[3]\tokenbox{>}\linebreak[3]\tokenbox{~\$}\linebreak[3]\tokenbox{~ls}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{1}\linebreak[3]\tokenbox{~/}\linebreak[3]\tokenbox{tmp}\linebreak[3]\tokenbox{~|}\linebreak[3]\tokenbox{~w}\linebreak[3]\tokenbox{c}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{l}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{<}\linebreak[3]\tokenbox{d}\linebreak[3]\tokenbox{ave}\linebreak[3]\tokenbox{che}\linebreak[3]\tokenbox{ney}\linebreak[3]\tokenbox{>}\linebreak[3]\tokenbox{~201}\linebreak[3]\tokenbox{76}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{<}\linebreak[3]\tokenbox{d}\linebreak[3]\tokenbox{ave}\linebreak[3]\tokenbox{che}\linebreak[3]\tokenbox{ney}\linebreak[3]\tokenbox{>}\linebreak[3]\tokenbox{~prot}\linebreak[3]\tokenbox{ip}\linebreak[3]\tokenbox{~-}\linebreak[3]\tokenbox{~don}\linebreak[3]\tokenbox{'t}\linebreak[3]\tokenbox{~leave}\linebreak[3]\tokenbox{~tests}\linebreak[3]\tokenbox{~running}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~loop}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{<}\linebreak[3]\tokenbox{d}\linebreak[3]\tokenbox{ave}\linebreak[3]\tokenbox{che}\linebreak[3]\tokenbox{ney}\linebreak[3]\tokenbox{>}\linebreak[3]\tokenbox{~http}\linebreak[3]\tokenbox{://}\linebreak[3]\tokenbox{paste}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{ubuntu}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{com}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{13}\linebreak[3]\tokenbox{157}\linebreak[3]\tokenbox{24}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{~<<}\linebreak[3]\tokenbox{~24}\linebreak[3]\tokenbox{~hour}\linebreak[3]\tokenbox{~stress}\linebreak[3]\tokenbox{~test}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{<}\linebreak[3]\tokenbox{d}\linebreak[3]\tokenbox{ave}\linebreak[3]\tokenbox{che}\linebreak[3]\tokenbox{ney}\linebreak[3]\tokenbox{>}\linebreak[3]\tokenbox{~no}\linebreak[3]\tokenbox{~G}\linebreak[3]\tokenbox{OM}\linebreak[3]\tokenbox{AX}\linebreak[3]\tokenbox{PROC}\linebreak[3]\tokenbox{S}\linebreak[3]\tokenbox{~tom}\linebreak[3]\tokenbox{f}\linebreak[3]\tokenbox{ool}\linebreak[3]\tokenbox{ery}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{<}\linebreak[3]\tokenbox{d}\linebreak[3]\tokenbox{ave}\linebreak[3]\tokenbox{che}\linebreak[3]\tokenbox{ney}\linebreak[3]\tokenbox{>}\linebreak[3]\tokenbox{~just}\linebreak[3]\tokenbox{~while}\linebreak[3]\tokenbox{~true}\linebreak[3]\tokenbox{~;}\linebreak[3]\tokenbox{~do}\linebreak[3]\tokenbox{~go}\linebreak[3]\tokenbox{~test}\linebreak[3]\tokenbox{~./}\linebreak[3]\tokenbox{...}\linebreak[3]\tokenbox{~;}\linebreak[3]\tokenbox{~done}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{\#}\linebreak[3]\tokenbox{ju}\linebreak[3]\tokenbox{ju}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{dev}\linebreak[3]\tokenbox{~2012}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{10}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{30}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{<}\linebreak[3]\tokenbox{Sp}\linebreak[3]\tokenbox{am}\linebreak[3]\tokenbox{ap}\linebreak[3]\tokenbox{S}\linebreak[3]\tokenbox{>}\linebreak[3]\tokenbox{~Hey}\linebreak[3]\tokenbox{~can}\linebreak[3]\tokenbox{~somebody}\linebreak[3]\tokenbox{~from}\linebreak[3]\tokenbox{~ju}\linebreak[3]\tokenbox{ju}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{core}\linebreak[3]\tokenbox{~please}\linebreak[3]\tokenbox{~come}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~this}\linebreak[3]\tokenbox{~session}\linebreak[3]\tokenbox{~at}\linebreak[3]\tokenbox{~11}\linebreak[3]\tokenbox{:}\linebreak[3]\tokenbox{00}\linebreak[3]\tokenbox{:}\linebreak[3]\tokenbox{~~}\linebreak[3]\tokenbox{http}\linebreak[3]\tokenbox{://}\linebreak[3]\tokenbox{sum}\linebreak[3]\tokenbox{mit}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{ubuntu}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{com}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{uds}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{r}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{me}\linebreak[3]\tokenbox{eting}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{213}\linebreak[3]\tokenbox{26}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{server}\linebreak[3]\tokenbox{cloud}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{r}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{ju}\linebreak[3]\tokenbox{ju}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{ci}\linebreak[3]\tokenbox{/}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{<}\linebreak[3]\tokenbox{rog}\linebreak[3]\tokenbox{pe}\linebreak[3]\tokenbox{p}\linebreak[3]\tokenbox{pe}\linebreak[3]\tokenbox{>}\linebreak[3]\tokenbox{~Sp}\linebreak[3]\tokenbox{am}\linebreak[3]\tokenbox{ap}\linebreak[3]\tokenbox{S}\linebreak[3]\tokenbox{:}\linebreak[3]\tokenbox{~will}\linebreak[3]\tokenbox{~do}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{<}\linebreak[3]\tokenbox{Sp}\linebreak[3]\tokenbox{am}\linebreak[3]\tokenbox{ap}\linebreak[3]\tokenbox{S}\linebreak[3]\tokenbox{>}\linebreak[3]\tokenbox{~ro}\linebreak[3]\tokenbox{g}\linebreak[3]\tokenbox{pe}\linebreak[3]\tokenbox{p}\linebreak[3]\tokenbox{pe}\linebreak[3]\tokenbox{:}\linebreak[3]\tokenbox{~ty}\linebreak[3]\tokenbox{!}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{<}\linebreak[3]\tokenbox{Sp}\linebreak[3]\tokenbox{am}\linebreak[3]\tokenbox{ap}\linebreak[3]\tokenbox{S}\linebreak[3]\tokenbox{>}\linebreak[3]\tokenbox{~anybody}\linebreak[3]\tokenbox{~from}\linebreak[3]\tokenbox{~go}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{aware}\linebreak[3]\tokenbox{~team}\linebreak[3]\tokenbox{~please}\linebreak[3]\tokenbox{~join}\linebreak[3]\tokenbox{~us}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~B}\linebreak[3]\tokenbox{3}\linebreak[3]\tokenbox{-}\linebreak[3]\tokenbox{M}\linebreak[3]\tokenbox{1}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{<}\linebreak[3]\tokenbox{Sp}\linebreak[3]\tokenbox{am}\linebreak[3]\tokenbox{ap}\linebreak[3]\tokenbox{S}\linebreak[3]\tokenbox{>}\linebreak[3]\tokenbox{~d}\linebreak[3]\tokenbox{ave}\linebreak[3]\tokenbox{che}\linebreak[3]\tokenbox{ney}\linebreak[3]\tokenbox{:}\linebreak[3]\tokenbox{~around}\linebreak[3]\tokenbox{?}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{<}\linebreak[3]\tokenbox{Sp}\linebreak[3]\tokenbox{am}\linebreak[3]\tokenbox{ap}\linebreak[3]\tokenbox{S}\linebreak[3]\tokenbox{>}\linebreak[3]\tokenbox{~ro}\linebreak[3]\tokenbox{g}\linebreak[3]\tokenbox{pe}\linebreak[3]\tokenbox{p}\linebreak[3]\tokenbox{pe}\linebreak[3]\tokenbox{:}\linebreak[3]\tokenbox{~?}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{<}\linebreak[3]\tokenbox{Sp}\linebreak[3]\tokenbox{am}\linebreak[3]\tokenbox{ap}\linebreak[3]\tokenbox{S}\linebreak[3]\tokenbox{>}\linebreak[3]
}
\end{tokenized}
\end{minipage}

==> Figures/tokenization/examples_new/Wikipedia.tex <==
\begin{minipage}{\textwidth}
\subcaption*{{GPT-2 Tokenization}}
\small\vspace{-0.5\baselineskip}\centering{104 tokens}
\begin{tokenized}
\parbox{\linewidth}{\small
\tokenbox{Gl}\linebreak[3]\tokenbox{ene}\linebreak[3]\tokenbox{a}\linebreak[3]\tokenbox{~funer}\linebreak[3]\tokenbox{ula}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{Gl}\linebreak[3]\tokenbox{ene}\linebreak[3]\tokenbox{a}\linebreak[3]\tokenbox{~funer}\linebreak[3]\tokenbox{ula}\linebreak[3]\tokenbox{~is}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~species}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~beetle}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~family}\linebreak[3]\tokenbox{~Cer}\linebreak[3]\tokenbox{am}\linebreak[3]\tokenbox{by}\linebreak[3]\tokenbox{c}\linebreak[3]\tokenbox{idae}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~It}\linebreak[3]\tokenbox{~was}\linebreak[3]\tokenbox{~described}\linebreak[3]\tokenbox{~by}\linebreak[3]\tokenbox{~James}\linebreak[3]\tokenbox{~Thomson}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~18}\linebreak[3]\tokenbox{57}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~It}\linebreak[3]\tokenbox{~is}\linebreak[3]\tokenbox{~known}\linebreak[3]\tokenbox{~from}\linebreak[3]\tokenbox{~Sum}\linebreak[3]\tokenbox{atra}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~India}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~Malaysia}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~Java}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{Sub}\linebreak[3]\tokenbox{species}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{~Gl}\linebreak[3]\tokenbox{ene}\linebreak[3]\tokenbox{a}\linebreak[3]\tokenbox{~funer}\linebreak[3]\tokenbox{ula}\linebreak[3]\tokenbox{~funer}\linebreak[3]\tokenbox{ula}\linebreak[3]\tokenbox{~(}\linebreak[3]\tokenbox{J}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~Thomson}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~18}\linebreak[3]\tokenbox{57}\linebreak[3]\tokenbox{)}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{~Gl}\linebreak[3]\tokenbox{ene}\linebreak[3]\tokenbox{a}\linebreak[3]\tokenbox{~funer}\linebreak[3]\tokenbox{ula}\linebreak[3]\tokenbox{~j}\linebreak[3]\tokenbox{av}\linebreak[3]\tokenbox{ana}\linebreak[3]\tokenbox{~(}\linebreak[3]\tokenbox{Pic}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~1946}\linebreak[3]\tokenbox{)}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{References}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{Category}\linebreak[3]\tokenbox{:}\linebreak[3]\tokenbox{Gl}\linebreak[3]\tokenbox{ene}\linebreak[3]\tokenbox{a}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{Category}\linebreak[3]\tokenbox{:}\linebreak[3]\tokenbox{Be}\linebreak[3]\tokenbox{et}\linebreak[3]\tokenbox{les}\linebreak[3]\tokenbox{~described}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~18}\linebreak[3]\tokenbox{57}\linebreak[3]
}
\end{tokenized}
\end{minipage}
\vskip1.5em
\begin{minipage}{\textwidth}
\subcaption*{{\model{} Tokenization}}
\small\vspace{-0.5\baselineskip}\centering{108 tokens}
\begin{tokenized}
\parbox{\linewidth}{\small
\tokenbox{Gl}\linebreak[3]\tokenbox{ene}\linebreak[3]\tokenbox{a}\linebreak[3]\tokenbox{~fun}\linebreak[3]\tokenbox{er}\linebreak[3]\tokenbox{ula}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{Gl}\linebreak[3]\tokenbox{ene}\linebreak[3]\tokenbox{a}\linebreak[3]\tokenbox{~fun}\linebreak[3]\tokenbox{er}\linebreak[3]\tokenbox{ula}\linebreak[3]\tokenbox{~is}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~species}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~beet}\linebreak[3]\tokenbox{le}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~family}\linebreak[3]\tokenbox{~Cer}\linebreak[3]\tokenbox{amb}\linebreak[3]\tokenbox{yc}\linebreak[3]\tokenbox{idae}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~It}\linebreak[3]\tokenbox{~was}\linebreak[3]\tokenbox{~described}\linebreak[3]\tokenbox{~by}\linebreak[3]\tokenbox{~James}\linebreak[3]\tokenbox{~Thomson}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~18}\linebreak[3]\tokenbox{57}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~It}\linebreak[3]\tokenbox{~is}\linebreak[3]\tokenbox{~known}\linebreak[3]\tokenbox{~from}\linebreak[3]\tokenbox{~Sum}\linebreak[3]\tokenbox{atra}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~India}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~Malaysia}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~Java}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{Sub}\linebreak[3]\tokenbox{species}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{~Gl}\linebreak[3]\tokenbox{ene}\linebreak[3]\tokenbox{a}\linebreak[3]\tokenbox{~fun}\linebreak[3]\tokenbox{er}\linebreak[3]\tokenbox{ula}\linebreak[3]\tokenbox{~fun}\linebreak[3]\tokenbox{er}\linebreak[3]\tokenbox{ula}\linebreak[3]\tokenbox{~(}\linebreak[3]\tokenbox{J}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{~Thomson}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~18}\linebreak[3]\tokenbox{57}\linebreak[3]\tokenbox{)}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{~Gl}\linebreak[3]\tokenbox{ene}\linebreak[3]\tokenbox{a}\linebreak[3]\tokenbox{~fun}\linebreak[3]\tokenbox{er}\linebreak[3]\tokenbox{ula}\linebreak[3]\tokenbox{~jav}\linebreak[3]\tokenbox{ana}\linebreak[3]\tokenbox{~(}\linebreak[3]\tokenbox{Pic}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~1946}\linebreak[3]\tokenbox{)}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{References}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{$\hookleftarrow$}\newline
\tokenbox{Category}\linebreak[3]\tokenbox{:}\linebreak[3]\tokenbox{Gl}\linebreak[3]\tokenbox{ene}\linebreak[3]\tokenbox{a}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{Category}\linebreak[3]\tokenbox{:}\linebreak[3]\tokenbox{Be}\linebreak[3]\tokenbox{et}\linebreak[3]\tokenbox{les}\linebreak[3]\tokenbox{~described}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~18}\linebreak[3]\tokenbox{57}\linebreak[3]
}
\end{tokenized}
\end{minipage}

==> Figures/tokenization/examples_new/YoutubeSubtitles.tex <==
\begin{minipage}{\textwidth}
\subcaption*{{GPT-2 Tokenization}}
\small\vspace{-0.5\baselineskip}\centering{282 tokens}
\begin{tokenized}
\parbox{\linewidth}{\small
\tokenbox{Hello}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~welcome}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~another}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{ML}\linebreak[3]\tokenbox{5}\linebreak[3]\tokenbox{~neural}\linebreak[3]\tokenbox{~network}\linebreak[3]\tokenbox{~video}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{t}\linebreak[3]\tokenbox{utorial}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{I}\linebreak[3]\tokenbox{'m}\linebreak[3]\tokenbox{~following}\linebreak[3]\tokenbox{~up}\linebreak[3]\tokenbox{~on}\linebreak[3]\tokenbox{~what}\linebreak[3]\tokenbox{~I}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{did}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~previous}\linebreak[3]\tokenbox{~video}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{where}\linebreak[3]\tokenbox{~I}\linebreak[3]\tokenbox{~built}\linebreak[3]\tokenbox{~this}\linebreak[3]\tokenbox{~example}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{This}\linebreak[3]\tokenbox{~example}\linebreak[3]\tokenbox{~has}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{this}\linebreak[3]\tokenbox{~interaction}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{where}\linebreak[3]\tokenbox{~you}\linebreak[3]\tokenbox{~click}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~mouse}\linebreak[3]\tokenbox{~all}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{over}\linebreak[3]\tokenbox{~this}\linebreak[3]\tokenbox{~canvas}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~press}\linebreak[3]\tokenbox{~keys}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{to}\linebreak[3]\tokenbox{~assign}\linebreak[3]\tokenbox{~each}\linebreak[3]\tokenbox{~x}\linebreak[3]\tokenbox{y}\linebreak[3]\tokenbox{~point}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{a}\linebreak[3]\tokenbox{~label}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~C}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~D}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~E}\linebreak[3]\tokenbox{--}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{and}\linebreak[3]\tokenbox{~I}\linebreak[3]\tokenbox{~added}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~bunch}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~notes}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{since}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~previous}\linebreak[3]\tokenbox{~video}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{So}\linebreak[3]\tokenbox{~I}\linebreak[3]\tokenbox{~have}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~full}\linebreak[3]\tokenbox{~scale}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{C}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~D}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~E}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~F}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~G}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~A}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~B}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{Then}\linebreak[3]\tokenbox{~I}\linebreak[3]\tokenbox{~trained}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{model}\linebreak[3]\tokenbox{~with}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~inputs}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{being}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~x}\linebreak[3]\tokenbox{y}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~all}\linebreak[3]\tokenbox{~these}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{points}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~target}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{being}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~actual}\linebreak[3]\tokenbox{~label}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{And}\linebreak[3]\tokenbox{~once}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~model}\linebreak[3]\tokenbox{~is}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{trained}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~it}\linebreak[3]\tokenbox{~can}\linebreak[3]\tokenbox{~make}\linebreak[3]\tokenbox{~guesses}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{So}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~theory}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~I}\linebreak[3]\tokenbox{~just}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{col}\linebreak[3]\tokenbox{lected}\linebreak[3]\tokenbox{~this}\linebreak[3]\tokenbox{~data}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{set}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~trained}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~model}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{When}\linebreak[3]\tokenbox{~I}\linebreak[3]\tokenbox{~click}\linebreak[3]\tokenbox{~into}\linebreak[3]\tokenbox{~it}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{when}\linebreak[3]\tokenbox{~I}\linebreak[3]\tokenbox{~click}\linebreak[3]\tokenbox{~over}\linebreak[3]\tokenbox{~here}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{I}\linebreak[3]\tokenbox{~should}\linebreak[3]\tokenbox{~hear}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{mus}\linebreak[3]\tokenbox{ical}\linebreak[3]\tokenbox{~note}\linebreak[3]\tokenbox{~D}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{I}\linebreak[3]\tokenbox{~should}\linebreak[3]\tokenbox{~hear}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{mus}\linebreak[3]\tokenbox{ical}\linebreak[3]\tokenbox{~note}\linebreak[3]\tokenbox{~E}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~G}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~A}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{And}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~between}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~it}\linebreak[3]\tokenbox{'s}\linebreak[3]\tokenbox{~sort}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{interesting}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~see}\linebreak[3]\tokenbox{~what}\linebreak[3]\tokenbox{~I}\linebreak[3]\tokenbox{~get}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{But}\linebreak[3]\tokenbox{~it}\linebreak[3]\tokenbox{~works}\linebreak[3]\tokenbox{~as}\linebreak[3]\tokenbox{~expected}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{I}\linebreak[3]\tokenbox{~ran}\linebreak[3]\tokenbox{~into}\linebreak[3]\tokenbox{~like}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~pretty}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{significant}\linebreak[3]\tokenbox{~problem}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{while}\linebreak[3]\tokenbox{~working}\linebreak[3]\tokenbox{~on}\linebreak[3]\tokenbox{~this}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{Because}\linebreak[3]\tokenbox{~once}\linebreak[3]\tokenbox{~I}\linebreak[3]\tokenbox{'ve}\linebreak[3]\tokenbox{~collected}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{data}\linebreak[3]\tokenbox{~set}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~trained}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~model}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{if}\linebreak[3]\tokenbox{~I}\linebreak[3]\tokenbox{~had}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~bug}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~code}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{or}\linebreak[3]\tokenbox{~something}\linebreak[3]\tokenbox{~I}\linebreak[3]\tokenbox{~need}\linebreak[3]
}
\end{tokenized}
\end{minipage}
\vskip1.5em
\begin{minipage}{\textwidth}
\subcaption*{{\model{} Tokenization}}
\small\vspace{-0.5\baselineskip}\centering{283 tokens}
\begin{tokenized}
\parbox{\linewidth}{\small
\tokenbox{Hello}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~welcome}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~another}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{ML}\linebreak[3]\tokenbox{5}\linebreak[3]\tokenbox{~neural}\linebreak[3]\tokenbox{~network}\linebreak[3]\tokenbox{~video}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{t}\linebreak[3]\tokenbox{utorial}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{I}\linebreak[3]\tokenbox{'m}\linebreak[3]\tokenbox{~following}\linebreak[3]\tokenbox{~up}\linebreak[3]\tokenbox{~on}\linebreak[3]\tokenbox{~what}\linebreak[3]\tokenbox{~I}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{did}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~previous}\linebreak[3]\tokenbox{~video}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{where}\linebreak[3]\tokenbox{~I}\linebreak[3]\tokenbox{~built}\linebreak[3]\tokenbox{~this}\linebreak[3]\tokenbox{~example}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{This}\linebreak[3]\tokenbox{~example}\linebreak[3]\tokenbox{~has}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{this}\linebreak[3]\tokenbox{~interaction}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{where}\linebreak[3]\tokenbox{~you}\linebreak[3]\tokenbox{~click}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~mouse}\linebreak[3]\tokenbox{~all}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{over}\linebreak[3]\tokenbox{~this}\linebreak[3]\tokenbox{~canvas}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~press}\linebreak[3]\tokenbox{~keys}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{to}\linebreak[3]\tokenbox{~assign}\linebreak[3]\tokenbox{~each}\linebreak[3]\tokenbox{~x}\linebreak[3]\tokenbox{y}\linebreak[3]\tokenbox{~point}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{a}\linebreak[3]\tokenbox{~label}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~C}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~D}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~E}\linebreak[3]\tokenbox{--}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{and}\linebreak[3]\tokenbox{~I}\linebreak[3]\tokenbox{~added}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~bunch}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~notes}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{since}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~previous}\linebreak[3]\tokenbox{~video}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{So}\linebreak[3]\tokenbox{~I}\linebreak[3]\tokenbox{~have}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~full}\linebreak[3]\tokenbox{~scale}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{C}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~D}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~E}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~F}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~G}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~A}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~B}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{Then}\linebreak[3]\tokenbox{~I}\linebreak[3]\tokenbox{~trained}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{model}\linebreak[3]\tokenbox{~with}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~inputs}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{being}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~x}\linebreak[3]\tokenbox{y}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{~all}\linebreak[3]\tokenbox{~these}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{points}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~target}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{being}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~actual}\linebreak[3]\tokenbox{~label}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{And}\linebreak[3]\tokenbox{~once}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~model}\linebreak[3]\tokenbox{~is}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{trained}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~it}\linebreak[3]\tokenbox{~can}\linebreak[3]\tokenbox{~make}\linebreak[3]\tokenbox{~guess}\linebreak[3]\tokenbox{es}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{So}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~theory}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~I}\linebreak[3]\tokenbox{~just}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{col}\linebreak[3]\tokenbox{lected}\linebreak[3]\tokenbox{~this}\linebreak[3]\tokenbox{~data}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{set}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~trained}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~model}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{When}\linebreak[3]\tokenbox{~I}\linebreak[3]\tokenbox{~click}\linebreak[3]\tokenbox{~into}\linebreak[3]\tokenbox{~it}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{when}\linebreak[3]\tokenbox{~I}\linebreak[3]\tokenbox{~click}\linebreak[3]\tokenbox{~over}\linebreak[3]\tokenbox{~here}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{I}\linebreak[3]\tokenbox{~should}\linebreak[3]\tokenbox{~hear}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{mus}\linebreak[3]\tokenbox{ical}\linebreak[3]\tokenbox{~note}\linebreak[3]\tokenbox{~D}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{I}\linebreak[3]\tokenbox{~should}\linebreak[3]\tokenbox{~hear}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{mus}\linebreak[3]\tokenbox{ical}\linebreak[3]\tokenbox{~note}\linebreak[3]\tokenbox{~E}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~G}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~A}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{And}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~between}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{~it}\linebreak[3]\tokenbox{'s}\linebreak[3]\tokenbox{~sort}\linebreak[3]\tokenbox{~of}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{interesting}\linebreak[3]\tokenbox{~to}\linebreak[3]\tokenbox{~see}\linebreak[3]\tokenbox{~what}\linebreak[3]\tokenbox{~I}\linebreak[3]\tokenbox{~get}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{But}\linebreak[3]\tokenbox{~it}\linebreak[3]\tokenbox{~works}\linebreak[3]\tokenbox{~as}\linebreak[3]\tokenbox{~expected}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{I}\linebreak[3]\tokenbox{~ran}\linebreak[3]\tokenbox{~into}\linebreak[3]\tokenbox{~like}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~pretty}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{significant}\linebreak[3]\tokenbox{~problem}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{while}\linebreak[3]\tokenbox{~working}\linebreak[3]\tokenbox{~on}\linebreak[3]\tokenbox{~this}\linebreak[3]\tokenbox{.}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{Because}\linebreak[3]\tokenbox{~once}\linebreak[3]\tokenbox{~I}\linebreak[3]\tokenbox{'ve}\linebreak[3]\tokenbox{~collected}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{data}\linebreak[3]\tokenbox{~set}\linebreak[3]\tokenbox{~and}\linebreak[3]\tokenbox{~trained}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~model}\linebreak[3]\tokenbox{,}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{if}\linebreak[3]\tokenbox{~I}\linebreak[3]\tokenbox{~had}\linebreak[3]\tokenbox{~a}\linebreak[3]\tokenbox{~bug}\linebreak[3]\tokenbox{~in}\linebreak[3]\tokenbox{~the}\linebreak[3]\tokenbox{~code}\linebreak[3]\tokenbox{$\hookleftarrow$}\newline
\tokenbox{or}\linebreak[3]\tokenbox{~something}\linebreak[3]\tokenbox{~I}\linebreak[3]\tokenbox{~need}\linebreak[3]
}
\end{tokenized}
\end{minipage}
